Dark energy: EFTs and supergravity

The subject of this thesis is cosmological implications of string compactifications understood in a broad sense. In the first half of the thesis, we will begin by reviewing the four-dimensional description of the tree-level perturbative type IIB action. We will then review a number of open questions in cosmology and their relevance with regards to the remainder of the thesis. We will first explore some of these cosmological questions from the perspective of effective field theories motivated by supergravity. From the naturalness of dark energy and how to obtain a naturally light dark energy field in terms of the clockwork mechanism and the Dvali-Kaloper-Sorbo four-form mixing. We also discuss the coincidence problem for dynamical models of dark energy consistent with a quintessence field slowly rolling down a potential slope, of the type one would expect from the asymptotics of moduli space. In the second half of the thesis, we introduce the effects of perturbative and non-perturbative corrections to the tree-level type IIB action. We then focus on obtaining a viable model of quintessence from the type IIB effective field theory. However, we are able to show that such a model must have a non-supersymmetric Minkowski vacuum at leading order. When we consider the effects of quantum fluctuations during the early Universe, we see that such models must have extremely fine-tuned initial conditions to describe a slow-rolling scalar field at present times. We conclude that quintessence faces more challenges than a true cosmological constant, to the point that quintessence is very unattractive for model building modulo a ruling out of the cosmological constant by observations. Following this line of reasoning, we consider whether other perturbative corrections can generate de Sitter solutions in an appropriate setting.

==> Appendices/gbds_details.tex <==
\chapter{Some explicit results for the quadratic curvature corrections}

\section{Coefficients of the leading order correction in the GB coupling expansion}\label{app:coeffs}
\begin{align}
    A_{n,p}&= 4n(p-7)(1-p) + 4n^2(1-p) + 4p(p-11) + 48 \ ,
    \\
    B_{n,p}&= -4\left[(n - 1)p^2 + (n^2 - 4n + 3)p - n^2 + 3n\right](p - 1)\ ,
    \\
    C_{n,p}&= 8\left[(n -1 )p^3 + (n^2 -11n + 14)p^2 - (2n^2 - 19n + 27)p + n^2 - 7n + 12\right]\ ,
    \\
    D_{n,p}&= 8(p- n)(np - n - p + 3)(p - 1)\ ,
    \\
    E_{n,p}&=4\left[2(3n - 5)p^3 - (2n^2 + 15n - 31)p^2 + (3n^2 + 12n - 31)p + n^2 - 7n + 12\right],
    \\
    F_{n,p}&=4(p - 1)(4n^2p^2 - 7n^2p - 7np^2 + n^2 + 14np + p^2 - 3n - 3p)\ .
\end{align}


\section{Field equations}
\label{sec:fieldeqs}

The $D$-dimensional field equations associated with \eqref{eq:action} read:
\begin{align}
	\begin{split}
		\label{eq:EinsteinD}
		0&=f(\varphi)\left(4R_A^{~C}R_{BC}+\dfrac12\mathcal{G}g_{AB}-2RR_{AB}+4R^{CD}R_{ACBD}-2R_A^{~CDE}R_{BCDE}\right)
		\\
		&\quad+\dfrac12\nabla_A\varphi\nabla_B\varphi-\dfrac14(\nabla\varphi)^2g_{AB}+2f'(\varphi)\left(R\,\nabla_A\nabla_B\varphi-4R_{(B}^{~C}\nabla_{A)}\nabla_C\varphi+2G_{AB}\Box\varphi\right.
		\\
		&\quad+2g_{AB}R^{CD}\nabla_C\nabla_D\varphi-2R_{ACBD}\nabla^C\nabla^D\varphi\left.\right)+2f''(\varphi)\left[R\,\nabla_A\varphi\nabla_B\varphi\right.\vphantom{\dfrac12}
		\\
		&\quad\left.-4R_{C(B}\nabla_{A)}\varphi\nabla^C\varphi+2G_{AB}(\nabla\varphi)^2+2g_{AB}R^{CD}\nabla_B\varphi\nabla_C\varphi-2R_{ACBD}\nabla^C\varphi\nabla^D\varphi\right] \vphantom{\dfrac12}
		\\
		&\quad-\dfrac{1}{2\kappa_D^2}G_{AB}-g(\varphi)\left[\dfrac{1}{2k!}H_{A_1...A_k}H^{A_1...A_k}g_{AB}-\dfrac{1}{(k-1)!}H_{A_1...A_{k-1}A}H^{A_1...A_{k-1}}_{~~~~~~~~~B}\right]
		\\
		&\quad-\dfrac12V(\varphi)g_{AB},
	\end{split}
	\\
	0&=\Box\varphi+f'(\varphi)\mathcal{G}-V'(\varphi)-\dfrac{g'(\varphi)}{k!}H_{A_1...A_k}H^{A_1...A_k},
	\label{eq:scalD}
	\\
	0&=\nabla_B\left[g(\varphi)H^{A_1...A_{k-1}B}\right].
	\label{eq:topform}
\end{align}

==> Bibliography/bib.tex <==
\begin{thebibliography}{99}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% MY PAPERS %%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cite{1912.04905}
\bibitem{1912.04905}
L.~Bordin, F.~Cunillera, A.~Leh\'ebel and A.~Padilla,
%``A natural theory of dark energy,''
Phys. Rev. D \textbf{101} (2020), 085012
doi:10.1103/PhysRevD.101.085012
[arXiv:1912.04905 [hep-th]].
%6 citations counted in INSPIRE as of 05 Oct 2021

%\cite{2105.03426}
\bibitem{2105.03426}
F.~Cunillera and A.~Padilla,
%``A stringy perspective on the coincidence problem,''
[arXiv:2105.03426 [hep-th]].
%0 citations counted in INSPIRE as of 05 Oct 2021

%\cite{Cicoli:2021fsd}
\bibitem{Cicoli:2021fsd}
M.~Cicoli, F.~Cunillera, A.~Padilla and F.~G.~Pedro,
%``Quintessence and the Swampland: The parametrically controlled regime of moduli space,''
[arXiv:2112.10779 [hep-th]].
%0 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Cunillera:2021fbc}
\bibitem{Cunillera:2021fbc}
F.~Cunillera, W.~T.~Emond, A.~Leh\'ebel and A.~Padilla,
%``Quadratic curvature corrections to stringy effective actions and the absence of de Sitter vacua,''
[arXiv:2112.05771 [hep-th]].
%1 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Cicoli:2021skd}
\bibitem{Cicoli:2021skd}
M.~Cicoli, F.~Cunillera, A.~Padilla and F.~G.~Pedro,
%``Quintessence and the Swampland: The numerically controlled regime of moduli space,''
[arXiv:2112.10783 [hep-th]].
%0 citations counted in INSPIRE as of 06 Jan 2022


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF MY PAPERS %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% INTRO %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cite{Polchinski:1998rq}
\bibitem{Polchinski:1998rq}
J.~Polchinski,
%``String theory. Vol. 1: An introduction to the bosonic string,''
doi:10.1017/CBO9780511816079
%488 citations counted in INSPIRE as of 06 Jan 2022

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF INTRO %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CHAPTER 1 %%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cite{Yau:1977ms}
\bibitem{Yau:1977ms}
S.~T.~Yau,
%``Calabi's Conjecture and some new results in algebraic geometry,''
Proc. Nat. Acad. Sci. \textbf{74} (1977), 1798-1799
doi:10.1073/pnas.74.5.1798
%270 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Grimm:2004uq}
\bibitem{Grimm:2004uq}
T.~W.~Grimm and J.~Louis,
%``The Effective action of N = 1 Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{699} (2004), 387-426
doi:10.1016/j.nuclphysb.2004.08.005
[arXiv:hep-th/0403067 [hep-th]].
%366 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Grimm:2004ua}
\bibitem{Grimm:2004ua}
T.~W.~Grimm and J.~Louis,
%``The Effective action of type IIA Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{718} (2005), 153-202
doi:10.1016/j.nuclphysb.2005.04.007
[arXiv:hep-th/0412277 [hep-th]].
%265 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Grimm:2005fa}
\bibitem{Grimm:2005fa}
T.~W.~Grimm,
%``The Effective action of type II Calabi-Yau orientifolds,''
Fortsch. Phys. \textbf{53} (2005), 1179-1271
doi:10.1002/prop.200510253
[arXiv:hep-th/0507153 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Polchinski:1998rr}
\bibitem{Polchinski:1998rr}
J.~Polchinski,
%``String theory. Vol. 2: Superstring theory and beyond,''
doi:10.1017/CBO9780511618123
%438 citations counted in INSPIRE as of 05 Nov 2021

%\cite{hep-th/9908007}
\bibitem{hep-th/9908007}
R.~Bohm, H.~Gunther, C.~Herrmann and J.~Louis,
%``Compactification of type IIB string theory on Calabi-Yau threefolds,''
Nucl. Phys. B \textbf{569} (2000), 229-246
doi:10.1016/S0550-3213(99)00796-8
[arXiv:hep-th/9908007 [hep-th]].
%78 citations counted in INSPIRE as of 15 Oct 2021

%\cite{hep-th/0507153}
\bibitem{hep-th/0507153}
T.~W.~Grimm,
%``The Effective action of type II Calabi-Yau orientifolds,''
Fortsch. Phys. \textbf{53} (2005), 1179-1271
doi:10.1002/prop.200510253
[arXiv:hep-th/0507153 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Ferrara:1988ff}
\bibitem{Ferrara:1988ff}
S.~Ferrara and S.~Sabharwal,
%``Dimensional Reduction of Type {II} Superstrings,''
Class. Quant. Grav. \textbf{6} (1989), L77
doi:10.1088/0264-9381/6/4/002
%71 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Ferrara:1989ik}
\bibitem{Ferrara:1989ik}
S.~Ferrara and S.~Sabharwal,
%``Quaternionic Manifolds for Type II Superstring Vacua of Calabi-Yau Spaces,''
Nucl. Phys. B \textbf{332} (1990), 317-332
doi:10.1016/0550-3213(90)90097-W
%327 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9804208}
\bibitem{hep-th/9804208}
A.~Dabholkar,
%``Lectures on orientifolds and duality,''
[arXiv:hep-th/9804208 [hep-th]].
%110 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/0103068}
\bibitem{hep-th/0103068}
M.~Haack and J.~Louis,
%``M theory compactified on Calabi-Yau fourfolds with background flux,''
Phys. Lett. B \textbf{507} (2001), 296-304
doi:10.1016/S0370-2693(01)00464-6
[arXiv:hep-th/0103068 [hep-th]].
%145 citations counted in INSPIRE as of 13 Oct 2021

%\cite{hep-th/0107044}
\bibitem{hep-th/0107044}
K.~Becker and M.~Becker,
%``Supersymmetry breaking, M theory and fluxes,''
JHEP \textbf{07} (2001), 038
doi:10.1088/1126-6708/2001/07/038
[arXiv:hep-th/0107044 [hep-th]].
%131 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0907.0665}
\bibitem{0907.0665}
M.~Cicoli,
%``String Loop Moduli Stabilisation and Cosmology in IIB Flux Compactifications,''
Fortsch. Phys. \textbf{58} (2010), 115-338
doi:10.1002/prop.200900096
[arXiv:0907.0665 [hep-th]].
%18 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Wess:1992cp}
\bibitem{Wess:1992cp}
J.~Wess and J.~Bagger,
%``Supersymmetry and supergravity,''
%429 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Gates:1983nr}
\bibitem{Gates:1983nr}
S.~J.~Gates, M.~T.~Grisaru, M.~Rocek and W.~Siegel,
%``Superspace Or One Thousand and One Lessons in Supersymmetry,''
Front. Phys. \textbf{58} (1983), 1-548
[arXiv:hep-th/0108200 [hep-th]].
%815 citations counted in INSPIRE as of 09 Nov 2021

%\cite{hep-th/0105097}
\bibitem{hep-th/0105097}
S.~B.~Giddings, S.~Kachru and J.~Polchinski,
%``Hierarchies from fluxes in string compactifications,''
Phys. Rev. D \textbf{66} (2002), 106006
doi:10.1103/PhysRevD.66.106006
[arXiv:hep-th/0105097 [hep-th]].
%1942 citations counted in INSPIRE as of 03 Nov 2021

%\cite{hep-th/9910053}
\bibitem{hep-th/9910053}
R.~C.~Myers,
%``Dielectric branes,''
JHEP \textbf{12} (1999), 022
doi:10.1088/1126-6708/1999/12/022
[arXiv:hep-th/9910053 [hep-th]].
%1365 citations counted in INSPIRE as of 08 Nov 2021

%\cite{hep-th/0007018}
\bibitem{hep-th/0007018}
J.~M.~Maldacena and C.~Nunez,
%``Supergravity description of field theories on curved manifolds and a no go theorem,''
Int. J. Mod. Phys. A \textbf{16} (2001), 822-855
doi:10.1142/S0217751X01003937
[arXiv:hep-th/0007018 [hep-th]].
%1017 citations counted in INSPIRE as of 01 Nov 2021

%\cite{hep-th/9602052}
\bibitem{hep-th/9602052}
J.~Polchinski, S.~Chaudhuri and C.~V.~Johnson,
%``Notes on D-branes,''
[arXiv:hep-th/9602052 [hep-th]].
%598 citations counted in INSPIRE as of 25 Oct 2021

%\cite{Johnson:2003glb}
\bibitem{Johnson:2003glb}
C.~V.~Johnson,
%``D-branes,''
doi:10.1017/CBO9780511606540
%50 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Becker:2006dvp}
\bibitem{Becker:2006dvp}
K.~Becker, M.~Becker and J.~H.~Schwarz,
%``String theory and M-theory: A modern introduction,''
%150 citations counted in INSPIRE as of 29 Oct 2021

%\cite{Green:1987mn}
\bibitem{Green:1987mn}
M.~B.~Green, J.~H.~Schwarz and E.~Witten,
%``SUPERSTRING THEORY. VOL. 2: LOOP AMPLITUDES, ANOMALIES AND PHENOMENOLOGY,''
%249 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0007191}
\bibitem{hep-th/0007191}
I.~R.~Klebanov and M.~J.~Strassler,
%``Supergravity and a confining gauge theory: Duality cascades and chi SB resolution of naked singularities,''
JHEP \textbf{08} (2000), 052
doi:10.1088/1126-6708/2000/08/052
[arXiv:hep-th/0007191 [hep-th]].
%1781 citations counted in INSPIRE as of 26 Oct 2021

%\cite{0708.2865}
\bibitem{0708.2865}
C.~P.~Burgess,
%``Lectures on Cosmic Inflation and its Potential Stringy Realizations,''
PoS P \textbf{2GC} (2006), 008
doi:10.1088/0264-9381/24/21/S04
[arXiv:0708.2865 [hep-th]].
%151 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0710.2951}
\bibitem{0710.2951}
L.~McAllister and E.~Silverstein,
%``String Cosmology: A Review,''
Gen. Rel. Grav. \textbf{40} (2008), 565-605
doi:10.1007/s10714-007-0556-6
[arXiv:0710.2951 [hep-th]].
%326 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0808.2811}
\bibitem{0808.2811}
D.~Baumann, A.~Dymarsky, S.~Kachru, I.~R.~Klebanov and L.~McAllister,
%``Holographic Systematics of D-brane Inflation,''
JHEP \textbf{03} (2009), 093
doi:10.1088/1126-6708/2009/03/093
[arXiv:0808.2811 [hep-th]].
%94 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0802.2916}
\bibitem{0802.2916}
E.~Pajer,
%``Inflation at the Tip,''
JCAP \textbf{04} (2008), 031
doi:10.1088/1475-7516/2008/04/031
[arXiv:0802.2916 [hep-th]].
%47 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0810.5001}
\bibitem{0810.5001}
A.~Avgoustidis and I.~Zavala,
%``Warped Wilson Line DBI Inflation,''
JCAP \textbf{01} (2009), 045
doi:10.1088/1475-7516/2009/01/045
[arXiv:0810.5001 [hep-th]].
%27 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9912152}
\bibitem{hep-th/9912152}
T.~R.~Taylor and C.~Vafa,
%``R R flux on Calabi-Yau and partial supersymmetry breaking,''
Phys. Lett. B \textbf{474} (2000), 130-137
doi:10.1016/S0370-2693(00)00005-8
[arXiv:hep-th/9912152 [hep-th]].
%449 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0204254}
\bibitem{hep-th/0204254}
K.~Becker, M.~Becker, M.~Haack and J.~Louis,
%``Supersymmetry breaking and alpha-prime corrections to flux induced potentials,''
JHEP \textbf{06} (2002), 060
doi:10.1088/1126-6708/2002/06/060
[arXiv:hep-th/0204254 [hep-th]].
%409 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0208123}
\bibitem{hep-th/0208123}
O.~DeWolfe and S.~B.~Giddings,
%``Scales and hierarchies in warped compactifications and brane worlds,''
Phys. Rev. D \textbf{67} (2003), 066008
doi:10.1103/PhysRevD.67.066008
[arXiv:hep-th/0208123 [hep-th]].
%277 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0403067}
\bibitem{hep-th/0403067}
T.~W.~Grimm and J.~Louis,
%``The Effective action of N = 1 Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{699} (2004), 387-426
doi:10.1016/j.nuclphysb.2004.08.005
[arXiv:hep-th/0403067 [hep-th]].
%366 citations counted in INSPIRE as of 09 Nov 2021

%\cite{deWit:1986mwo}
\bibitem{deWit:1986mwo}
B.~de Wit, D.~J.~Smit and N.~D.~Hari Dass,
%``Residual Supersymmetry of Compactified D=10 Supergravity,''
Nucl. Phys. B \textbf{283} (1987), 165
doi:10.1016/0550-3213(87)90267-7
%266 citations counted in INSPIRE as of 01 Nov 2021

%\cite{hep-th/9510017}
\bibitem{hep-th/9510017}
J.~Polchinski,
%``Dirichlet Branes and Ramond-Ramond charges,''
Phys. Rev. Lett. \textbf{75} (1995), 4724-4727
doi:10.1103/PhysRevLett.75.4724
[arXiv:hep-th/9510017 [hep-th]].
%2785 citations counted in INSPIRE as of 09 Nov 2021

%\cite{0803.1194}
\bibitem{0803.1194}
F.~Denef,
%``Les Houches Lectures on Constructing String Vacua,''
Les Houches \textbf{87} (2008), 483-610
[arXiv:0803.1194 [hep-th]].
%428 citations counted in INSPIRE as of 08 Nov 2021

%\cite{Cicoli:2007xp}
\bibitem{Cicoli:2007xp}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``Systematics of String Loop Corrections in Type IIB Calabi-Yau Flux Compactifications,''
JHEP \textbf{01} (2008), 052
doi:10.1088/1126-6708/2008/01/052
[arXiv:0708.1873 [hep-th]].
%174 citations counted in INSPIRE as of 14 Oct 2021

%\cite{Cicoli:2008va}
\bibitem{Cicoli:2008va}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``General Analysis of LARGE Volume Scenarios with String Loop Moduli Stabilisation,''
JHEP \textbf{10} (2008), 105
doi:10.1088/1126-6708/2008/10/105
[arXiv:0805.1029 [hep-th]].
%163 citations counted in INSPIRE as of 02 Nov 2021

%\cite{Kachru:2019dvo}
\bibitem{Kachru:2019dvo}
S.~Kachru, M.~Kim, L.~Mcallister and M.~Zimet,
%``de Sitter Vacua from Ten Dimensions,''
[arXiv:1908.04788 [hep-th]].
%39 citations counted in INSPIRE as of 08 Nov 2021

%\cite{AbdusSalam:2020ywo}
\bibitem{AbdusSalam:2020ywo}
S.~AbdusSalam, S.~Abel, M.~Cicoli, F.~Quevedo and P.~Shukla,
%``A systematic approach to K\"ahler moduli stabilisation,''
JHEP \textbf{08} (2020) no.08, 047
doi:10.1007/JHEP08(2020)047
[arXiv:2005.11329 [hep-th]].
%15 citations counted in INSPIRE as of 28 Oct 2021

%\cite{Cicoli:2021rub}
\bibitem{Cicoli:2021rub}
M.~Cicoli, F.~Quevedo, R.~Savelli, A.~Schachner and R.~Valandro,
%``Systematics of the $\alpha'$ Expansion in F-Theory,''
JHEP \textbf{2021} (2021), 99
doi:10.1007/JHEP08(2021)099
[arXiv:2106.04592 [hep-th]].
%2 citations counted in INSPIRE as of 04 Nov 2021

%\cite{Palti:2019pca}
\bibitem{Palti:2019pca}
E.~Palti,
%``The Swampland: Introduction and Review,''
Fortsch. Phys. \textbf{67} (2019) no.6, 1900037
doi:10.1002/prop.201900037
[arXiv:1903.06239 [hep-th]].
%441 citations counted in INSPIRE as of 09 Nov 2021

%\cite{hep-th/0509212}
\bibitem{hep-th/0509212}
C.~Vafa,
%``The String landscape and the swampland,''
[arXiv:hep-th/0509212 [hep-th]].
%626 citations counted in INSPIRE as of 09 Nov 2021

%\cite{hep-th/0605264}
\bibitem{hep-th/0605264}
H.~Ooguri and C.~Vafa,
%``On the Geometry of the String Landscape and the Swampland,''
Nucl. Phys. B \textbf{766} (2007), 21-33
doi:10.1016/j.nuclphysb.2006.10.033
[arXiv:hep-th/0605264 [hep-th]].
%593 citations counted in INSPIRE as of 03 Nov 2021

%\cite{1610.00010}
\bibitem{1610.00010}
D.~Klaewer and E.~Palti,
%``Super-Planckian Spatial Field Variations and Quantum Gravity,''
JHEP \textbf{01} (2017), 088
doi:10.1007/JHEP01(2017)088
[arXiv:1610.00010 [hep-th]].
%176 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1602.06517}
\bibitem{1602.06517}
F.~Baume and E.~Palti,
%``Backreacted Axion Field Ranges in String Theory,''
JHEP \textbf{08} (2016), 043
doi:10.1007/JHEP08(2016)043
[arXiv:1602.06517 [hep-th]].
%106 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1903.06239}
\bibitem{1903.06239}
E.~Palti,
%``The Swampland: Introduction and Review,''
Fortsch. Phys. \textbf{67} (2019) no.6, 1900037
doi:10.1002/prop.201900037
[arXiv:1903.06239 [hep-th]].
%441 citations counted in INSPIRE as of 09 Nov 2021

%\cite{1611.00394}
\bibitem{1611.00394}
I.~Valenzuela,
%``Backreaction Issues in Axion Monodromy and Minkowski 4-forms,''
JHEP \textbf{06} (2017), 098
doi:10.1007/JHEP06(2017)098
[arXiv:1611.00394 [hep-th]].
%75 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1611.07084}
\bibitem{1611.07084}
S.~Bielleman, L.~E.~Ibanez, F.~G.~Pedro, I.~Valenzuela and C.~Wieck,
%``Higgs-otic Inflation and Moduli Stabilization,''
JHEP \textbf{02} (2017), 073
doi:10.1007/JHEP02(2017)073
[arXiv:1611.07084 [hep-th]].
%28 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1703.05776}
\bibitem{1703.05776}
R.~Blumenhagen, I.~Valenzuela and F.~Wolf,
%``The Swampland Conjecture and F-term Axion Monodromy Inflation,''
JHEP \textbf{07} (2017), 145
doi:10.1007/JHEP07(2017)145
[arXiv:1703.05776 [hep-th]].
%96 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1708.06761}
\bibitem{1708.06761}
A.~Hebecker, P.~Henkenjohann and L.~T.~Witkowski,
%``Flat Monodromies and a Moduli Space Size Conjecture,''
JHEP \textbf{12} (2017), 033
doi:10.1007/JHEP12(2017)033
[arXiv:1708.06761 [hep-th]].
%54 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1801.05434}
\bibitem{1801.05434}
M.~Cicoli, D.~Ciupke, C.~Mayrhofer and P.~Shukla,
%``A Geometrical Upper Bound on the Inflaton Range,''
JHEP \textbf{05} (2018), 001
doi:10.1007/JHEP05(2018)001
[arXiv:1801.05434 [hep-th]].
%57 citations counted in INSPIRE as of 13 Oct 2021

%\cite{1904.05379}
\bibitem{1904.05379}
A.~Font, A.~Herr\'aez and L.~E.~Ib\'a\~nez,
%``The Swampland Distance Conjecture and Towers of Tensionless Branes,''
JHEP \textbf{08} (2019), 044
doi:10.1007/JHEP08(2019)044
[arXiv:1904.05379 [hep-th]].
%57 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1806.09718}
\bibitem{1806.09718}
P.~Agrawal, G.~Obied, P.~J.~Steinhardt and C.~Vafa,
%``On the Cosmological Implications of the String Swampland,''
Phys. Lett. B \textbf{784} (2018), 271-276
doi:10.1016/j.physletb.2018.07.040
[arXiv:1806.09718 [hep-th]].
%356 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1807.06581}
\bibitem{1807.06581}
F.~Denef, A.~Hebecker and T.~Wrase,
%``de Sitter swampland conjecture and the Higgs potential,''
Phys. Rev. D \textbf{98} (2018) no.8, 086004
doi:10.1103/PhysRevD.98.086004
[arXiv:1807.06581 [hep-th]].
%126 citations counted in INSPIRE as of 14 Oct 2021

%\cite{Conlon:2018eyr}
\bibitem{Conlon:2018eyr}
J.~P.~Conlon,
%``The de Sitter swampland conjecture and supersymmetric AdS vacua,''
Int. J. Mod. Phys. A \textbf{33} (2018) no.29, 1850178
%doi:10.1142/S0217751X18501786
[arXiv:1808.05040 [hep-th]].
%67 citations counted in INSPIRE as of 10 Dec 2021

%\cite{1807.05193}
\bibitem{1807.05193}
S.~K.~Garg and C.~Krishnan,
%``Bounds on Slow Roll and the de Sitter Swampland,''
JHEP \textbf{11} (2019), 075
doi:10.1007/JHEP11(2019)075
[arXiv:1807.05193 [hep-th]].
%390 citations counted in INSPIRE as of 09 Nov 2021

%\cite{1810.05506}
\bibitem{1810.05506}
H.~Ooguri, E.~Palti, G.~Shiu and C.~Vafa,
%``Distance and de Sitter Conjectures on the Swampland,''
Phys. Lett. B \textbf{788} (2019), 180-184
doi:10.1016/j.physletb.2018.11.018
[arXiv:1810.05506 [hep-th]].
%416 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Dine:1985he}
\bibitem{Dine:1985he}
M.~Dine and N.~Seiberg,
%``Is the Superstring Weakly Coupled?,''
Phys. Lett. B \textbf{162} (1985), 299-302
doi:10.1016/0370-2693(85)90927-X
%357 citations counted in INSPIRE as of 15 Oct 2021

%\cite{2008.12399}
\bibitem{2008.12399}
M.~Dine, J.~A.~P.~Law-Smith, S.~Sun, D.~Wood and Y.~Yu,
%``Obstacles to Constructing de Sitter Space in String Theory,''
JHEP \textbf{02} (2021), 050
doi:10.1007/JHEP02(2021)050
[arXiv:2008.12399 [hep-th]].
%7 citations counted in INSPIRE as of 15 Oct 2021

%%%%%%%%%%%%%%%%%%%% ROBERT WEBSITE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{robert}
R.~Smith,
online: https://tracingcurves.wordpress.com, %/2019/10/20/notes-on-the-swampland-4-the-distance-conjecture-for-arbitrary-calabi-yau-manifolds-the-emergence-proposal-and-the-de-sitter-conjecture/
taken: 18-10-2021.
%%%%%%%%%%%%%%%%%%%% ROBERT WEBSITE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF CHAPTER 1 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% NO CHAPTER 2 -- MOVED TO A SECTION IN CHAPTER 1 %%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CHAPTER 3 %%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\cite{Gildener:1976ai}
\bibitem{Gildener:1976ai}
E.~Gildener,
%``Gauge Symmetry Hierarchies,''
Phys. Rev. D \textbf{14} (1976), 1667
doi:10.1103/PhysRevD.14.1667
%781 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Weinberg:1978ym}
\bibitem{Weinberg:1978ym}
S.~Weinberg,
%``Gauge Hierarchies,''
Phys. Lett. B \textbf{82} (1979), 387-391
doi:10.1016/0370-2693(79)90248-X
%350 citations counted in INSPIRE as of 29 Oct 2021

%\cite{Peskin:1995ev}
\bibitem{Peskin:1995ev}
M.~E.~Peskin and D.~V.~Schroeder,
%``An Introduction to quantum field theory,''
%1470 citations counted in INSPIRE as of 08 Nov 2021

%\cite{Dimopoulos:1981zb}
\bibitem{Dimopoulos:1981zb}
S.~Dimopoulos and H.~Georgi,
%``Softly Broken Supersymmetry and SU(5),''
Nucl. Phys. B \textbf{193} (1981), 150-162
doi:10.1016/0550-3213(81)90522-8
%3031 citations counted in INSPIRE as of 03 Nov 2021

%\cite{tHooft:1979rat}
\bibitem{tHooft:1979rat}
G.~'t Hooft,
%``Naturalness, chiral symmetry, and spontaneous chiral symmetry breaking,''
NATO Sci. Ser. B \textbf{59} (1980), 135-157
doi:10.1007/978-1-4684-7571-5\_9
%721 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Susskind:1978ms}
\bibitem{Susskind:1978ms}
L.~Susskind,
%``Dynamics of Spontaneous Symmetry Breaking in the Weinberg-Salam Theory,''
Phys. Rev. D \textbf{20} (1979), 2619-2625
doi:10.1103/PhysRevD.20.2619
%2864 citations counted in INSPIRE as of 05 Nov 2021

%\cite{Dimopoulos:1979za}
\bibitem{Dimopoulos:1979za}
S.~Dimopoulos, L.~Susskind and S.~Raby,
%``Technicolour,''
AIP Conf. Proc. \textbf{59} (1980), 407-452
doi:10.1063/1.32174
%0 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Farhi:1979zx}
\bibitem{Farhi:1979zx}
E.~Farhi and L.~Susskind,
%``A Technicolored G.U.T.,''
Phys. Rev. D \textbf{20} (1979), 3404-3411
doi:10.1103/PhysRevD.20.3404
%331 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0801.2562}
\bibitem{0801.2562}
G.~F.~Giudice,
%``Naturally Speaking: The Naturalness Criterion and Physics at the LHC,''
doi:10.1142/9789812779762\_0010
[arXiv:0801.2562 [hep-ph]].
%203 citations counted in INSPIRE as of 02 Nov 2021

%\cite{Weinberg:1988cp}
\bibitem{Weinberg:1988cp}
S.~Weinberg,
%``The Cosmological Constant Problem,''
Rev. Mod. Phys. \textbf{61} (1989), 1-23
doi:10.1103/RevModPhys.61.1
%5119 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1309.4133}
\bibitem{1309.4133}
C.~P.~Burgess,
%``The Cosmological Constant Problem: Why it's hard to get Dark Energy from Micro-physics,''
doi:10.1093/acprof:oso/9780198728856.003.0004
[arXiv:1309.4133 [hep-th]].
%144 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1502.05296}
\bibitem{1502.05296}
A.~Padilla,
%``Lectures on the Cosmological Constant Problem,''
[arXiv:1502.05296 [hep-th]].
%180 citations counted in INSPIRE as of 22 Oct 2021

%\cite{Weinberg:1987dv}
\bibitem{Weinberg:1987dv}
S.~Weinberg,
%``Anthropic Bound on the Cosmological Constant,''
Phys. Rev. Lett. \textbf{59} (1987), 2607
doi:10.1103/PhysRevLett.59.2607
%965 citations counted in INSPIRE as of 03 Nov 2021

%\cite{Barrow:1986nmg}
\bibitem{Barrow:1986nmg}
J.~D.~Barrow and F.~J.~Tipler,
%``The Anthropic Cosmological Principle,''
%14 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Weinberg:1996xe}
\bibitem{Weinberg:1996xe}
S.~Weinberg,
%``Theories of the cosmological constant,''
[arXiv:astro-ph/9610044 [astro-ph]].
%83 citations counted in INSPIRE as of 11 Oct 2021

%\cite{astro-ph/9701099}
\bibitem{astro-ph/9701099}
H.~Martel, P.~R.~Shapiro and S.~Weinberg,
%``Likely values of the cosmological constant,''
Astrophys. J. \textbf{492} (1998), 29
doi:10.1086/305016
[arXiv:astro-ph/9701099 [astro-ph]].
%252 citations counted in INSPIRE as of 11 Oct 2021

%\cite{astro-ph/9908115}
\bibitem{astro-ph/9908115}
J.~Garriga and A.~Vilenkin,
%``On likely values of the cosmological constant,''
Phys. Rev. D \textbf{61} (2000), 083502
doi:10.1103/PhysRevD.61.083502
[arXiv:astro-ph/9908115 [astro-ph]].
%126 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2013zca}
\bibitem{Kaloper:2013zca}
N.~Kaloper and A.~Padilla,
%``Sequestering the Standard Model Vacuum Energy,''
Phys. Rev. Lett. \textbf{112} (2014) no.9, 091304
doi:10.1103/PhysRevLett.112.091304
[arXiv:1309.6562 [hep-th]].
%128 citations counted in INSPIRE as of 20 Oct 2021

%\cite{Kaloper:2014dqa}
\bibitem{Kaloper:2014dqa}
N.~Kaloper and A.~Padilla,
%``Vacuum Energy Sequestering: The Framework and Its Cosmological Consequences,''
Phys. Rev. D \textbf{90} (2014) no.8, 084023
doi:10.1103/PhysRevD.90.084023
[arXiv:1406.0711 [hep-th]].
%85 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2014fca}
\bibitem{Kaloper:2014fca}
N.~Kaloper and A.~Padilla,
%``Sequestration of Vacuum Energy and the End of the Universe,''
Phys. Rev. Lett. \textbf{114} (2015) no.10, 101302
doi:10.1103/PhysRevLett.114.101302
[arXiv:1409.7073 [hep-th]].
%40 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2015jra}
\bibitem{Kaloper:2015jra}
N.~Kaloper, A.~Padilla, D.~Stefanyszyn and G.~Zahariade,
%``Manifestly Local Theory of Vacuum Energy Sequestering,''
Phys. Rev. Lett. \textbf{116} (2016) no.5, 051302
doi:10.1103/PhysRevLett.116.051302
[arXiv:1505.01492 [hep-th]].
%66 citations counted in INSPIRE as of 13 Oct 2021

%\cite{Kaloper:2016yfa}
\bibitem{Kaloper:2016yfa}
N.~Kaloper, A.~Padilla and D.~Stefanyszyn,
%``Sequestering effects on and of vacuum decay,''
Phys. Rev. D \textbf{94} (2016) no.2, 025022
doi:10.1103/PhysRevD.94.025022
[arXiv:1604.04000 [hep-th]].
%17 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2016jsd}
\bibitem{Kaloper:2016jsd}
N.~Kaloper and A.~Padilla,
%``Vacuum Energy Sequestering and Graviton Loops,''
Phys. Rev. Lett. \textbf{118} (2017) no.6, 061303
doi:10.1103/PhysRevLett.118.061303
[arXiv:1606.04958 [hep-th]].
%29 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0209226}
\bibitem{hep-th/0209226}
A.~Adams, J.~McGreevy and E.~Silverstein,
%``Decapitating tadpoles,''
[arXiv:hep-th/0209226 [hep-th]].
%18 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1706.04778}
\bibitem{1706.04778}
F.~Niedermann and A.~Padilla,
%``Gravitational Mechanisms to Self-Tune the Cosmological Constant: Obstructions and Ways Forward,''
Phys. Rev. Lett. \textbf{119} (2017) no.25, 251306
doi:10.1103/PhysRevLett.119.251306
[arXiv:1706.04778 [hep-th]].
%13 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0004134}
\bibitem{hep-th/0004134}
R.~Bousso and J.~Polchinski,
%``Quantization of four form fluxes and dynamical neutralization of the cosmological constant,''
JHEP \textbf{06} (2000), 006
doi:10.1088/1126-6708/2000/06/006
[arXiv:hep-th/0004134 [hep-th]].
%1208 citations counted in INSPIRE as of 22 Oct 2021

%\cite{Ashok:2003gk}
\bibitem{Ashok:2003gk}
S.~Ashok and M.~R.~Douglas,
%``Counting flux vacua,''
JHEP \textbf{01} (2004), 060
doi:10.1088/1126-6708/2004/01/060
[arXiv:hep-th/0307049 [hep-th]].
%382 citations counted in INSPIRE as of 02 Nov 2021

%\cite{Denef:2004ze}
\bibitem{Denef:2004ze}
F.~Denef and M.~R.~Douglas,
%``Distributions of flux vacua,''
JHEP \textbf{05} (2004), 072
doi:10.1088/1126-6708/2004/05/072
[arXiv:hep-th/0404116 [hep-th]].
%505 citations counted in INSPIRE as of 02 Nov 2021

%\cite{Demirtas:2021ote}
\bibitem{Demirtas:2021ote}
M.~Demirtas, M.~Kim, L.~McAllister, J.~Moritz and A.~Rios-Tascon,
%``A Cosmological Constant That is Too Small,''
[arXiv:2107.09065 [hep-th]].
%6 citations counted in INSPIRE as of 13 Oct 2021

%\cite{Demirtas:2021nlu}
\bibitem{Demirtas:2021nlu}
M.~Demirtas, M.~Kim, L.~McAllister, J.~Moritz and A.~Rios-Tascon,
%``Small Cosmological Constants in String Theory,''
[arXiv:2107.09064 [hep-th]].
%8 citations counted in INSPIRE as of 14 Oct 2021

%\cite{astro-ph/9807002}
\bibitem{astro-ph/9807002}
I.~Zlatev, L.~M.~Wang and P.~J.~Steinhardt,
%``Quintessence, cosmic coincidence, and the cosmological constant,''
Phys. Rev. Lett. \textbf{82} (1999), 896-899
doi:10.1103/PhysRevLett.82.896
[arXiv:astro-ph/9807002 [astro-ph]].
%2178 citations counted in INSPIRE as of 02 Nov 2021

%\cite{arXiv:1807.06209}
\bibitem{arXiv:1807.06209}
N.~Aghanim \textit{et al.} [Planck],
%``Planck 2018 results. VI. Cosmological parameters,''
Astron. Astrophys. \textbf{641} (2020), A6
[erratum: Astron. Astrophys. \textbf{652} (2021), C4]
doi:10.1051/0004-6361/201833910
[arXiv:1807.06209 [astro-ph.CO]].
%6245 citations counted in INSPIRE as of 09 Nov 2021

%\cite{arXiv:1410.2509}
\bibitem{arXiv:1410.2509}
H.~E.~S.~Velten, R.~F.~vom Marttens and W.~Zimdahl,
%``Aspects of the cosmological \textquotedblleft{}coincidence problem\textquotedblright{},''
Eur. Phys. J. C \textbf{74} (2014) no.11, 3160
doi:10.1140/epjc/s10052-014-3160-4
[arXiv:1410.2509 [astro-ph.CO]].
%109 citations counted in INSPIRE as of 12 Oct 2021

%\cite{arXiv:astro-ph/9701131}
\bibitem{arXiv:astro-ph/9701131}
F.~C.~Adams and G.~Laughlin,
%``A Dying universe: The Long term fate and evolution of astrophysical objects,''
Rev. Mod. Phys. \textbf{69} (1997), 337-372
doi:10.1103/RevModPhys.69.337
[arXiv:astro-ph/9701131 [astro-ph]].
%96 citations counted in INSPIRE as of 11 Oct 2021

%\cite{astro-ph/9906210}
\bibitem{astro-ph/9906210}
J.~Garriga, M.~Livio and A.~Vilenkin,
%``The Cosmological constant and the time of its dominance,''
Phys. Rev. D \textbf{61} (2000), 023503
doi:10.1103/PhysRevD.61.023503
[arXiv:astro-ph/9906210 [astro-ph]].
%120 citations counted in INSPIRE as of 11 Oct 2021

%\cite{astro-ph/0005265}
\bibitem{astro-ph/0005265}
S.~Weinberg,
%``The Cosmological constant problems,''
[arXiv:astro-ph/0005265 [astro-ph]].
%429 citations counted in INSPIRE as of 08 Nov 2021

%\cite{astro-ph/9907168}
\bibitem{astro-ph/9907168}
S.~A.~Bludman,
%``Vacuum energy: If not now, then when?,''
Nucl. Phys. A \textbf{663} (2000), 865-868
doi:10.1016/S0375-9474(99)00733-2
[arXiv:astro-ph/9907168 [astro-ph]].
%28 citations counted in INSPIRE as of 11 Oct 2021

%\cite{arXiv:1103.2401}
\bibitem{arXiv:1103.2401}
A.~Barreira and P.~P.~Avelino,
%``Anthropic versus cosmological solutions to the coincidence problem,''
Phys. Rev. D \textbf{83} (2011), 103001
doi:10.1103/PhysRevD.83.103001
[arXiv:1103.2401 [astro-ph.CO]].
%20 citations counted in INSPIRE as of 11 Oct 2021

%\cite{astro-ph/0004134}
\bibitem{astro-ph/0004134}
C.~Armendariz-Picon, V.~F.~Mukhanov and P.~J.~Steinhardt,
%``A Dynamical solution to the problem of a small cosmological constant and late time cosmic acceleration,''
Phys. Rev. Lett. \textbf{85} (2000), 4438-4441
doi:10.1103/PhysRevLett.85.4438
[arXiv:astro-ph/0004134 [astro-ph]].
%1613 citations counted in INSPIRE as of 04 Nov 2021

%\cite{arXiv:astro-ph/0006373}
\bibitem{arXiv:astro-ph/0006373}
C.~Armendariz-Picon, V.~F.~Mukhanov and P.~J.~Steinhardt,
%``Essentials of k essence,''
Phys. Rev. D \textbf{63} (2001), 103510
doi:10.1103/PhysRevD.63.103510
[arXiv:astro-ph/0006373 [astro-ph]].
%1540 citations counted in INSPIRE as of 02 Nov 2021

%\cite{arXiv:astro-ph/0304277}
\bibitem{arXiv:astro-ph/0304277}
M.~Malquarti, E.~J.~Copeland and A.~R.~Liddle,
%``K-essence and the coincidence problem,''
Phys. Rev. D \textbf{68} (2003), 023512
doi:10.1103/PhysRevD.68.023512
[arXiv:astro-ph/0304277 [astro-ph]].
%119 citations counted in INSPIRE as of 11 Oct 2021

%\cite{astro-ph/0410508}
\bibitem{astro-ph/0410508}
R.~J.~Scherrer,
%``Phantom dark energy, cosmic doomsday, and the coincidence problem,''
Phys. Rev. D \textbf{71} (2005), 063519
doi:10.1103/PhysRevD.71.063519
[arXiv:astro-ph/0410508 [astro-ph]].
%78 citations counted in INSPIRE as of 11 Oct 2021

%\cite{arXiv:astro-ph/0411033}
\bibitem{arXiv:astro-ph/0411033}
P.~P.~Avelino,
%``The Coincidence problem in linear dark energy models,''
Phys. Lett. B \textbf{611} (2005), 15-20
doi:10.1016/j.physletb.2005.02.037
[arXiv:astro-ph/0411033 [astro-ph]].
%33 citations counted in INSPIRE as of 11 Oct 2021

%\cite{DAmico:2017ngr}
\bibitem{DAmico:2017ngr}
G.~D'Amico, N.~Kaloper, A.~Padilla, D.~Stefanyszyn, A.~Westphal and G.~Zahariade,
%``An \'etude on global vacuum energy sequester,''
JHEP \textbf{09} (2017), 074
doi:10.1007/JHEP09(2017)074
[arXiv:1705.08950 [hep-th]].
%18 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Niedermann:2017cel}
\bibitem{Niedermann:2017cel}
F.~Niedermann and A.~Padilla,
%``Gravitational Mechanisms to Self-Tune the Cosmological Constant: Obstructions and Ways Forward,''
Phys. Rev. Lett. \textbf{119} (2017) no.25, 251306
doi:10.1103/PhysRevLett.119.251306
[arXiv:1706.04778 [hep-th]].
%13 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Coltman:2019mql}
\bibitem{Coltman:2019mql}
B.~Coltman, Y.~Li and A.~Padilla,
%``Cosmological consequences of Omnia Sequestra,''
JCAP \textbf{06} (2019), 017
doi:10.1088/1475-7516/2019/06/017
[arXiv:1903.02829 [hep-th]].
%4 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Iben:1983ts}
\bibitem{Iben:1983ts}
I.~Iben and A.~Renzini,
%``Asymptotic giant branch evolution and beyond,''
Ann. Rev. Astron. Astrophys. \textbf{21} (1983), 271-342
doi:10.1146/annurev.aa.21.090183.001415
%358 citations counted in INSPIRE as of 03 Nov 2021

%\cite{Livio:1998mq}
\bibitem{Livio:1998mq}
M.~Livio,
%``How rare are extraterrestrial civilizations and when did they emerge?,''
Astrophys. J. \textbf{511} (1999), 429
doi:10.1086/306668
[arXiv:astro-ph/9808237 [astro-ph]].
%22 citations counted in INSPIRE as of 11 Oct 2021

%\cite{astro-ph/0006373}
\bibitem{astro-ph/0006373}
C.~Armendariz-Picon, V.~F.~Mukhanov and P.~J.~Steinhardt,
%``Essentials of k essence,''
Phys. Rev. D \textbf{63} (2001), 103510
doi:10.1103/PhysRevD.63.103510
[arXiv:astro-ph/0006373 [astro-ph]].
%1540 citations counted in INSPIRE as of 02 Nov 2021

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% END CHAPTER 3 %%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CHAPTER 4 %%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cite{1511.00132}
\bibitem{1511.00132}
K.~Choi and S.~H.~Im,
%``Realizing the relaxion from multiple axions and its UV completion with high scale supersymmetry,''
JHEP \textbf{01} (2016), 149
doi:10.1007/JHEP01(2016)149
[arXiv:1511.00132 [hep-ph]].
%213 citations counted in INSPIRE as of 05 Nov 2021

%\cite{1511.01827}
\bibitem{1511.01827}
D.~E.~Kaplan and R.~Rattazzi,
%``Large field excursions and approximate discrete symmetries from a clockwork axion,''
Phys. Rev. D \textbf{93} (2016) no.8, 085007
doi:10.1103/PhysRevD.93.085007
[arXiv:1511.01827 [hep-ph]].
%238 citations counted in INSPIRE as of 05 Nov 2021

%\cite{hep-th/0410286}
\bibitem{hep-th/0410286}
G.~Dvali,
%``Large hierarchies from attractor vacua,''
Phys. Rev. D \textbf{74} (2006), 025018
doi:10.1103/PhysRevD.74.025018
[arXiv:hep-th/0410286 [hep-th]].
%92 citations counted in INSPIRE as of 12 Oct 2021

%\cite{hep-th/0507215}
\bibitem{hep-th/0507215}
G.~Dvali,
%``Three-form gauging of axion symmetries and gravity,''
[arXiv:hep-th/0507215 [hep-th]].
%123 citations counted in INSPIRE as of 02 Nov 2021

%\cite{0811.1989}
\bibitem{0811.1989}
N.~Kaloper and L.~Sorbo,
%``A Natural Framework for Chaotic Inflation,''
Phys. Rev. Lett. \textbf{102} (2009), 121301
doi:10.1103/PhysRevLett.102.121301
[arXiv:0811.1989 [hep-th]].
%318 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1101.0026}
\bibitem{1101.0026}
N.~Kaloper, A.~Lawrence and L.~Sorbo,
%``An Ignoble Approach to Large Field Inflation,''
JCAP \textbf{03} (2011), 023
doi:10.1088/1475-7516/2011/03/023
[arXiv:1101.0026 [hep-th]].
%268 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0303252}
\bibitem{hep-th/0303252}
T.~Banks, M.~Dine, P.~J.~Fox and E.~Gorbatov,
%``On the possibility of large axion decay constants,''
JCAP \textbf{06} (2003), 001
doi:10.1088/1475-7516/2003/06/001
[arXiv:hep-th/0303252 [hep-th]].
%337 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0409138}
\bibitem{hep-th/0409138}
S.~Ghosh,
%``Extended space duality in the noncommutative plane,''
Phys. Lett. B \textbf{601} (2004), 93-98
doi:10.1016/j.physletb.2004.09.023
[arXiv:hep-th/0409138 [hep-th]].
%5 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/0601001}
\bibitem{hep-th/0601001}
N.~Arkani-Hamed, L.~Motl, A.~Nicolis and C.~Vafa,
%``The String landscape, black holes and gravity as the weakest force,''
JHEP \textbf{06} (2007), 060
doi:10.1088/1126-6708/2007/06/060
[arXiv:hep-th/0601001 [hep-th]].
%890 citations counted in INSPIRE as of 09 Nov 2021

%\cite{1503.04783}
\bibitem{1503.04783}
J.~Brown, W.~Cottrell, G.~Shiu and P.~Soler,
%``Fencing in the Swampland: Quantum Gravity Constraints on Large Field Inflation,''
JHEP \textbf{10} (2015), 023
doi:10.1007/JHEP10(2015)023
[arXiv:1503.04783 [hep-th]].
%198 citations counted in INSPIRE as of 01 Nov 2021

%\cite{1402.2287}
\bibitem{1402.2287}
C.~Cheung and G.~N.~Remmen,
%``Naturalness and the Weak Gravity Conjecture,''
Phys. Rev. Lett. \textbf{113} (2014), 051601
doi:10.1103/PhysRevLett.113.051601
[arXiv:1402.2287 [hep-ph]].
%166 citations counted in INSPIRE as of 05 Nov 2021

%\cite{1503.00795}
\bibitem{1503.00795}
T.~Rudelius,
%``Constraints on Axion Inflation from the Weak Gravity Conjecture,''
JCAP \textbf{09} (2015), 020
doi:10.1088/1475-7516/2015/9/020
[arXiv:1503.00795 [hep-th]].
%177 citations counted in INSPIRE as of 01 Nov 2021

%\cite{1610.07962}
\bibitem{1610.07962}
G.~F.~Giudice and M.~McCullough,
%``A Clockwork Theory,''
JHEP \textbf{02} (2017), 036
doi:10.1007/JHEP02(2017)036
[arXiv:1610.07962 [hep-ph]].
%160 citations counted in INSPIRE as of 05 Nov 2021

%\cite{tHooft:1979rat}
\bibitem{tHooft:1979rat}
G.~'t Hooft,
%``Naturalness, chiral symmetry, and spontaneous chiral symmetry breaking,''
NATO Sci. Ser. B \textbf{59} (1980), 135-157
doi:10.1007/978-1-4684-7571-5\_9
%721 citations counted in INSPIRE as of 09 Nov 2021

%\cite{0803.3085}
\bibitem{0803.3085}
E.~Silverstein and A.~Westphal,
%``Monodromy in the CMB: Gravity Waves and String Inflation,''
Phys. Rev. D \textbf{78} (2008), 106003
doi:10.1103/PhysRevD.78.106003
[arXiv:0803.3085 [hep-th]].
%800 citations counted in INSPIRE as of 26 Oct 2021

%\cite{0808.0706}
\bibitem{0808.0706}
L.~McAllister, E.~Silverstein and A.~Westphal,
%``Gravity Waves and Linear Inflation from Axion Monodromy,''
Phys. Rev. D \textbf{82} (2010), 046003
doi:10.1103/PhysRevD.82.046003
[arXiv:0808.0706 [hep-th]].
%722 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1611.00394}
\bibitem{1611.00394}
I.~Valenzuela,
%``Backreaction Issues in Axion Monodromy and Minkowski 4-forms,''
JHEP \textbf{06} (2017), 098
doi:10.1007/JHEP06(2017)098
[arXiv:1611.00394 [hep-th]].
%75 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1607.06105}
\bibitem{1607.06105}
N.~Kaloper and A.~Lawrence,
%``London equation for monodromy inflation,''
Phys. Rev. D \textbf{95} (2017) no.6, 063526
doi:10.1103/PhysRevD.95.063526
[arXiv:1607.06105 [hep-th]].
%32 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1806.04740}
\bibitem{1806.04740}
A.~Padilla,
%``Monodromy inflation and an emergent mechanism for stabilising the cosmological constant,''
JHEP \textbf{01} (2019), 175
doi:10.1007/JHEP01(2019)175
[arXiv:1806.04740 [hep-th]].
%7 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1903.07612}
\bibitem{1903.07612}
B.~K.~El-Menoufi, S.~Nagy, F.~Niedermann and A.~Padilla,
%``Quantum corrections to vacuum energy sequestering (with monodromy),''
Class. Quant. Grav. \textbf{36} (2019) no.21, 215014
doi:10.1088/1361-6382/ab46f6
[arXiv:1903.07612 [hep-th]].
%4 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1806.03308}
\bibitem{1806.03308}
N.~Kaloper,
%``Irrational Monodromies of Vacuum Energy,''
JHEP \textbf{11} (2019), 106
doi:10.1007/JHEP11(2019)106
[arXiv:1806.03308 [hep-th]].
%8 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2013zca}
\bibitem{Kaloper:2013zca}
N.~Kaloper and A.~Padilla,
%``Sequestering the Standard Model Vacuum Energy,''
Phys. Rev. Lett. \textbf{112} (2014) no.9, 091304
doi:10.1103/PhysRevLett.112.091304
[arXiv:1309.6562 [hep-th]].
%128 citations counted in INSPIRE as of 20 Oct 2021

%\cite{Kaloper:2014dqa}
\bibitem{Kaloper:2014dqa}
N.~Kaloper and A.~Padilla,
%``Vacuum Energy Sequestering: The Framework and Its Cosmological Consequences,''
Phys. Rev. D \textbf{90} (2014) no.8, 084023
doi:10.1103/PhysRevD.90.084023
[arXiv:1406.0711 [hep-th]].
%85 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2014fca}
\bibitem{Kaloper:2014fca}
N.~Kaloper and A.~Padilla,
%``Sequestration of Vacuum Energy and the End of the Universe,''
Phys. Rev. Lett. \textbf{114} (2015) no.10, 101302
doi:10.1103/PhysRevLett.114.101302
[arXiv:1409.7073 [hep-th]].
%40 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2015jra}
\bibitem{Kaloper:2015jra}
N.~Kaloper, A.~Padilla, D.~Stefanyszyn and G.~Zahariade,
%``Manifestly Local Theory of Vacuum Energy Sequestering,''
Phys. Rev. Lett. \textbf{116} (2016) no.5, 051302
doi:10.1103/PhysRevLett.116.051302
[arXiv:1505.01492 [hep-th]].
%66 citations counted in INSPIRE as of 13 Oct 2021

%\cite{Kaloper:2016yfa}
\bibitem{Kaloper:2016yfa}
N.~Kaloper, A.~Padilla and D.~Stefanyszyn,
%``Sequestering effects on and of vacuum decay,''
Phys. Rev. D \textbf{94} (2016) no.2, 025022
doi:10.1103/PhysRevD.94.025022
[arXiv:1604.04000 [hep-th]].
%17 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2016jsd}
\bibitem{Kaloper:2016jsd}
N.~Kaloper and A.~Padilla,
%``Vacuum Energy Sequestering and Graviton Loops,''
Phys. Rev. Lett. \textbf{118} (2017) no.6, 061303
doi:10.1103/PhysRevLett.118.061303
[arXiv:1606.04958 [hep-th]].
%29 citations counted in INSPIRE as of 11 Oct 2021

%\cite{DAmico:2017ngr}
\bibitem{DAmico:2017ngr}
G.~D'Amico, N.~Kaloper, A.~Padilla, D.~Stefanyszyn, A.~Westphal and G.~Zahariade,
%``An \'etude on global vacuum energy sequester,''
JHEP \textbf{09} (2017), 074
doi:10.1007/JHEP09(2017)074
[arXiv:1705.08950 [hep-th]].
%18 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Niedermann:2017cel}
\bibitem{Niedermann:2017cel}
F.~Niedermann and A.~Padilla,
%``Gravitational Mechanisms to Self-Tune the Cosmological Constant: Obstructions and Ways Forward,''
Phys. Rev. Lett. \textbf{119} (2017) no.25, 251306
doi:10.1103/PhysRevLett.119.251306
[arXiv:1706.04778 [hep-th]].
%13 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Coltman:2019mql}
\bibitem{Coltman:2019mql}
B.~Coltman, Y.~Li and A.~Padilla,
%``Cosmological consequences of Omnia Sequestra,''
JCAP \textbf{06} (2019), 017
doi:10.1088/1475-7516/2019/06/017
[arXiv:1903.02829 [hep-th]].
%4 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9510227}
\bibitem{hep-th/9510227}
J.~Polchinski and A.~Strominger,
%``New vacua for type II string theory,''
Phys. Lett. B \textbf{388} (1996), 736-742
doi:10.1016/S0370-2693(96)01219-1
[arXiv:hep-th/9510227 [hep-th]].
%346 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0004134}
\bibitem{hep-th/0004134}
R.~Bousso and J.~Polchinski,
%``Quantization of four form fluxes and dynamical neutralization of the cosmological constant,''
JHEP \textbf{06} (2000), 006
doi:10.1088/1126-6708/2000/06/006
[arXiv:hep-th/0004134 [hep-th]].
%1208 citations counted in INSPIRE as of 22 Oct 2021

%\cite{Lee:1987qc}
\bibitem{Lee:1987qc}
K.~M.~Lee and E.~J.~Weinberg,
%``Decay of the True Vacuum in Curved Space-time,''
Phys. Rev. D \textbf{36} (1987), 1088
doi:10.1103/PhysRevD.36.1088
%149 citations counted in INSPIRE as of 05 Nov 2021

%\cite{hep-th/0607223}
\bibitem{hep-th/0607223}
B.~S.~Acharya, F.~Benini and R.~Valandro,
%``Fixing moduli in exact type IIA flux vacua,''
JHEP \textbf{02} (2007), 018
doi:10.1088/1126-6708/2007/02/018
[arXiv:hep-th/0607223 [hep-th]].
%96 citations counted in INSPIRE as of 25 Oct 2021

%\cite{0812.3551}
\bibitem{0812.3551}
C.~Caviezel, P.~Koerber, S.~Kors, D.~Lust, T.~Wrase and M.~Zagermann,
%``On the Cosmology of Type IIA Compactifications on SU(3)-structure Manifolds,''
JHEP \textbf{04} (2009), 010
doi:10.1088/1126-6708/2009/04/010
[arXiv:0812.3551 [hep-th]].
%133 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1807.09698}
\bibitem{1807.09698}
D.~Andriot,
%``New constraints on classical de Sitter: flirting with the swampland,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800103
doi:10.1002/prop.201800103
[arXiv:1807.09698 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Ibanez:2017vfl}
\bibitem{Ibanez:2017vfl}
L.~E.~Ibanez and M.~Montero,
%``A Note on the WGC, Effective Field Theory and Clockwork within String Theory,''
JHEP \textbf{02} (2018), 057
doi:10.1007/JHEP02(2018)057
[arXiv:1709.02392 [hep-th]].
%36 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1507.06793}
\bibitem{1507.06793}
S.~Bielleman, L.~E.~Ibanez and I.~Valenzuela,
%``Minkowski 3-forms, Flux String Vacua, Axion Stability and Naturalness,''
JHEP \textbf{12} (2015), 119
doi:10.1007/JHEP12(2015)119
[arXiv:1507.06793 [hep-th]].
%69 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1606.00508}
\bibitem{1606.00508}
F.~Carta, F.~Marchesano, W.~Staessens and G.~Zoccarato,
%``Open string multi-branched and K\"ahler potentials,''
JHEP \textbf{09} (2016), 062
doi:10.1007/JHEP09(2016)062
[arXiv:1606.00508 [hep-th]].
%56 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0103233}
\bibitem{hep-th/0103233}
E.~Bergshoeff, R.~Kallosh, T.~Ortin, D.~Roest and A.~Van Proeyen,
%``New formulations of D = 10 supersymmetry and D8 - O8 domain walls,''
Class. Quant. Grav. \textbf{18} (2001), 3359-3382
doi:10.1088/0264-9381/18/17/303
[arXiv:hep-th/0103233 [hep-th]].
%303 citations counted in INSPIRE as of 08 Nov 2021

%\cite{hep-th/0411271}
\bibitem{hep-th/0411271}
A.~Saltman and E.~Silverstein,
%``A New handle on de Sitter compactifications,''
JHEP \textbf{01} (2006), 139
doi:10.1088/1126-6708/2006/01/139
[arXiv:hep-th/0411271 [hep-th]].
%99 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0505160}
\bibitem{hep-th/0505160}
O.~DeWolfe, A.~Giryavets, S.~Kachru and W.~Taylor,
%``Type IIA moduli stabilization,''
JHEP \textbf{07} (2005), 066
doi:10.1088/1126-6708/2005/07/066
[arXiv:hep-th/0505160 [hep-th]].
%375 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1705.10162}
\bibitem{1705.10162}
G.~F.~Giudice and M.~McCullough,
%``Comment on ''Disassembling the Clockwork Mechanism'',''
[arXiv:1705.10162 [hep-ph]].
%43 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-ph/9905221}
\bibitem{hep-ph/9905221}
L.~Randall and R.~Sundrum,
%``A Large mass hierarchy from a small extra dimension,''
Phys. Rev. Lett. \textbf{83} (1999), 3370-3373
doi:10.1103/PhysRevLett.83.3370
[arXiv:hep-ph/9905221 [hep-ph]].
%9255 citations counted in INSPIRE as of 05 Nov 2021

%\cite{1808.08967}
\bibitem{1808.08967}
M.~Cicoli, S.~De Alwis, A.~Maharana, F.~Muia and F.~Quevedo,
%``De Sitter vs Quintessence in String Theory,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800079
doi:10.1002/prop.201800079
[arXiv:1808.08967 [hep-th]].
%134 citations counted in INSPIRE as of 02 Nov 2021
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF CHAPTER 4 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% CHAPTER 5 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cite{Ooguri:2006in}
\bibitem{distance1}
H.~Ooguri and C.~Vafa,
%``On the Geometry of the String Landscape and the Swampland,''
Nucl. Phys. B \textbf{766} (2007), 21-33
%doi:10.1016/j.nuclphysb.2006.10.033
[arXiv:hep-th/0605264 [hep-th]].
%483 citations counted in INSPIRE as of 17 Dec 2020


%\cite{Klaewer:2016kiy}
\bibitem{distance2}
D.~Klaewer and E.~Palti,
%``Super-Planckian Spatial Field Variations and Quantum Gravity,''
JHEP \textbf{01} (2017), 088
%doi:10.1007/JHEP01(2017)088
[arXiv:1610.00010 [hep-th]].
%154 citations counted in INSPIRE as of 17 Dec 2020


%\cite{Grimm:2018ohb}
\bibitem{distance3}
T.~W.~Grimm, E.~Palti and I.~Valenzuela,
%``Infinite Distances in Field Space and Massless Towers of States,''
JHEP \textbf{08} (2018), 143
%doi:10.1007/JHEP08(2018)143
[arXiv:1802.08264 [hep-th]].
%128 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Blumenhagen:2018nts}
\bibitem{distance4}
R.~Blumenhagen, D.~Kl\"awer, L.~Schlechter and F.~Wolf,
%``The Refined Swampland Distance Conjecture in Calabi-Yau Moduli Spaces,''
JHEP \textbf{06} (2018), 052
%doi:10.1007/JHEP06(2018)052
[arXiv:1803.04989 [hep-th]].
%68 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Agrawal:2018own}
\bibitem{swampcos}
P.~Agrawal, G.~Obied, P.~J.~Steinhardt and C.~Vafa,
%``On the Cosmological Implications of the String Swampland,''
Phys. Lett. B \textbf{784} (2018), 271-276
%doi:10.1016/j.physletb.2018.07.040
[arXiv:1806.09718 [hep-th]].
%287 citations counted in INSPIRE as of 18 Dec 2020


%\cite{Obied:2018sgi}
\bibitem{dscon1}
G.~Obied, H.~Ooguri, L.~Spodyneiko and C.~Vafa,
%``De Sitter Space and the Swampland,''
[arXiv:1806.08362 [hep-th]].
%475 citations counted in INSPIRE as of 17 Dec 2020


%\cite{Garg:2018reu}
\bibitem{chet}
S.~K.~Garg and C.~Krishnan,
%``Bounds on Slow Roll and the de Sitter Swampland,''
JHEP \textbf{11} (2019), 075
%doi:10.1007/JHEP11(2019)075
[arXiv:1807.05193 [hep-th]].
%369 citations counted in INSPIRE as of 06 Aug 2021


%\cite{Ooguri:2018wrx}
\bibitem{dscon2}
H.~Ooguri, E.~Palti, G.~Shiu and C.~Vafa,
%``Distance and de Sitter Conjectures on the Swampland,''
Phys. Lett. B \textbf{788} (2019), 180-184
%doi:10.1016/j.physletb.2018.11.018
[arXiv:1810.05506 [hep-th]].
%306 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Baume:2016psm}
\bibitem{moredist1}
F.~Baume and E.~Palti,
%``Backreacted Axion Field Ranges in String Theory,''
JHEP \textbf{08} (2016), 043
%doi:10.1007/JHEP08(2016)043
[arXiv:1602.06517 [hep-th]].
%99 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Hebecker:2017lxm}
\bibitem{moredist2}
A.~Hebecker, P.~Henkenjohann and L.~T.~Witkowski,
%``Flat Monodromies and a Moduli Space Size Conjecture,''
JHEP \textbf{12} (2017), 033
%doi:10.1007/JHEP12(2017)033
[arXiv:1708.06761 [hep-th]].
%49 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Cicoli:2018tcq}
\bibitem{moredist3}
M.~Cicoli, D.~Ciupke, C.~Mayrhofer and P.~Shukla,
%``A Geometrical Upper Bound on the Inflaton Range,''
JHEP \textbf{05} (2018), 001
%doi:10.1007/JHEP05(2018)001
[arXiv:1801.05434 [hep-th]].
%47 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Blumenhagen:2017cxt}
\bibitem{moredist4}
R.~Blumenhagen, I.~Valenzuela and F.~Wolf,
%``The Swampland Conjecture and F-term Axion Monodromy Inflation,''
JHEP \textbf{07} (2017), 145
%doi:10.1007/JHEP07(2017)145
[arXiv:1703.05776 [hep-th]].
%86 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Heidenreich:2018kpg}
\bibitem{moredist4}
B.~Heidenreich, M.~Reece and T.~Rudelius,
%``Emergence of Weak Coupling at Large Distance in Quantum Gravity,''
Phys. Rev. Lett. \textbf{121} (2018) no.5, 051601
%doi:10.1103/PhysRevLett.121.051601
[arXiv:1802.08698 [hep-th]].
%83 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Landete:2018kqf}
\bibitem{moredist5}
A.~Landete and G.~Shiu,
%``Mass Hierarchies and Dynamical Field Range,''
Phys. Rev. D \textbf{98} (2018) no.6, 066012
d%oi:10.1103/PhysRevD.98.066012
[arXiv:1806.01874 [hep-th]].
%33 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Lee:2018urn}
\bibitem{moredist6}
S.~J.~Lee, W.~Lerche and T.~Weigand,
%``Tensionless Strings and the Weak Gravity Conjecture,''
JHEP \textbf{10} (2018), 164
%doi:10.1007/JHEP10(2018)164
[arXiv:1808.05958 [hep-th]].
%87 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Blumenhagen:2018hsh}
\bibitem{moredist7}
R.~Blumenhagen,
%``Large Field Inflation/Quintessence and the Refined Swampland Distance Conjecture,''
PoS \textbf{CORFU2017} (2018), 175
%doi:10.22323/1.318.0175
[arXiv:1804.10504 [hep-th]].
%47 citations counted in INSPIRE as of 17 Dec 2020

  %\cite{Mukhanov:2007zz}
\bibitem{mukbook}
V.~Mukhanov and S.~Winitzki,
``Introduction to quantum effects in gravity.''
%122 citations counted in INSPIRE as of 26 Apr 2021

%\cite{Bordin:2019fek}
\bibitem{dsstuff}
F.~Cunillera and A.~Padilla,
In preparation.

\bibitem{AS}
M.~Abramowitz and I.~Stegun,
``Handbook of Mathematical Functions with Formulas, Graphs, and Mathematical Tables."
%122 citations counted in INSPIRE as of 26 Apr 2021

%\cite{Khoury:2003aq}
\bibitem{cham1}
J.~Khoury and A.~Weltman,
%``Chameleon fields: Awaiting surprises for tests of gravity in space,''
Phys. Rev. Lett. \textbf{93} (2004), 171104
%doi:10.1103/PhysRevLett.93.171104
[arXiv:astro-ph/0309300 [astro-ph]].
%1202 citations counted in INSPIRE as of 30 Apr 2021

%\cite{Khoury:2003rn}
\bibitem{cham2}
J.~Khoury and A.~Weltman,
%``Chameleon cosmology,''
Phys. Rev. D \textbf{69} (2004), 044026
%doi:10.1103/PhysRevD.69.044026
[arXiv:astro-ph/0309411 [astro-ph]].
%1279 citations counted in INSPIRE as of 30 Apr 2021

%\cite{Padilla:2015wlv}
\bibitem{cham3}
A.~Padilla, E.~Platts, D.~Stefanyszyn, A.~Walters, A.~Weltman and T.~Wilson,
%``How to Avoid a Swift Kick in the Chameleons,''
JCAP \textbf{03} (2016), 058
%doi:10.1088/1475-7516/2016/03/058
[arXiv:1511.05761 [hep-th]].
%11 citations counted in INSPIRE as of 30 Apr 2021

%\cite{Font:2019cxq}
\bibitem{Font:2019cxq}
A.~Font, A.~Herr\'aez and L.~E.~Ib\'a\~nez,
%``The Swampland Distance Conjecture and Towers of Tensionless Branes,''
JHEP \textbf{08} (2019), 044
%doi:10.1007/JHEP08(2019)044
[arXiv:1904.05379 [hep-th]].
%39 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Hebecker:2019csg}
\bibitem{Heb}
A.~Hebecker, T.~Skrzypek and M.~Wittner,
%``The $F$-term Problem and other Challenges of Stringy Quintessence,''
JHEP \textbf{11} (2019), 134
%doi:10.1007/JHEP11(2019)134
[arXiv:1909.08625 [hep-th]].
%13 citations counted in INSPIRE as of 07 Jul 2021

%\cite{1808.09440}
\bibitem{1808.09440}
Y.~Akrami, R.~Kallosh, A.~Linde and V.~Vardanyan,
%``The Landscape, the Swampland and the Era of Precision Cosmology,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800075
doi:10.1002/prop.201800075
[arXiv:1808.09440 [hep-th]].
%192 citations counted in INSPIRE as of 08 Nov 2021

%\cite{hep-th/0603057}
\bibitem{hep-th/0603057}
E.~J.~Copeland, M.~Sami and S.~Tsujikawa,
%``Dynamics of dark energy,''
Int. J. Mod. Phys. D \textbf{15} (2006), 1753-1936
doi:10.1142/S021827180600942X
[arXiv:hep-th/0603057 [hep-th]].
%4649 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1909.11063}
\bibitem{1909.11063}
A.~Bedroya and C.~Vafa,
%``Trans-Planckian Censorship and the Swampland,''
JHEP \textbf{09} (2020), 123
doi:10.1007/JHEP09(2020)123
[arXiv:1909.11063 [hep-th]].
%190 citations counted in INSPIRE as of 02 Nov 2021

%\cite{2110.07300}
\bibitem{2110.07300}
M.~Dine and Y.~Yu,
%``Comments on the Transplanckian Censorship Conjecture,''
[arXiv:2110.07300 [hep-th]].
%0 citations counted in INSPIRE as of 03 Nov 2021

%\cite{Banerjee:2020xcn}
\bibitem{2006.00244}
A.~Banerjee, H.~Cai, L.~Heisenberg, E.~\'O.~Colg\'ain, M.~M.~Sheikh-Jabbari and T.~Yang,
%``Hubble sinks in the low-redshift swampland,''
Phys. Rev. D \textbf{103} (2021) no.8, L081305
doi:10.1103/PhysRevD.103.L081305
[arXiv:2006.00244 [astro-ph.CO]].
%52 citations counted in INSPIRE as of 09 Nov 2021
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF CHAPTER 5 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CHAPTER 6 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\cite{2008.12399}
\bibitem{2008.12399}
M.~Dine, J.~A.~P.~Law-Smith, S.~Sun, D.~Wood and Y.~Yu,
%``Obstacles to Constructing de Sitter Space in String Theory,''
JHEP \textbf{02} (2021), 050
doi:10.1007/JHEP02(2021)050
[arXiv:2008.12399 [hep-th]].
%7 citations counted in INSPIRE as of 15 Oct 2021

%\cite{1807.09698}
\bibitem{1807.09698}
D.~Andriot,
%``New constraints on classical de Sitter: flirting with the swampland,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800103
doi:10.1002/prop.201800103
[arXiv:1807.09698 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1703.05776}
\bibitem{1703.05776}
R.~Blumenhagen, I.~Valenzuela and F.~Wolf,
%``The Swampland Conjecture and F-term Axion Monodromy Inflation,''
JHEP \textbf{07} (2017), 145
doi:10.1007/JHEP07(2017)145
[arXiv:1703.05776 [hep-th]].
%96 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1610.01533}
\bibitem{1610.01533}
H.~Ooguri and C.~Vafa,
%``Non-supersymmetric AdS and the Swampland,''
Adv. Theor. Math. Phys. \textbf{21} (2017), 1787-1801
doi:10.4310/ATMP.2017.v21.n7.a8
[arXiv:1610.01533 [hep-th]].
%253 citations counted in INSPIRE as of 06 Jan 2022

%\cite{hep-th/0007018}
\bibitem{hep-th/0007018}
J.~M.~Maldacena and C.~Nunez,
%``Supergravity description of field theories on curved manifolds and a no go theorem,''
Int. J. Mod. Phys. A \textbf{16} (2001), 822-855
doi:10.1142/S0217751X01003937
[arXiv:hep-th/0007018 [hep-th]].
%1017 citations counted in INSPIRE as of 01 Nov 2021

%\cite{0711.2512}
\bibitem{0711.2512}
M.~P.~Hertzberg, S.~Kachru, W.~Taylor and M.~Tegmark,
%``Inflationary Constraints on Type IIA String Theory,''
JHEP \textbf{12} (2007), 095
doi:10.1088/1126-6708/2007/12/095
[arXiv:0711.2512 [hep-th]].
%213 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1810.09406}
\bibitem{1810.09406}
S.~K.~Garg, C.~Krishnan and M.~Zaid Zaz,
%``Bounds on Slow Roll at the Boundary of the Landscape,''
JHEP \textbf{03} (2019), 029
doi:10.1007/JHEP03(2019)029
[arXiv:1810.09406 [hep-th]].
%69 citations counted in INSPIRE as of 14 Dec 2021

%\cite{2005.10168}
\bibitem{2005.10168}
B.~Valeixo Bento, D.~Chakraborty, S.~L.~Parameswaran and I.~Zavala,
%``Dark Energy in String Theory,''
PoS \textbf{CORFU2019} (2020), 123
doi:10.22323/1.376.0123
[arXiv:2005.10168 [hep-th]].
%4 citations counted in INSPIRE as of 14 Dec 2021

%\cite{1909.08625}
\bibitem{1909.08625}
A.~Hebecker, T.~Skrzypek and M.~Wittner,
%``The $F$-term Problem and other Challenges of Stringy Quintessence,''
JHEP \textbf{11} (2019), 134
doi:10.1007/JHEP11(2019)134
[arXiv:1909.08625 [hep-th]].
%16 citations counted in INSPIRE as of 14 Dec 2021

%\cite{1808.08967}
\bibitem{1808.08967}
M.~Cicoli, S.~De Alwis, A.~Maharana, F.~Muia and F.~Quevedo,
%``De Sitter vs Quintessence in String Theory,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800079
doi:10.1002/prop.201800079
[arXiv:1808.08967 [hep-th]].
%139 citations counted in INSPIRE as of 06 Jan 2022

%\cite{hep-th/0605264}
\bibitem{hep-th/0605264}
H.~Ooguri and C.~Vafa,
%``On the Geometry of the String Landscape and the Swampland,''
Nucl. Phys. B \textbf{766} (2007), 21-33
doi:10.1016/j.nuclphysb.2006.10.033
[arXiv:hep-th/0605264 [hep-th]].
%617 citations counted in INSPIRE as of 06 Jan 2022

%\cite{1610.00010}
\bibitem{1610.00010}
D.~Klaewer and E.~Palti,
%``Super-Planckian Spatial Field Variations and Quantum Gravity,''
JHEP \textbf{01} (2017), 088
doi:10.1007/JHEP01(2017)088
[arXiv:1610.00010 [hep-th]].
%183 citations counted in INSPIRE as of 22 Dec 2021

%\cite{1802.08264}
\bibitem{1802.08264}
T.~W.~Grimm, E.~Palti and I.~Valenzuela,
%``Infinite Distances in Field Space and Massless Towers of States,''
JHEP \textbf{08} (2018), 143
doi:10.1007/JHEP08(2018)143
[arXiv:1802.08264 [hep-th]].
%174 citations counted in INSPIRE as of 30 Dec 2021

%\cite{1803.04989}
\bibitem{1803.04989}
R.~Blumenhagen, D.~Kl\"awer, L.~Schlechter and F.~Wolf,
%``The Refined Swampland Distance Conjecture in Calabi-Yau Moduli Spaces,''
JHEP \textbf{06} (2018), 052
doi:10.1007/JHEP06(2018)052
[arXiv:1803.04989 [hep-th]].
%95 citations counted in INSPIRE as of 06 Jan 2022

%\cite{1904.05379}
\bibitem{1904.05379}
A.~Font, A.~Herr\'aez and L.~E.~Ib\'a\~nez,
%``The Swampland Distance Conjecture and Towers of Tensionless Branes,''
JHEP \textbf{08} (2019), 044
doi:10.1007/JHEP08(2019)044
[arXiv:1904.05379 [hep-th]].
%63 citations counted in INSPIRE as of 06 Jan 2022

%\cite{1810.05506}
\bibitem{1810.05506}
H.~Ooguri, E.~Palti, G.~Shiu and C.~Vafa,
%``Distance and de Sitter Conjectures on the Swampland,''
Phys. Lett. B \textbf{788} (2019), 180-184
doi:10.1016/j.physletb.2018.11.018
[arXiv:1810.05506 [hep-th]].
%434 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Burgess:2020qsc}
\bibitem{Burgess:2020qsc}
C.~P.~Burgess, M.~Cicoli, D.~Ciupke, S.~Krippendorf and F.~Quevedo,
%``UV Shadows in EFTs: Accidental Symmetries, Robustness and No-Scale Supergravity,''
Fortsch. Phys. \textbf{68} (2020) no.10, 2000076
doi:10.1002/prop.202000076
[arXiv:2006.06694 [hep-th]].
%16 citations counted in INSPIRE as of 22 Dec 2021

%\cite{hep-th/0507153}
\bibitem{hep-th/0507153}
T.~W.~Grimm,
%``The Effective action of type II Calabi-Yau orientifolds,''
Fortsch. Phys. \textbf{53} (2005), 1179-1271
doi:10.1002/prop.200510253
[arXiv:hep-th/0507153 [hep-th]].
%77 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2013rwa}
\bibitem{Cicoli:2013rwa}
M.~Cicoli, S.~de Alwis and A.~Westphal,
%``Heterotic Moduli Stabilisation,''
JHEP \textbf{10} (2013), 199
doi:10.1007/JHEP10(2013)199
[arXiv:1304.1809 [hep-th]].
%47 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2020cfj}
\bibitem{Cicoli:2020cfj}
M.~Cicoli, G.~Dibitetto and F.~G.~Pedro,
%``New accelerating solutions in late-time cosmology,''
Phys. Rev. D \textbf{101} (2020) no.10, 103524
doi:10.1103/PhysRevD.101.103524
[arXiv:2002.02695 [gr-qc]].
%12 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2020noz}
\bibitem{Cicoli:2020noz}
M.~Cicoli, G.~Dibitetto and F.~G.~Pedro,
%``Out of the Swampland with Multifield Quintessence?,''
JHEP \textbf{10} (2020), 035
doi:10.1007/JHEP10(2020)035
[arXiv:2007.11011 [hep-th]].
%16 citations counted in INSPIRE as of 22 Dec 2021

\bibitem{Brinkman:2022}
M.~Brinkmann, M.~Cicoli, G.~Dibitetto and F.~G.~Pedro,
To appear

%\cite{Boyle:2001du}
\bibitem{Boyle:2001du}
L.~A.~Boyle, R.~R.~Caldwell and M.~Kamionkowski,
%``Spintessence! New models for dark matter and dark energy,''
Phys. Lett. B \textbf{545} (2002), 17-22
doi:10.1016/S0370-2693(02)02590-X
[arXiv:astro-ph/0105318 [astro-ph]].
%160 citations counted in INSPIRE as of 22 Dec 2021

%\cite{AbdusSalam:2020ywo}
\bibitem{AbdusSalam:2020ywo}
S.~AbdusSalam, S.~Abel, M.~Cicoli, F.~Quevedo and P.~Shukla,
%``A systematic approach to K\"ahler moduli stabilisation,''
JHEP \textbf{08} (2020) no.08, 047
doi:10.1007/JHEP08(2020)047
[arXiv:2005.11329 [hep-th]].
%20 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2021rub}
\bibitem{Cicoli:2021rub}
M.~Cicoli, F.~Quevedo, R.~Savelli, A.~Schachner and R.~Valandro,
%``Systematics of the $\alpha'$ Expansion in F-Theory,''
JHEP \textbf{2021} (2021), 99
doi:10.1007/JHEP08(2021)099
[arXiv:2106.04592 [hep-th]].
%6 citations counted in INSPIRE as of 05 Jan 2022

\bibitem{Cicoli:2021skd}
M.~Cicoli, F.~Cunillera, A.~Padilla and F.~G.~Pedro,
%``Quintessence and the Swampland: The numerically controlled regime of moduli space,''
[arXiv:2112.10783 [hep-th]].
%0 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Romans:1985tz}
\bibitem{Romans:1985tz}
L.~J.~Romans,
%``Massive N=2a Supergravity in Ten-Dimensions,''
Phys. Lett. B \textbf{169} (1986), 374
doi:10.1016/0370-2693(86)90375-8
%555 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Dyson:1952tj}
\bibitem{Dyson:1952tj}
F.~J.~Dyson,
%``Divergence of perturbation theory in quantum electrodynamics,''
Phys. Rev. \textbf{85} (1952), 631-632
doi:10.1103/PhysRev.85.631
%594 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1205.5368}
\bibitem{1205.5368}
T.~Aoyama, M.~Hayakawa, T.~Kinoshita and M.~Nio,
%``Tenth-Order QED Contribution to the Electron g-2 and an Improved Value of the Fine Structure Constant,''
Phys. Rev. Lett. \textbf{109} (2012), 111807
doi:10.1103/PhysRevLett.109.111807
[arXiv:1205.5368 [hep-ph]].
%357 citations counted in INSPIRE as of 01 Nov 2021

%\cite{Hanneke:2008tm}
\bibitem{Hanneke:2008tm}
D.~Hanneke, S.~Fogwell and G.~Gabrielse,
%``New Measurement of the Electron Magnetic Moment and the Fine Structure Constant,''
Phys. Rev. Lett. \textbf{100} (2008), 120801
doi:10.1103/PhysRevLett.100.120801
[arXiv:0801.1134 [physics.atom-ph]].
%725 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Bender:1969si}
\bibitem{Bender:1969si}
C.~M.~Bender and T.~T.~Wu,
%``Anharmonic oscillator,''
Phys. Rev. \textbf{184} (1969), 1231-1260
doi:10.1103/PhysRev.184.1231
%467 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Banks:1972xa}
\bibitem{Banks:1972xa}
T.~I.~Banks and C.~M.~Bender,
%``Anharmonic oscillator with polynomial self-interaction,''
J. Math. Phys. \textbf{13} (1972), 1320-1324
doi:10.1063/1.1666140
%18 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Bender:1973rz}
\bibitem{Bender:1973rz}
C.~M.~Bender and T.~T.~Wu,
%``Anharmonic oscillator. 2: A Study of perturbation theory in large order,''
Phys. Rev. D \textbf{7} (1973), 1620-1636
doi:10.1103/PhysRevD.7.1620
%347 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Graffi:1970erh}
\bibitem{Graffi:1970erh}
S.~Graffi, V.~Grecchi and B.~Simon,
%``Borel summability: Application to the anharmonic oscillator,''
Phys. Lett. B \textbf{32} (1970), 631-634
doi:10.1016/0370-2693(70)90564-2
%115 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1610.01533}
\bibitem{1610.01533}
H.~Ooguri and C.~Vafa,
%``Non-supersymmetric AdS and the Swampland,''
Adv. Theor. Math. Phys. \textbf{21} (2017), 1787-1801
doi:10.4310/ATMP.2017.v21.n7.a8
[arXiv:1610.01533 [hep-th]].
%242 citations counted in INSPIRE as of 03 Nov 2021

%\cite{1611.01395}
\bibitem{1611.01395}
U.~Danielsson and G.~Dibitetto,
%``Fate of stringy AdS vacua and the weak gravity conjecture,''
Phys. Rev. D \textbf{96} (2017) no.2, 026020
doi:10.1103/PhysRevD.96.026020
[arXiv:1611.01395 [hep-th]].
%34 citations counted in INSPIRE as of 19 Oct 2021

%\cite{1611.08953}
\bibitem{1611.08953}
T.~Banks,
%``Note on a Paper by Ooguri and Vafa,''
[arXiv:1611.08953 [hep-th]].
%17 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1708.03293}
\bibitem{1708.03293}
U.~H.~Danielsson, G.~Dibitetto and S.~C.~Vargas,
%``A swamp of non-SUSY vacua,''
JHEP \textbf{11} (2017), 152
doi:10.1007/JHEP11(2017)152
[arXiv:1708.03293 [hep-th]].
%19 citations counted in INSPIRE as of 29 Oct 2021

%\cite{2003.10452}
\bibitem{2003.10452}
E.~Palti, C.~Vafa and T.~Weigand,
%``Supersymmetric Protection and the Swampland,''
JHEP \textbf{06} (2020), 168
doi:10.1007/JHEP06(2020)168
[arXiv:2003.10452 [hep-th]].
%27 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1808.09440}
\bibitem{1808.09440}
Y.~Akrami, R.~Kallosh, A.~Linde and V.~Vardanyan,
%``The Landscape, the Swampland and the Era of Precision Cosmology,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800075
doi:10.1002/prop.201800075
[arXiv:1808.09440 [hep-th]].
%192 citations counted in INSPIRE as of 08 Nov 2021

%\cite{2106.04592}
\bibitem{2106.04592}
M.~Cicoli, F.~Quevedo, R.~Savelli, A.~Schachner and R.~Valandro,
%``Systematics of the $\alpha'$ Expansion in F-Theory,''
JHEP \textbf{2021} (2021), 99
doi:10.1007/JHEP08(2021)099
[arXiv:2106.04592 [hep-th]].
%2 citations counted in INSPIRE as of 04 Nov 2021

%\cite{1908.04788}
\bibitem{1908.04788}
S.~Kachru, M.~Kim, L.~Mcallister and M.~Zimet,
%``de Sitter Vacua from Ten Dimensions,''
[arXiv:1908.04788 [hep-th]].
%39 citations counted in INSPIRE as of 08 Nov 2021

%\cite{hep-th/0301240}
\bibitem{hep-th/0301240}
S.~Kachru, R.~Kallosh, A.~D.~Linde and S.~P.~Trivedi,
%``De Sitter vacua in string theory,''
Phys. Rev. D \textbf{68} (2003), 046005
doi:10.1103/PhysRevD.68.046005
[arXiv:hep-th/0301240 [hep-th]].
%3046 citations counted in INSPIRE as of 08 Nov 2021
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF CHAPTER 6 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CHAPTER 7 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cite{1808.08967}
\bibitem{1808.08967}
M.~Cicoli, S.~De Alwis, A.~Maharana, F.~Muia and F.~Quevedo,
%``De Sitter vs Quintessence in String Theory,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800079
doi:10.1002/prop.201800079
[arXiv:1808.08967 [hep-th]].
%139 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Cicoli:2018kdo}
\bibitem{Cicoli:2018kdo}
M.~Cicoli, S.~De Alwis, A.~Maharana, F.~Muia and F.~Quevedo,
%``De Sitter vs Quintessence in String Theory,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800079
doi:10.1002/prop.201800079
[arXiv:1808.08967 [hep-th]].
%139 citations counted in INSPIRE as of 06 Jan 2022

%\cite{AbdusSalam:2020ywo}
\bibitem{AbdusSalam:2020ywo}
S.~AbdusSalam, S.~Abel, M.~Cicoli, F.~Quevedo and P.~Shukla,
%``A systematic approach to K\"ahler moduli stabilisation,''
JHEP \textbf{08} (2020) no.08, 047
doi:10.1007/JHEP08(2020)047
[arXiv:2005.11329 [hep-th]].
%20 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2021rub}
\bibitem{Cicoli:2021rub}
M.~Cicoli, F.~Quevedo, R.~Savelli, A.~Schachner and R.~Valandro,
%``Systematics of the $\alpha'$ Expansion in F-Theory,''
JHEP \textbf{2021} (2021), 99
doi:10.1007/JHEP08(2021)099
[arXiv:2106.04592 [hep-th]].
%6 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Becker:2002nn}
\bibitem{Becker:2002nn}
K.~Becker, M.~Becker, M.~Haack and J.~Louis,
%``Supersymmetry breaking and alpha-prime corrections to flux induced potentials,''
JHEP \textbf{06} (2002), 060
doi:10.1088/1126-6708/2002/06/060
[arXiv:hep-th/0204254 [hep-th]].
%414 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Berg:2007wt}
\bibitem{Berg:2007wt}
M.~Berg, M.~Haack and E.~Pajer,
%``Jumping Through Loops: On Soft Terms from Large Volume Compactifications,''
JHEP \textbf{09} (2007), 031
doi:10.1088/1126-6708/2007/09/031
[arXiv:0704.0737 [hep-th]].
%171 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2007xp}
\bibitem{Cicoli:2007xp}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``Systematics of String Loop Corrections in Type IIB Calabi-Yau Flux Compactifications,''
JHEP \textbf{01} (2008), 052
doi:10.1088/1126-6708/2008/01/052
[arXiv:0708.1873 [hep-th]].
%180 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Ciupke:2015msa}
\bibitem{Ciupke:2015msa}
D.~Ciupke, J.~Louis and A.~Westphal,
%``Higher-Derivative Supergravity and Moduli Stabilization,''
JHEP \textbf{10} (2015), 094
doi:10.1007/JHEP10(2015)094
[arXiv:1505.03092 [hep-th]].
%73 citations counted in INSPIRE as of 03 Jan 2022

%\cite{Blumenhagen:2009qh}
\bibitem{Blumenhagen:2009qh}
R.~Blumenhagen, M.~Cvetic, S.~Kachru and T.~Weigand,
%``D-Brane Instantons in Type II Orientifolds,''
Ann. Rev. Nucl. Part. Sci. \textbf{59} (2009), 269-296
doi:10.1146/annurev.nucl.010909.083113
[arXiv:0902.3251 [hep-th]].
%239 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Kachru:2003aw}
\bibitem{Kachru:2003aw}
S.~Kachru, R.~Kallosh, A.~D.~Linde and S.~P.~Trivedi,
%``De Sitter vacua in string theory,''
Phys. Rev. D \textbf{68} (2003), 046005
doi:10.1103/PhysRevD.68.046005
[arXiv:hep-th/0301240 [hep-th]].
%3070 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Blanco-Pillado:2004aap}
\bibitem{Blanco-Pillado:2004aap}
J.~J.~Blanco-Pillado, C.~P.~Burgess, J.~M.~Cline, C.~Escoda, M.~Gomez-Reino, R.~Kallosh, A.~D.~Linde and F.~Quevedo,
%``Racetrack inflation,''
JHEP \textbf{11} (2004), 063
doi:10.1088/1126-6708/2004/11/063
[arXiv:hep-th/0406230 [hep-th]].
%270 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Kallosh:2004yh}
\bibitem{Kallosh:2004yh}
R.~Kallosh and A.~D.~Linde,
%``Landscape, the scale of SUSY breaking, and inflation,''
JHEP \textbf{12} (2004), 004
doi:10.1088/1126-6708/2004/12/004
[arXiv:hep-th/0411011 [hep-th]].
%289 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Balasubramanian:2005zx}
\bibitem{Balasubramanian:2005zx}
V.~Balasubramanian, P.~Berglund, J.~P.~Conlon and F.~Quevedo,
%``Systematics of moduli stabilisation in Calabi-Yau flux compactifications,''
JHEP \textbf{03} (2005), 007
doi:10.1088/1126-6708/2005/03/007
[arXiv:hep-th/0502058 [hep-th]].
%914 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Conlon:2005ki}
\bibitem{Conlon:2005ki}
J.~P.~Conlon, F.~Quevedo and K.~Suruliz,
%``Large-volume flux compactifications: Moduli spectrum and D3/D7 soft supersymmetry breaking,''
JHEP \textbf{08} (2005), 007
doi:10.1088/1126-6708/2005/08/007
[arXiv:hep-th/0505076 [hep-th]].
%486 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2008va}
\bibitem{Cicoli:2008va}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``General Analysis of LARGE Volume Scenarios with String Loop Moduli Stabilisation,''
JHEP \textbf{10} (2008), 105
doi:10.1088/1126-6708/2008/10/105
[arXiv:0805.1029 [hep-th]].
%168 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Grisaru:1986dk}
\bibitem{Grisaru:1986dk}
M.~T.~Grisaru, A.~E.~M.~van de Ven and D.~Zanon,
%``Two-Dimensional Supersymmetric Sigma Models on Ricci Flat Kahler Manifolds Are Not Finite,''
Nucl. Phys. B \textbf{277} (1986), 388-408
doi:10.1016/0550-3213(86)90448-7
%235 citations counted in INSPIRE as of 09 Dec 2021

%\cite{Witten:1985bz}
\bibitem{Witten:1985bz}
E.~Witten,
%``New Issues in Manifolds of SU(3) Holonomy,''
Nucl. Phys. B \textbf{268} (1986), 79
doi:10.1016/0550-3213(86)90202-6
%657 citations counted in INSPIRE as of 03 Dec 2021

%\cite{hep-th/0510213}
\bibitem{hep-th/0510213}
C.~P.~Burgess, C.~Escoda and F.~Quevedo,
%``Nonrenormalization of flux superpotentials in string theory,''
JHEP \textbf{06} (2006), 044
doi:10.1088/1126-6708/2006/06/044
[arXiv:hep-th/0510213 [hep-th]].
%40 citations counted in INSPIRE as of 06 Jan 2022

%\cite{hep-th/0404087}
\bibitem{hep-th/0404087}
M.~Berg, M.~Haack and B.~Kors,
%``Loop corrections to volume moduli and inflation in string theory,''
Phys. Rev. D \textbf{71} (2005), 026005
doi:10.1103/PhysRevD.71.026005
[arXiv:hep-th/0404087 [hep-th]].
%212 citations counted in INSPIRE as of 03 Dec 2021

%\cite{Polchinski:1998rr}
\bibitem{Polchinski:1998rr}
J.~Polchinski,
%``String theory. Vol. 2: Superstring theory and beyond,''
doi:10.1017/CBO9780511618123
%448 citations counted in INSPIRE as of 05 Jan 2022

%\cite{hep-th/0204254}
\bibitem{hep-th/0204254}
K.~Becker, M.~Becker, M.~Haack and J.~Louis,
%``Supersymmetry breaking and alpha-prime corrections to flux induced potentials,''
JHEP \textbf{06} (2002), 060
doi:10.1088/1126-6708/2002/06/060
[arXiv:hep-th/0204254 [hep-th]].
%414 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Candelas:1990rm}
\bibitem{Candelas:1990rm}
P.~Candelas, X.~C.~De La Ossa, P.~S.~Green and L.~Parkes,
%``A Pair of Calabi-Yau manifolds as an exactly soluble superconformal theory,''
Nucl. Phys. B \textbf{359} (1991), 21-74
doi:10.1016/0550-3213(91)90292-6
%903 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Ferrara:1989ik}
\bibitem{Ferrara:1989ik}
S.~Ferrara and S.~Sabharwal,
%``Quaternionic Manifolds for Type II Superstring Vacua of Calabi-Yau Spaces,''
Nucl. Phys. B \textbf{332} (1990), 317-332
doi:10.1016/0550-3213(90)90097-W
%328 citations counted in INSPIRE as of 03 Dec 2021

%\cite{Greene:1990ud}
\bibitem{Greene:1990ud}
B.~R.~Greene and M.~R.~Plesser,
%``Duality in {Calabi-Yau} Moduli Space,''
Nucl. Phys. B \textbf{338} (1990), 15-37
doi:10.1016/0550-3213(90)90622-K
%460 citations counted in INSPIRE as of 20 Dec 2021

%\cite{Candelas:1989ug}
\bibitem{Candelas:1989ug}
P.~Candelas, P.~S.~Green and T.~Hubsch,
%``Rolling Among Calabi-Yau Vacua,''
Nucl. Phys. B \textbf{330} (1990), 49
doi:10.1016/0550-3213(90)90302-T
%208 citations counted in INSPIRE as of 24 Dec 2021

%\cite{hep-th/0507153}
\bibitem{hep-th/0507153}
T.~W.~Grimm,
%``The Effective action of type II Calabi-Yau orientifolds,''
Fortsch. Phys. \textbf{53} (2005), 1179-1271
doi:10.1002/prop.200510253
[arXiv:hep-th/0507153 [hep-th]].
%77 citations counted in INSPIRE as of 22 Dec 2021

%\cite{hep-th/0508043}
\bibitem{hep-th/0508043}
M.~Berg, M.~Haack and B.~Kors,
%``String loop corrections to Kahler potentials in orientifolds,''
JHEP \textbf{11} (2005), 030
doi:10.1088/1126-6708/2005/11/030
[arXiv:hep-th/0508043 [hep-th]].
%219 citations counted in INSPIRE as of 05 Jan 2022

%\cite{0704.0737}
\bibitem{0704.0737}
M.~Berg, M.~Haack and E.~Pajer,
%``Jumping Through Loops: On Soft Terms from Large Volume Compactifications,''
JHEP \textbf{09} (2007), 031
doi:10.1088/1126-6708/2007/09/031
[arXiv:0704.0737 [hep-th]].
%171 citations counted in INSPIRE as of 22 Dec 2021

%\cite{hep-th/0502058}
\bibitem{hep-th/0502058}
V.~Balasubramanian, P.~Berglund, J.~P.~Conlon and F.~Quevedo,
%``Systematics of moduli stabilisation in Calabi-Yau flux compactifications,''
JHEP \textbf{03} (2005), 007
doi:10.1088/1126-6708/2005/03/007
[arXiv:hep-th/0502058 [hep-th]].
%914 citations counted in INSPIRE as of 30 Dec 2021

%\cite{1505.03092}
\bibitem{1505.03092}
D.~Ciupke, J.~Louis and A.~Westphal,
%``Higher-Derivative Supergravity and Moduli Stabilization,''
JHEP \textbf{10} (2015), 094
doi:10.1007/JHEP10(2015)094
[arXiv:1505.03092 [hep-th]].
%73 citations counted in INSPIRE as of 03 Jan 2022

%\cite{Freeman:1986br}
\bibitem{Freeman:1986br}
M.~D.~Freeman and C.~N.~Pope,
%``Beta Functions and Superstring Compactifications,''
Phys. Lett. B \textbf{174} (1986), 48-50
doi:10.1016/0370-2693(86)91127-5
%105 citations counted in INSPIRE as of 03 Dec 2021

%\cite{0902.3251}
\bibitem{0902.3251}
R.~Blumenhagen, M.~Cvetic, S.~Kachru and T.~Weigand,
%``D-Brane Instantons in Type II Orientifolds,''
Ann. Rev. Nucl. Part. Sci. \textbf{59} (2009), 269-296
doi:10.1146/annurev.nucl.010909.083113
[arXiv:0902.3251 [hep-th]].
%239 citations counted in INSPIRE as of 22 Dec 2021

%\cite{2005.11329}
\bibitem{2005.11329}
S.~AbdusSalam, S.~Abel, M.~Cicoli, F.~Quevedo and P.~Shukla,
%``A systematic approach to K\"ahler moduli stabilisation,''
JHEP \textbf{08} (2020) no.08, 047
doi:10.1007/JHEP08(2020)047
[arXiv:2005.11329 [hep-th]].
%20 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Blanco-Pillado:2006dgl}
\bibitem{Blanco-Pillado:2006dgl}
J.~J.~Blanco-Pillado, C.~P.~Burgess, J.~M.~Cline, C.~Escoda, M.~Gomez-Reino, R.~Kallosh, A.~D.~Linde and F.~Quevedo,
%``Inflating in a better racetrack,''
JHEP \textbf{09} (2006), 002
doi:10.1088/1126-6708/2006/09/002
[arXiv:hep-th/0603129 [hep-th]].
%145 citations counted in INSPIRE as of 03 Dec 2021

%\cite{Westphal:2006tn}
\bibitem{Westphal:2006tn}
A.~Westphal,
%``de Sitter string vacua from Kahler uplifting,''
JHEP \textbf{03} (2007), 102
doi:10.1088/1126-6708/2007/03/102
[arXiv:hep-th/0611332 [hep-th]].
%147 citations counted in INSPIRE as of 22 Dec 2021

%\cite{hep-th/0307049}
\bibitem{hep-th/0307049}
S.~Ashok and M.~R.~Douglas,
%``Counting flux vacua,''
JHEP \textbf{01} (2004), 060
doi:10.1088/1126-6708/2004/01/060
[arXiv:hep-th/0307049 [hep-th]].
%390 citations counted in INSPIRE as of 06 Jan 2022

%\cite{hep-th/0404116}
\bibitem{hep-th/0404116}
F.~Denef and M.~R.~Douglas,
%``Distributions of flux vacua,''
JHEP \textbf{05} (2004), 072
doi:10.1088/1126-6708/2004/05/072
[arXiv:hep-th/0404116 [hep-th]].
%512 citations counted in INSPIRE as of 06 Jan 2022

%\cite{hep-th/0411183}
\bibitem{hep-th/0411183}
F.~Denef and M.~R.~Douglas,
%``Distributions of nonsupersymmetric flux vacua,''
JHEP \textbf{03} (2005), 061
doi:10.1088/1126-6708/2005/03/061
[arXiv:hep-th/0411183 [hep-th]].
%237 citations counted in INSPIRE as of 30 Dec 2021

%\cite{1511.03209}
\bibitem{1511.03209}
W.~Taylor and Y.~N.~Wang,
%``The F-theory geometry with most flux vacua,''
JHEP \textbf{12} (2015), 164
doi:10.1007/JHEP12(2015)164
[arXiv:1511.03209 [hep-th]].
%100 citations counted in INSPIRE as of 03 Jan 2022

%\cite{2107.09064}
\bibitem{2107.09064}
M.~Demirtas, M.~Kim, L.~McAllister, J.~Moritz and A.~Rios-Tascon,
%``Small cosmological constants in string theory,''
JHEP \textbf{12} (2021), 136
doi:10.1007/JHEP12(2021)136
[arXiv:2107.09064 [hep-th]].
%11 citations counted in INSPIRE as of 06 Jan 2022

%\cite{hep-th/0411011}
\bibitem{hep-th/0411011}
R.~Kallosh and A.~D.~Linde,
%``Landscape, the scale of SUSY breaking, and inflation,''
JHEP \textbf{12} (2004), 004
doi:10.1088/1126-6708/2004/12/004
[arXiv:hep-th/0411011 [hep-th]].
%289 citations counted in INSPIRE as of 22 Dec 2021

%\cite{0907.0665}
\bibitem{0907.0665}
M.~Cicoli,
%``String Loop Moduli Stabilisation and Cosmology in IIB Flux Compactifications,''
Fortsch. Phys. \textbf{58} (2010), 115-338
doi:10.1002/prop.200900096
[arXiv:0907.0665 [hep-th]].
%18 citations counted in INSPIRE as of 03 Dec 2021

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF CHAPTER 7 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CHAPTER 8 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\cite{Obied:2018sgi}
\bibitem{Obied:2018sgi}
G.~Obied, H.~Ooguri, L.~Spodyneiko and C.~Vafa,
%``De Sitter Space and the Swampland,''
[arXiv:1806.08362 [hep-th]].
%637 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Planck:2018vyg}
\bibitem{Planck:2018vyg}
N.~Aghanim \textit{et al.} [Planck],
%``Planck 2018 results. VI. Cosmological parameters,''
Astron. Astrophys. \textbf{641} (2020), A6
[erratum: Astron. Astrophys. \textbf{652} (2021), C4]
doi:10.1051/0004-6361/201833910
[arXiv:1807.06209 [astro-ph.CO]].
%6700 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Planck:2018jri}
\bibitem{Planck:2018jri}
Y.~Akrami \textit{et al.} [Planck],
%``Planck 2018 results. X. Constraints on inflation,''
Astron. Astrophys. \textbf{641} (2020), A10
doi:10.1051/0004-6361/201833887
[arXiv:1807.06211 [astro-ph.CO]].
%1652 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Amendola:2016saw}
\bibitem{Amendola:2016saw}
L.~Amendola, S.~Appleby, A.~Avgoustidis, D.~Bacon, T.~Baker, M.~Baldi, N.~Bartolo, A.~Blanchard, C.~Bonvin and S.~Borgani, \textit{et al.}
%``Cosmology and fundamental physics with the Euclid satellite,''
Living Rev. Rel. \textbf{21} (2018) no.1, 2
doi:10.1007/s41114-017-0010-3
[arXiv:1606.00180 [astro-ph.CO]].
%544 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Denef:2018etk}
\bibitem{Denef:2018etk}
F.~Denef, A.~Hebecker and T.~Wrase,
%``de Sitter swampland conjecture and the Higgs potential,''
Phys. Rev. D \textbf{98} (2018) no.8, 086004
doi:10.1103/PhysRevD.98.086004
[arXiv:1807.06581 [hep-th]].
%129 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Conlon:2018eyr}
\bibitem{Conlon:2018eyr}
J.~P.~Conlon,
%``The de Sitter swampland conjecture and supersymmetric AdS vacua,''
Int. J. Mod. Phys. A \textbf{33} (2018) no.29, 1850178
doi:10.1142/S0217751X18501786
[arXiv:1808.05040 [hep-th]].
%69 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Garg:2018reu}
\bibitem{Garg:2018reu}
S.~K.~Garg and C.~Krishnan,
%``Bounds on Slow Roll and the de Sitter Swampland,''
JHEP \textbf{11} (2019), 075
doi:10.1007/JHEP11(2019)075
[arXiv:1807.05193 [hep-th]].
%413 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Ooguri:2018wrx}
\bibitem{Ooguri:2018wrx}
H.~Ooguri, E.~Palti, G.~Shiu and C.~Vafa,
%``Distance and de Sitter Conjectures on the Swampland,''
Phys. Lett. B \textbf{788} (2019), 180-184
doi:10.1016/j.physletb.2018.11.018
[arXiv:1810.05506 [hep-th]].
%434 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Louis:2012nb}
\bibitem{Louis:2012nb}
J.~Louis, M.~Rummel, R.~Valandro and A.~Westphal,
%``Building an explicit de Sitter,''
JHEP \textbf{10} (2012), 163
doi:10.1007/JHEP10(2012)163
[arXiv:1208.3208 [hep-th]].
%99 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2012vw}
\bibitem{Cicoli:2012vw}
M.~Cicoli, S.~Krippendorf, C.~Mayrhofer, F.~Quevedo and R.~Valandro,
%``D-Branes at del Pezzo Singularities: Global Embedding and Moduli Stabilisation,''
JHEP \textbf{09} (2012), 019
doi:10.1007/JHEP09(2012)019
[arXiv:1206.5237 [hep-th]].
%105 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2012fh}
\bibitem{Cicoli:2012fh}
M.~Cicoli, A.~Maharana, F.~Quevedo and C.~P.~Burgess,
%``De Sitter String Vacua from Dilaton-dependent Non-perturbative Effects,''
JHEP \textbf{06} (2012), 011
doi:10.1007/JHEP06(2012)011
[arXiv:1203.1750 [hep-th]].
%100 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2013cha}
\bibitem{Cicoli:2013cha}
M.~Cicoli, D.~Klevers, S.~Krippendorf, C.~Mayrhofer, F.~Quevedo and R.~Valandro,
%``Explicit de Sitter Flux Vacua for Global String Models with Chiral Matter,''
JHEP \textbf{05} (2014), 001
doi:10.1007/JHEP05(2014)001
[arXiv:1312.0014 [hep-th]].
%102 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Blaback:2013ht}
\bibitem{Blaback:2013ht}
J.~Bl\r{a}b\"ack, U.~Danielsson and G.~Dibitetto,
%``Fully stable dS vacua from generalised fluxes,''
JHEP \textbf{08} (2013), 054
doi:10.1007/JHEP08(2013)054
[arXiv:1301.7073 [hep-th]].
%92 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Braun:2015pza}
\bibitem{Braun:2015pza}
A.~P.~Braun, M.~Rummel, Y.~Sumitomo and R.~Valandro,
%``De Sitter vacua from a D-term generated racetrack potential in hypersurface Calabi-Yau compactifications,''
JHEP \textbf{12} (2015), 033
doi:10.1007/JHEP12(2015)033
[arXiv:1509.06918 [hep-th]].
%23 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cribiori:2019hrb}
\bibitem{Cribiori:2019hrb}
N.~Cribiori, R.~Kallosh, A.~Linde and C.~Roupec,
%``de Sitter Minima from M theory and String theory,''
Phys. Rev. D \textbf{101} (2020) no.4, 046018
doi:10.1103/PhysRevD.101.046018
[arXiv:1912.02791 [hep-th]].
%12 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Antoniadis:2019rkh}
\bibitem{Antoniadis:2019rkh}
I.~Antoniadis, Y.~Chen and G.~K.~Leontaris,
%``Logarithmic loop corrections, moduli stabilisation and de Sitter vacua in string theory,''
JHEP \textbf{01} (2020), 149
doi:10.1007/JHEP01(2020)149
[arXiv:1909.10525 [hep-th]].
%13 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Crino:2020qwk}
\bibitem{Crino:2020qwk}
C.~Crin\`o, F.~Quevedo and R.~Valandro,
%``On de Sitter String Vacua from Anti-D3-Branes in the Large Volume Scenario,''
JHEP \textbf{03} (2021), 258
doi:10.1007/JHEP03(2021)258
[arXiv:2010.15903 [hep-th]].
%17 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2021dhg}
\bibitem{Cicoli:2021dhg}
M.~Cicoli, I.~G.~Etxebarria, F.~Quevedo, A.~Schachner, P.~Shukla and R.~Valandro,
%``The Standard Model quiver in de Sitter string compactifications,''
JHEP \textbf{08} (2021), 109
doi:10.1007/JHEP08(2021)109
[arXiv:2106.11964 [hep-th]].
%7 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Kachru:2003aw}
\bibitem{Kachru:2003aw}
S.~Kachru, R.~Kallosh, A.~D.~Linde and S.~P.~Trivedi,
%``De Sitter vacua in string theory,''
Phys. Rev. D \textbf{68} (2003), 046005
doi:10.1103/PhysRevD.68.046005
[arXiv:hep-th/0301240 [hep-th]].
%3070 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Balasubramanian:2005zx}
\bibitem{Balasubramanian:2005zx}
V.~Balasubramanian, P.~Berglund, J.~P.~Conlon and F.~Quevedo,
%``Systematics of moduli stabilisation in Calabi-Yau flux compactifications,''
JHEP \textbf{03} (2005), 007
doi:10.1088/1126-6708/2005/03/007
[arXiv:hep-th/0502058 [hep-th]].
%914 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Conlon:2005ki}
\bibitem{Conlon:2005ki}
J.~P.~Conlon, F.~Quevedo and K.~Suruliz,
%``Large-volume flux compactifications: Moduli spectrum and D3/D7 soft supersymmetry breaking,''
JHEP \textbf{08} (2005), 007
doi:10.1088/1126-6708/2005/08/007
[arXiv:hep-th/0505076 [hep-th]].
%486 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2008va}
\bibitem{Cicoli:2008va}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``General Analysis of LARGE Volume Scenarios with String Loop Moduli Stabilisation,''
JHEP \textbf{10} (2008), 105
doi:10.1088/1126-6708/2008/10/105
[arXiv:0805.1029 [hep-th]].
%168 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Becker:2002nn}
\bibitem{Becker:2002nn}
K.~Becker, M.~Becker, M.~Haack and J.~Louis,
%``Supersymmetry breaking and alpha-prime corrections to flux induced potentials,''
JHEP \textbf{06} (2002), 060
doi:10.1088/1126-6708/2002/06/060
[arXiv:hep-th/0204254 [hep-th]].
%414 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Berg:2005ja}
\bibitem{Berg:2005ja}
M.~Berg, M.~Haack and B.~Kors,
%``String loop corrections to Kahler potentials in orientifolds,''
JHEP \textbf{11} (2005), 030
doi:10.1088/1126-6708/2005/11/030
[arXiv:hep-th/0508043 [hep-th]].
%219 citations counted in INSPIRE as of 05 Jan 2022

%\cite{vonGersdorff:2005ce}
\bibitem{vonGersdorff:2005ce}
G.~von Gersdorff and A.~Hebecker,
%``Radius stabilization by two-loop Casimir energy,''
Nucl. Phys. B \textbf{720} (2005), 211-227
doi:10.1016/j.nuclphysb.2005.06.001
[arXiv:hep-th/0504002 [hep-th]].
%29 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Berg:2007wt}
\bibitem{Berg:2007wt}
M.~Berg, M.~Haack and E.~Pajer,
%``Jumping Through Loops: On Soft Terms from Large Volume Compactifications,''
JHEP \textbf{09} (2007), 031
doi:10.1088/1126-6708/2007/09/031
[arXiv:0704.0737 [hep-th]].
%171 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2007xp}
\bibitem{Cicoli:2007xp}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``Systematics of String Loop Corrections in Type IIB Calabi-Yau Flux Compactifications,''
JHEP \textbf{01} (2008), 052
doi:10.1088/1126-6708/2008/01/052
[arXiv:0708.1873 [hep-th]].
%180 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Ciupke:2015msa}
\bibitem{Ciupke:2015msa}
D.~Ciupke, J.~Louis and A.~Westphal,
%``Higher-Derivative Supergravity and Moduli Stabilization,''
JHEP \textbf{10} (2015), 094
doi:10.1007/JHEP10(2015)094
[arXiv:1505.03092 [hep-th]].
%73 citations counted in INSPIRE as of 03 Jan 2022

%\cite{Antoniadis:2018hqy}
\bibitem{Antoniadis:2018hqy}
I.~Antoniadis, Y.~Chen and G.~K.~Leontaris,
%``Perturbative moduli stabilisation in type IIB/F-theory framework,''
Eur. Phys. J. C \textbf{78} (2018) no.9, 766
doi:10.1140/epjc/s10052-018-6248-4
[arXiv:1803.08941 [hep-th]].
%26 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Blumenhagen:2009qh}
\bibitem{Blumenhagen:2009qh}
R.~Blumenhagen, M.~Cvetic, S.~Kachru and T.~Weigand,
%``D-Brane Instantons in Type II Orientifolds,''
Ann. Rev. Nucl. Part. Sci. \textbf{59} (2009), 269-296
doi:10.1146/annurev.nucl.010909.083113
[arXiv:0902.3251 [hep-th]].
%239 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Burgess:2020qsc}
\bibitem{Burgess:2020qsc}
C.~P.~Burgess, M.~Cicoli, D.~Ciupke, S.~Krippendorf and F.~Quevedo,
%``UV Shadows in EFTs: Accidental Symmetries, Robustness and No-Scale Supergravity,''
Fortsch. Phys. \textbf{68} (2020) no.10, 2000076
doi:10.1002/prop.202000076
[arXiv:2006.06694 [hep-th]].
%16 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2021rub}
\bibitem{Cicoli:2021rub}
M.~Cicoli, F.~Quevedo, R.~Savelli, A.~Schachner and R.~Valandro,
%``Systematics of the $\alpha'$ Expansion in F-Theory,''
JHEP \textbf{2021} (2021), 99
doi:10.1007/JHEP08(2021)099
[arXiv:2106.04592 [hep-th]].
%6 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Maldacena:2000mw}
\bibitem{Maldacena:2000mw}
J.~M.~Maldacena and C.~Nunez,
%``Supergravity description of field theories on curved manifolds and a no go theorem,''
Int. J. Mod. Phys. A \textbf{16} (2001), 822-855
doi:10.1142/S0217751X01003937
[arXiv:hep-th/0007018 [hep-th]].
%1029 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Green:2011cn}
\bibitem{Green:2011cn}
S.~R.~Green, E.~J.~Martinec, C.~Quigley and S.~Sethi,
%``Constraints on String Cosmology,''
Class. Quant. Grav. \textbf{29} (2012), 075006
doi:10.1088/0264-9381/29/7/075006
[arXiv:1110.0545 [hep-th]].
%70 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Gautason:2012tb}
\bibitem{Gautason:2012tb}
F.~F.~Gautason, D.~Junghans and M.~Zagermann,
%``On Cosmological Constants from alpha'-Corrections,''
JHEP \textbf{06} (2012), 029
doi:10.1007/JHEP06(2012)029
[arXiv:1204.0807 [hep-th]].
%48 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Dasgupta:2014pma}
\bibitem{Dasgupta:2014pma}
K.~Dasgupta, R.~Gwyn, E.~McDonough, M.~Mia and R.~Tatar,
%``de Sitter Vacua in Type IIB String Theory: Classical Solutions and Quantum Corrections,''
JHEP \textbf{07} (2014), 054
doi:10.1007/JHEP07(2014)054
[arXiv:1402.5112 [hep-th]].
%64 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Kutasov:2015eba}
\bibitem{Kutasov:2015eba}
D.~Kutasov, T.~Maxfield, I.~Melnikov and S.~Sethi,
%``Constraining de Sitter Space in String Theory,''
Phys. Rev. Lett. \textbf{115} (2015) no.7, 071305
doi:10.1103/PhysRevLett.115.071305
[arXiv:1504.00056 [hep-th]].
%75 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Quigley:2015jia}
\bibitem{Quigley:2015jia}
C.~Quigley,
%``Gaugino Condensation and the Cosmological Constant,''
JHEP \textbf{06} (2015), 104
doi:10.1007/JHEP06(2015)104
[arXiv:1504.00652 [hep-th]].
%38 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Dine:2020vmr}
\bibitem{Dine:2020vmr}
M.~Dine, J.~A.~P.~Law-Smith, S.~Sun, D.~Wood and Y.~Yu,
%``Obstacles to Constructing de Sitter Space in String Theory,''
JHEP \textbf{02} (2021), 050
doi:10.1007/JHEP02(2021)050
[arXiv:2008.12399 [hep-th]].
%8 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Montero:2020rpl}
\bibitem{Montero:2020rpl}
M.~Montero, T.~Van Riet and G.~Venken,
%``A dS obstruction and its phenomenological consequences,''
JHEP \textbf{05} (2020), 114
doi:10.1007/JHEP05(2020)114
[arXiv:2001.11023 [hep-th]].
%13 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cunillera:2021fbc}
\bibitem{Cunillera:2021fbc}
F.~Cunillera, W.~T.~Emond, A.~Leh\'ebel and A.~Padilla,
%``Quadratic curvature corrections to stringy effective actions and the absence of de Sitter vacua,''
[arXiv:2112.05771 [hep-th]].
%1 citations counted in INSPIRE as of 03 Jan 2022

%\cite{Bedroya:2019snp}
\bibitem{Bedroya:2019snp}
A.~Bedroya and C.~Vafa,
%``Trans-Planckian Censorship and the Swampland,''
JHEP \textbf{09} (2020), 123
doi:10.1007/JHEP09(2020)123
[arXiv:1909.11063 [hep-th]].
%202 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Zlatev:1998tr}
\bibitem{Zlatev:1998tr}
I.~Zlatev, L.~M.~Wang and P.~J.~Steinhardt,
%``Quintessence, cosmic coincidence, and the cosmological constant,''
Phys. Rev. Lett. \textbf{82} (1999), 896-899
doi:10.1103/PhysRevLett.82.896
[arXiv:astro-ph/9807002 [astro-ph]].
%2193 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Velten:2014nra}
\bibitem{Velten:2014nra}
H.~E.~S.~Velten, R.~F.~vom Marttens and W.~Zimdahl,
%``Aspects of the cosmological \textquotedblleft{}coincidence problem\textquotedblright{},''
Eur. Phys. J. C \textbf{74} (2014) no.11, 3160
doi:10.1140/epjc/s10052-014-3160-4
[arXiv:1410.2509 [astro-ph.CO]].
%113 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Cunillera:2021izz}
\bibitem{Cunillera:2021izz}
F.~Cunillera and A.~Padilla,
%``A stringy perspective on the coincidence problem,''
JHEP \textbf{10} (2021), 055
doi:10.1007/JHEP10(2021)055
[arXiv:2105.03426 [hep-th]].
%4 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2021fsd}
\bibitem{Cicoli:2021fsd}
M.~Cicoli, F.~Cunillera, A.~Padilla and F.~G.~Pedro,
%``Quintessence and the Swampland: The parametrically controlled regime of moduli space,''
[arXiv:2112.10779 [hep-th]].
%0 citations counted in INSPIRE as of 29 Dec 2021

%\cite{Hertzberg:2007wc}
\bibitem{Hertzberg:2007wc}
M.~P.~Hertzberg, S.~Kachru, W.~Taylor and M.~Tegmark,
%``Inflationary Constraints on Type IIA String Theory,''
JHEP \textbf{12} (2007), 095
doi:10.1088/1126-6708/2007/12/095
[arXiv:0711.2512 [hep-th]].
%216 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Garg:2018zdg}
\bibitem{Garg:2018zdg}
S.~K.~Garg, C.~Krishnan and M.~Zaid Zaz,
%``Bounds on Slow Roll at the Boundary of the Landscape,''
JHEP \textbf{03} (2019), 029
doi:10.1007/JHEP03(2019)029
[arXiv:1810.09406 [hep-th]].
%71 citations counted in INSPIRE as of 22 Dec 2021

%\cite{ValeixoBento:2020ujr}
\bibitem{ValeixoBento:2020ujr}
B.~Valeixo Bento, D.~Chakraborty, S.~L.~Parameswaran and I.~Zavala,
%``Dark Energy in String Theory,''
PoS \textbf{CORFU2019} (2020), 123
doi:10.22323/1.376.0123
[arXiv:2005.10168 [hep-th]].
%6 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2020cfj}
\bibitem{Cicoli:2020cfj}
M.~Cicoli, G.~Dibitetto and F.~G.~Pedro,
%``New accelerating solutions in late-time cosmology,''
Phys. Rev. D \textbf{101} (2020) no.10, 103524
doi:10.1103/PhysRevD.101.103524
[arXiv:2002.02695 [gr-qc]].
%12 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2020noz}
\bibitem{Cicoli:2020noz}
M.~Cicoli, G.~Dibitetto and F.~G.~Pedro,
%``Out of the Swampland with Multifield Quintessence?,''
JHEP \textbf{10} (2020), 035
doi:10.1007/JHEP10(2020)035
[arXiv:2007.11011 [hep-th]].
%16 citations counted in INSPIRE as of 22 Dec 2021

\bibitem{BCDP}
M.~Brinkmann, M.~Cicoli, G.~Dibitetto and F. ~G.~Pedro,
To appear

%\cite{Cicoli:2018kdo}
\bibitem{Cicoli:2018kdo}
M.~Cicoli, S.~De Alwis, A.~Maharana, F.~Muia and F.~Quevedo,
%``De Sitter vs Quintessence in String Theory,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800079
doi:10.1002/prop.201800079
[arXiv:1808.08967 [hep-th]].
%139 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Hebecker:2019csg}
\bibitem{Hebecker:2019csg}
A.~Hebecker, T.~Skrzypek and M.~Wittner,
%``The $F$-term Problem and other Challenges of Stringy Quintessence,''
JHEP \textbf{11} (2019), 134
doi:10.1007/JHEP11(2019)134
[arXiv:1909.08625 [hep-th]].
%18 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Will:2014kxa}
\bibitem{Will:2014kxa}
C.~M.~Will,
%``The Confrontation between General Relativity and Experiment,''
Living Rev. Rel. \textbf{17} (2014), 4
doi:10.12942/lrr-2014-4
[arXiv:1403.7377 [gr-qc]].
%1609 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Colgain:2019joh}
\bibitem{Colgain:2019joh}
E.~\'O.~Colg\'ain and H.~Yavartanoo,
%``Testing the Swampland: $H_0$ tension,''
Phys. Lett. B \textbf{797} (2019), 134907
doi:10.1016/j.physletb.2019.134907
[arXiv:1905.02555 [astro-ph.CO]].
%45 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Banerjee:2020xcn}
\bibitem{Banerjee:2020xcn}
A.~Banerjee, H.~Cai, L.~Heisenberg, E.~\'O.~Colg\'ain, M.~M.~Sheikh-Jabbari and T.~Yang,
%``Hubble sinks in the low-redshift swampland,''
Phys. Rev. D \textbf{103} (2021) no.8, L081305
doi:10.1103/PhysRevD.103.L081305
[arXiv:2006.00244 [astro-ph.CO]].
%57 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Riess:2021jrx}
\bibitem{Riess:2021jrx}
A.~G.~Riess, W.~Yuan, L.~M.~Macri, D.~Scolnic, D.~Brout, S.~Casertano, D.~O.~Jones, Y.~Murakami, L.~Breuval and T.~G.~Brink, \textit{et al.}
%``A Comprehensive Measurement of the Local Value of the Hubble Constant with 1 km/s/Mpc Uncertainty from the Hubble Space Telescope and the SH0ES Team,''
[arXiv:2112.04510 [astro-ph.CO]].
%18 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Kallosh:2004yh}
\bibitem{Kallosh:2004yh}
R.~Kallosh and A.~D.~Linde,
%``Landscape, the scale of SUSY breaking, and inflation,''
JHEP \textbf{12} (2004), 004
doi:10.1088/1126-6708/2004/12/004
[arXiv:hep-th/0411011 [hep-th]].
%289 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2015wja}
\bibitem{Cicoli:2015wja}
M.~Cicoli, F.~Muia and F.~G.~Pedro,
%``Microscopic Origin of Volume Modulus Inflation,''
JCAP \textbf{12} (2015), 040
doi:10.1088/1475-7516/2015/12/040
[arXiv:1509.07748 [hep-th]].
%13 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2012tz}
\bibitem{Cicoli:2012tz}
M.~Cicoli, F.~G.~Pedro and G.~Tasinato,
%``Natural Quintessence in String Theory,''
JCAP \textbf{07} (2012), 044
doi:10.1088/1475-7516/2012/07/044
[arXiv:1203.6655 [hep-th]].
%47 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Akrami:2018ylq}
\bibitem{Akrami:2018ylq}
Y.~Akrami, R.~Kallosh, A.~Linde and V.~Vardanyan,
%``The Landscape, the Swampland and the Era of Precision Cosmology,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800075
doi:10.1002/prop.201800075
[arXiv:1808.09440 [hep-th]].
%198 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Agrawal:2018own}
\bibitem{Agrawal:2018own}
P.~Agrawal, G.~Obied, P.~J.~Steinhardt and C.~Vafa,
%``On the Cosmological Implications of the String Swampland,''
Phys. Lett. B \textbf{784} (2018), 271-276
doi:10.1016/j.physletb.2018.07.040
[arXiv:1806.09718 [hep-th]].
%367 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Ferrer:1997yz}
\bibitem{Ferrer:1997yz}
F.~Ferrer and J.~A.~Grifols,
%``Constraints on the mass of the superlight gravitino from the muon anomaly,''
Phys. Rev. D \textbf{56} (1997), 7466-7468
doi:10.1103/PhysRevD.56.7466
[arXiv:hep-ph/9704444 [hep-ph]].
%10 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Brignole:1997sk}
\bibitem{Brignole:1997sk}
A.~Brignole, F.~Feruglio and F.~Zwirner,
%``Signals of a superlight gravitino at $e^+ e^-$ colliders when the other superparticles are heavy,''
Nucl. Phys. B \textbf{516} (1998), 13-28
[erratum: Nucl. Phys. B \textbf{555} (1999), 653-655]
doi:10.1016/S0550-3213(97)00825-0
[arXiv:hep-ph/9711516 [hep-ph]].
%99 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Brignole:1998me}
\bibitem{Brignole:1998me}
A.~Brignole, F.~Feruglio, M.~L.~Mangano and F.~Zwirner,
%``Signals of a superlight gravitino at hadron colliders when the other superparticles are heavy,''
Nucl. Phys. B \textbf{526} (1998), 136-152
[erratum: Nucl. Phys. B \textbf{582} (2000), 759-761]
doi:10.1016/S0550-3213(98)00254-5
[arXiv:hep-ph/9801329 [hep-ph]].
%93 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Kawasaki:2008qe}
\bibitem{Kawasaki:2008qe}
M.~Kawasaki, K.~Kohri, T.~Moroi and A.~Yotsuyanagi,
%``Big-Bang Nucleosynthesis and Gravitino,''
Phys. Rev. D \textbf{78} (2008), 065011
doi:10.1103/PhysRevD.78.065011
[arXiv:0804.3745 [hep-ph]].
%457 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Burgess:2014tja}
\bibitem{Burgess:2014tja}
C.~P.~Burgess, M.~Cicoli, F.~Quevedo and M.~Williams,
%``Inflating with Large Effective Fields,''
JCAP \textbf{11} (2014), 045
doi:10.1088/1475-7516/2014/11/045
[arXiv:1404.6236 [hep-th]].
%44 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Burgess:2016owb}
\bibitem{Burgess:2016owb}
C.~P.~Burgess, M.~Cicoli, S.~de Alwis and F.~Quevedo,
%``Robust Inflation from Fibrous Strings,''
JCAP \textbf{05} (2016), 032
doi:10.1088/1475-7516/2016/05/032
[arXiv:1603.06789 [hep-th]].
%55 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2012sz}
\bibitem{Cicoli:2012sz}
M.~Cicoli, M.~Goodsell and A.~Ringwald,
%``The type IIB string axiverse and its low-energy phenomenology,''
JHEP \textbf{10} (2012), 146
doi:10.1007/JHEP10(2012)146
[arXiv:1206.0819 [hep-th]].
%339 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Arkani-Hamed:2006emk}
\bibitem{Arkani-Hamed:2006emk}
N.~Arkani-Hamed, L.~Motl, A.~Nicolis and C.~Vafa,
%``The String landscape, black holes and gravity as the weakest force,''
JHEP \textbf{06} (2007), 060
doi:10.1088/1126-6708/2007/06/060
[arXiv:hep-th/0601001 [hep-th]].
%909 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Kim:2004rp}
\bibitem{Kim:2004rp}
J.~E.~Kim, H.~P.~Nilles and M.~Peloso,
%``Completing natural inflation,''
JCAP \textbf{01} (2005), 005
doi:10.1088/1475-7516/2005/01/005
[arXiv:hep-ph/0409138 [hep-ph]].
%461 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Dimopoulos:2005ac}
\bibitem{Dimopoulos:2005ac}
S.~Dimopoulos, S.~Kachru, J.~McGreevy and J.~G.~Wacker,
%``N-flation,''
JCAP \textbf{08} (2008), 003
doi:10.1088/1475-7516/2008/08/003
[arXiv:hep-th/0507205 [hep-th]].
%579 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Kaloper:2005aj}
\bibitem{Kaloper:2005aj}
N.~Kaloper and L.~Sorbo,
%``Of pngb quintessence,''
JCAP \textbf{04} (2006), 007
doi:10.1088/1475-7516/2006/04/007
[arXiv:astro-ph/0511543 [astro-ph]].
%55 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Blanco-Pillado:2004aap}
\bibitem{Blanco-Pillado:2004aap}
J.~J.~Blanco-Pillado, C.~P.~Burgess, J.~M.~Cline, C.~Escoda, M.~Gomez-Reino, R.~Kallosh, A.~D.~Linde and F.~Quevedo,
%``Racetrack inflation,''
JHEP \textbf{11} (2004), 063
doi:10.1088/1126-6708/2004/11/063
[arXiv:hep-th/0406230 [hep-th]].
%270 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Choi:1999xn}
\bibitem{Choi:1999xn}
K.~Choi,
%``String or M theory axion as a quintessence,''
Phys. Rev. D \textbf{62} (2000), 043509
doi:10.1103/PhysRevD.62.043509
[arXiv:hep-ph/9902292 [hep-ph]].
%161 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Kaloper:2008qs}
\bibitem{Kaloper:2008qs}
N.~Kaloper and L.~Sorbo,
%``Where in the String Landscape is Quintessence,''
Phys. Rev. D \textbf{79} (2009), 043528
doi:10.1103/PhysRevD.79.043528
[arXiv:0810.5346 [hep-th]].
%61 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Panda:2010uq}
\bibitem{Panda:2010uq}
S.~Panda, Y.~Sumitomo and S.~P.~Trivedi,
%``Axions as Quintessence in String Theory,''
Phys. Rev. D \textbf{83} (2011), 083506
doi:10.1103/PhysRevD.83.083506
[arXiv:1011.5877 [hep-th]].
%70 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Kamionkowski:2014zda}
\bibitem{Kamionkowski:2014zda}
M.~Kamionkowski, J.~Pradler and D.~G.~E.~Walker,
%``Dark energy from the string axiverse,''
Phys. Rev. Lett. \textbf{113} (2014) no.25, 251302
doi:10.1103/PhysRevLett.113.251302
[arXiv:1409.0549 [hep-ph]].
%62 citations counted in INSPIRE as of 23 Dec 2021

%\cite{Olguin-Trejo:2018zun}
\bibitem{Olguin-Trejo:2018zun}
Y.~Olguin-Trejo, S.~L.~Parameswaran, G.~Tasinato and I.~Zavala,
%``Runaway Quintessence, Out of the Swampland,''
JCAP \textbf{01} (2019), 031
doi:10.1088/1475-7516/2019/01/031
[arXiv:1810.08634 [hep-th]].
%49 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Zyla:2020zbs}
\bibitem{Zyla:2020zbs}
P.~A.~Zyla \textit{et al.} [Particle Data Group],
%``Review of Particle Physics,''
PTEP \textbf{2020} (2020) no.8, 083C01
doi:10.1093/ptep/ptaa104
%2583 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Kapner:2006si}
\bibitem{Kapner:2006si}
D.~J.~Kapner, T.~S.~Cook, E.~G.~Adelberger, J.~H.~Gundlach, B.~R.~Heckel, C.~D.~Hoyle and H.~E.~Swanson,
%``Tests of the gravitational inverse-square law below the dark-energy length scale,''
Phys. Rev. Lett. \textbf{98} (2007), 021101
doi:10.1103/PhysRevLett.98.021101
[arXiv:hep-ph/0611184 [hep-ph]].
%781 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Damour:2010rp}
\bibitem{Damour:2010rp}
T.~Damour and J.~F.~Donoghue,
%``Equivalence Principle Violations and Couplings of a Light Dilaton,''
Phys. Rev. D \textbf{82} (2010), 084033
doi:10.1103/PhysRevD.82.084033
[arXiv:1007.2792 [gr-qc]].
%128 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Acharya:2018deu}
\bibitem{Acharya:2018deu}
B.~S.~Acharya, A.~Maharana and F.~Muia,
%``Hidden Sectors in String Theory: Kinetic Mixings, Fifth Forces and Quintessence,''
JHEP \textbf{03} (2019), 048
doi:10.1007/JHEP03(2019)048
[arXiv:1811.10633 [hep-th]].
%28 citations counted in INSPIRE as of 23 Dec 2021

%\cite{Cicoli:2011yy}
\bibitem{Cicoli:2011yy}
M.~Cicoli, C.~P.~Burgess and F.~Quevedo,
%``Anisotropic Modulus Stabilisation: Strings at LHC Scales with Micron-sized Extra Dimensions,''
JHEP \textbf{10} (2011), 119
doi:10.1007/JHEP10(2011)119
[arXiv:1105.2107 [hep-th]].
%76 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Burgess:2021qti}
\bibitem{Burgess:2021qti}
C.~P.~Burgess and F.~Quevedo,
%``Axion Homeopathy: Screening Dilaton Interactions,''
[arXiv:2110.10352 [hep-th]].
%4 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Burgess:2021obw}
\bibitem{Burgess:2021obw}
C.~P.~Burgess, D.~Dineen and F.~Quevedo,
%``Yoga Dark Energy: Natural Relaxation and Other Dark Implications of a Supersymmetric Gravity Sector,''
[arXiv:2111.07286 [hep-th]].
%1 citations counted in INSPIRE as of 29 Dec 2021

%\cite{Buchmuller:2004tz}
\bibitem{Buchmuller:2004tz}
W.~Buchmuller, K.~Hamaguchi, O.~Lebedev and M.~Ratz,
%``Maximal temperature in flux compactifications,''
JCAP \textbf{01} (2005), 004
doi:10.1088/1475-7516/2005/01/004
[arXiv:hep-th/0411109 [hep-th]].
%39 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Anguelova:2009ht}
\bibitem{Anguelova:2009ht}
L.~Anguelova, V.~Calo and M.~Cicoli,
%``LARGE Volume String Compactifications at Finite Temperature,''
JCAP \textbf{10} (2009), 025
doi:10.1088/1475-7516/2009/10/025
[arXiv:0904.0051 [hep-th]].
%35 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Conlon:2008cj}
\bibitem{Conlon:2008cj}
J.~P.~Conlon, R.~Kallosh, A.~D.~Linde and F.~Quevedo,
%``Volume Modulus Inflation and the Gravitino Mass Problem,''
JCAP \textbf{09} (2008), 011
doi:10.1088/1475-7516/2008/09/011
[arXiv:0806.0809 [hep-th]].
%100 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Westphal:2006tn}
\bibitem{Westphal:2006tn}
A.~Westphal,
%``de Sitter string vacua from Kahler uplifting,''
JHEP \textbf{03} (2007), 102
doi:10.1088/1126-6708/2007/03/102
[arXiv:hep-th/0611332 [hep-th]].
%147 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Hsu:2003cy}
\bibitem{Hsu:2003cy}
J.~P.~Hsu, R.~Kallosh and S.~Prokushkin,
%``On brane inflation with volume stabilization,''
JCAP \textbf{12} (2003), 009
doi:10.1088/1475-7516/2003/12/009
[arXiv:hep-th/0311077 [hep-th]].
%153 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Aparicio:2014wxa}
\bibitem{Aparicio:2014wxa}
L.~Aparicio, M.~Cicoli, S.~Krippendorf, A.~Maharana, F.~Muia and F.~Quevedo,
%``Sequestered de Sitter String Scenarios: Soft-terms,''
JHEP \textbf{11} (2014), 071
doi:10.1007/JHEP11(2014)071
[arXiv:1409.1931 [hep-th]].
%59 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Pitrou:2018cgg}
\bibitem{Pitrou:2018cgg}
C.~Pitrou, A.~Coc, J.~P.~Uzan and E.~Vangioni,
%``Precision big bang nucleosynthesis with improved Helium-4 predictions,''
Phys. Rept. \textbf{754} (2018), 1-66
doi:10.1016/j.physrep.2018.04.005
[arXiv:1801.08023 [astro-ph.CO]].
%175 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Davidson:2000dw}
\bibitem{Davidson:2000dw}
S.~Davidson, M.~Losada and A.~Riotto,
%``A New perspective on baryogenesis,''
Phys. Rev. Lett. \textbf{84} (2000), 4284-4287
doi:10.1103/PhysRevLett.84.4284
[arXiv:hep-ph/0001301 [hep-ph]].
%91 citations counted in INSPIRE as of 22 Dec 2021

%\cite{He:2010uk}
\bibitem{He:2010uk}
T.~He, S.~Kachru and A.~Westphal,
%``Gravity waves and the LHC: Towards high-scale inflation with low-energy SUSY,''
JHEP \textbf{06} (2010), 065
doi:10.1007/JHEP06(2010)065
[arXiv:1003.4265 [hep-th]].
%29 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Hellerman:2001yi}
\bibitem{Hellerman:2001yi}
S.~Hellerman, N.~Kaloper and L.~Susskind,
%``String theory and quintessence,''
JHEP \textbf{06} (2001), 003
doi:10.1088/1126-6708/2001/06/003
[arXiv:hep-th/0104180 [hep-th]].
%307 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2011it}
\bibitem{Cicoli:2011it}
M.~Cicoli, M.~Kreuzer and C.~Mayrhofer,
%``Toric K3-Fibred Calabi-Yau Manifolds with del Pezzo Divisors for String Compactifications,''
JHEP \textbf{02} (2012), 002
doi:10.1007/JHEP02(2012)002
[arXiv:1107.0383 [hep-th]].
%57 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2018tcq}
\bibitem{Cicoli:2018tcq}
M.~Cicoli, D.~Ciupke, C.~Mayrhofer and P.~Shukla,
%``A Geometrical Upper Bound on the Inflaton Range,''
JHEP \textbf{05} (2018), 001
doi:10.1007/JHEP05(2018)001
[arXiv:1801.05434 [hep-th]].
%61 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2015ylx}
\bibitem{Cicoli:2015ylx}
M.~Cicoli, F.~Quevedo and R.~Valandro,
%``De Sitter from T-branes,''
JHEP \textbf{03} (2016), 141
doi:10.1007/JHEP03(2016)141
[arXiv:1512.04558 [hep-th]].
%90 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2011qg}
\bibitem{Cicoli:2011qg}
M.~Cicoli, C.~Mayrhofer and R.~Valandro,
%``Moduli Stabilisation for Chiral Global Models,''
JHEP \textbf{02} (2012), 062
doi:10.1007/JHEP02(2012)062
[arXiv:1110.3333 [hep-th]].
%84 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2013mpa}
\bibitem{Cicoli:2013mpa}
M.~Cicoli, S.~Krippendorf, C.~Mayrhofer, F.~Quevedo and R.~Valandro,
%``D3/D7 Branes at Singularities: Constraints from Global Embedding and Moduli Stabilisation,''
JHEP \textbf{07} (2013), 150
doi:10.1007/JHEP07(2013)150
[arXiv:1304.0022 [hep-th]].
%54 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Cicoli:2017shd}
\bibitem{Cicoli:2017shd}
M.~Cicoli, I.~Garc\`\i{}a-Etxebarria, C.~Mayrhofer, F.~Quevedo, P.~Shukla and R.~Valandro,
%``Global Orientifolded Quivers with Inflation,''
JHEP \textbf{11} (2017), 134
doi:10.1007/JHEP11(2017)134
[arXiv:1706.06128 [hep-th]].
%33 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Danielsson:2018ztv}
\bibitem{Danielsson:2018ztv}
U.~H.~Danielsson and T.~Van Riet,
%``What if string theory has no de Sitter vacua?,''
Int. J. Mod. Phys. D \textbf{27} (2018) no.12, 1830007
doi:10.1142/S0218271818300070
[arXiv:1804.01120 [hep-th]].
%258 citations counted in INSPIRE as of 05 Jan 2022

%\cite{Cicoli:2021tzt}
\bibitem{Cicoli:2021tzt}
M.~Cicoli, A.~Schachner and P.~Shukla,
%``Systematics of type IIB moduli stabilisation with odd axions,''
[arXiv:2109.14624 [hep-th]].
%7 citations counted in INSPIRE as of 30 Dec 2021

%\cite{Cicoli:2021gss}
\bibitem{Cicoli:2021gss}
M.~Cicoli, V.~Guidetti, N.~Righi and A.~Westphal,
%``Fuzzy Dark Matter Candidates from String Theory,''
[arXiv:2110.02964 [hep-th]].
%2 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Shelton:2005cf}
\bibitem{Shelton:2005cf}
J.~Shelton, W.~Taylor and B.~Wecht,
%``Nongeometric flux compactifications,''
JHEP \textbf{10} (2005), 085
doi:10.1088/1126-6708/2005/10/085
[arXiv:hep-th/0508133 [hep-th]].
%412 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Benmachiche:2006df}
\bibitem{Benmachiche:2006df}
I.~Benmachiche and T.~W.~Grimm,
%``Generalized N=1 orientifold compactifications and the Hitchin functionals,''
Nucl. Phys. B \textbf{748} (2006), 200-252
doi:10.1016/j.nuclphysb.2006.05.003
[arXiv:hep-th/0602241 [hep-th]].
%143 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Plauschinn:2018wbo}
\bibitem{Plauschinn:2018wbo}
E.~Plauschinn,
%``Non-geometric backgrounds in string theory,''
Phys. Rept. \textbf{798} (2019), 1-122
doi:10.1016/j.physrep.2018.12.002
[arXiv:1811.11203 [hep-th]].
%60 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Scherrer:2007pu}
\bibitem{Scherrer:2007pu}
R.~J.~Scherrer and A.~A.~Sen,
%``Thawing quintessence with a nearly flat potential,''
Phys. Rev. D \textbf{77} (2008), 083515
doi:10.1103/PhysRevD.77.083515
[arXiv:0712.3450 [astro-ph]].
%167 citations counted in INSPIRE as of 23 Dec 2021

%\cite{Dutta:2008qn}
\bibitem{Dutta:2008qn}
S.~Dutta and R.~J.~Scherrer,
%``Hilltop Quintessence,''
Phys. Rev. D \textbf{78} (2008), 123525
doi:10.1103/PhysRevD.78.123525
[arXiv:0809.4441 [astro-ph]].
%79 citations counted in INSPIRE as of 23 Dec 2021

%\cite{Hardwick:2017fjo}
\bibitem{Hardwick:2017fjo}
R.~J.~Hardwick, V.~Vennin, C.~T.~Byrnes, J.~Torrado and D.~Wands,
%``The stochastic spectator,''
JCAP \textbf{10} (2017), 018
doi:10.1088/1475-7516/2017/10/018
[arXiv:1701.06473 [astro-ph.CO]].
%51 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Uhlenbeck:1930zz}
\bibitem{Uhlenbeck:1930zz}
G.~E.~Uhlenbeck and L.~S.~Ornstein,
%``On the Theory of the Brownian Motion,''
Phys. Rev. \textbf{36} (1930), 823-841
doi:10.1103/PhysRev.36.823
%151 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Perlmutter:1998np}
\bibitem{Perlmutter:1998np}
S.~Perlmutter \textit{et al.} [Supernova Cosmology Project],
%``Measurements of $\Omega$ and $\Lambda$ from 42 high redshift supernovae,''
Astrophys. J. \textbf{517} (1999), 565-586
doi:10.1086/307221
[arXiv:astro-ph/9812133 [astro-ph]].
%13792 citations counted in INSPIRE as of 06 Jan 2022

%\cite{SupernovaSearchTeam:1998fmf}
\bibitem{SupernovaSearchTeam:1998fmf}
A.~G.~Riess \textit{et al.} [Supernova Search Team],
%``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
Astron. J. \textbf{116} (1998), 1009-1038
doi:10.1086/300499
[arXiv:astro-ph/9805201 [astro-ph]].
%13829 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Aghanim:2018eyx}
\bibitem{Aghanim:2018eyx}
N.~Aghanim \textit{et al.} [Planck],
%``Planck 2018 results. VI. Cosmological parameters,''
Astron. Astrophys. \textbf{641} (2020), A6
[erratum: Astron. Astrophys. \textbf{652} (2021), C4]
doi:10.1051/0004-6361/201833910
[arXiv:1807.06209 [astro-ph.CO]].
%6700 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Weinberg:1987dv}
\bibitem{Weinberg:1987dv}
S.~Weinberg,
%``Anthropic Bound on the Cosmological Constant,''
Phys. Rev. Lett. \textbf{59} (1987), 2607
doi:10.1103/PhysRevLett.59.2607
%971 citations counted in INSPIRE as of 06 Jan 2022

%\cite{Niedermann:2017cel}
\bibitem{Niedermann:2017cel}
F.~Niedermann and A.~Padilla,
%``Gravitational Mechanisms to Self-Tune the Cosmological Constant: Obstructions and Ways Forward,''
Phys. Rev. Lett. \textbf{119} (2017) no.25, 251306
doi:10.1103/PhysRevLett.119.251306
[arXiv:1706.04778 [hep-th]].
%15 citations counted in INSPIRE as of 22 Dec 2021

%\cite{Copeland:2021czt}
\bibitem{Copeland:2021czt}
E.~J.~Copeland, S.~Ghataore, F.~Niedermann and A.~Padilla,
%``Generalised scalar-tensor theories and self-tuning,''
[arXiv:2111.11448 [gr-qc]].
%1 citations counted in INSPIRE as of 22 Dec 2021

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF CHAPTER 8 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% CHAPTER 9 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cite{Perlmutter:1998np}
\bibitem{SN1}
S.~Perlmutter \textit{et al.} [Supernova Cosmology Project],
%``Measurements of $\Omega$ and $\Lambda$ from 42 high redshift supernovae,''
Astrophys. J. \textbf{517} (1999), 565-586
%doi:10.1086/307221
[arXiv:astro-ph/9812133 [astro-ph]].
%12981 citations counted in INSPIRE as of 17 Dec 2020
%\cite{Perlmutter:1998np}
\bibitem{SN2}
  A.~G.~Riess {\it et al.} [Supernova Search Team],
  %``Observational evidence from supernovae for an accelerating universe and a cosmological constant,''
  Astron.\ J.\  {\bf 116} (1998) 1009
%  doi:10.1086/300499
  [astro-ph/9805201].
  %%CITATION = doi:10.1086/300499;%%
  %11582 citations counted in INSPIRE as of 24 Jul 2019
%\cite{Riess:2019cxk}

%\cite{Aghanim:2018eyx}
\bibitem{CMB}
  N.~Aghanim {\it et al.} [Planck Collaboration],
  %``Planck 2018 results. VI. Cosmological parameters,''
  arXiv:1807.06209 [astro-ph.CO].
  %%CITATION = ARXIV:1807.06209;%%
  %1183 citations counted in INSPIRE as of 24 Jul 2019
  
  %\cite{Copeland:2006wr}
\bibitem{derev}
  E.~J.~Copeland, M.~Sami and S.~Tsujikawa,
  %``Dynamics of dark energy,''
  Int.\ J.\ Mod.\ Phys.\ D {\bf 15} (2006) 1753
 % doi:10.1142/S021827180600942X
  [hep-th/0603057].
  %%CITATION = doi:10.1142/S021827180600942X;%%
  %3887 citations counted in INSPIRE as of 24 Jul 2019
 
 %\cite{deSitter:1917zz}
\bibitem{dS}
W.~de Sitter,
%``Einstein's theory of gravitation and its astronomical consequences, Third Paper,''
Mon. Not. Roy. Astron. Soc. \textbf{78} (1917), 3-28
%218 citations counted in INSPIRE as of 17 Dec 2020 
  
  %\cite{Peebles:1987ek}
\bibitem{quin1a}
P.~J.~E.~Peebles and B.~Ratra,
%``Cosmology with a Time Variable Cosmological Constant,''
Astrophys. J. Lett. \textbf{325} (1988), L17
%doi:10.1086/185100
%1593 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Ratra:1987rm}
\bibitem{quin1b}
B.~Ratra and P.~J.~E.~Peebles,
%``Cosmological Consequences of a Rolling Homogeneous Scalar Field,''
Phys. Rev. D \textbf{37} (1988), 3406
%doi:10.1103/PhysRevD.37.3406
%3734 citations counted in INSPIRE as of 17 Dec 2020
  
  %\cite{Caldwell:1997ii}
\bibitem{quin2}
R.~R.~Caldwell, R.~Dave and P.~J.~Steinhardt,
%``Cosmological imprint of an energy component with general equation of state,''
Phys. Rev. Lett. \textbf{80} (1998), 1582-1585
%doi:10.1103/PhysRevLett.80.1582
[arXiv:astro-ph/9708069 [astro-ph]].
%2939 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Kachru:2003aw}
\bibitem{Kachru:2003aw}
S.~Kachru, R.~Kallosh, A.~D.~Linde and S.~P.~Trivedi,
%``De Sitter vacua in string theory,''
Phys. Rev. D \textbf{68} (2003), 046005
%doi:10.1103/PhysRevD.68.046005
[arXiv:hep-th/0301240 [hep-th]].
%3051 citations counted in INSPIRE as of 16 Nov 2021

%\cite{hep-th/0502058}
\bibitem{hep-th/0502058}
V.~Balasubramanian, P.~Berglund, J.~P.~Conlon and F.~Quevedo,
%``Systematics of moduli stabilisation in Calabi-Yau flux compactifications,''
JHEP \textbf{03} (2005), 007
%doi:10.1088/1126-6708/2005/03/007
[arXiv:hep-th/0502058 [hep-th]].
%906 citations counted in INSPIRE as of 16 Nov 2021

%\cite{Cicoli:2007xp}
\bibitem{Cicoli:2007xp}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``Systematics of String Loop Corrections in Type IIB Calabi-Yau Flux Compactifications,''
JHEP \textbf{01} (2008), 052
%doi:10.1088/1126-6708/2008/01/052
[arXiv:0708.1873 [hep-th]].
%176 citations counted in INSPIRE as of 16 Nov 2021

%\cite{Cicoli:2008va}
\bibitem{Cicoli:2008va}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``General Analysis of LARGE Volume Scenarios with String Loop Moduli Stabilisation,''
JHEP \textbf{10} (2008), 105
%doi:10.1088/1126-6708/2008/10/105
[arXiv:0805.1029 [hep-th]].
%165 citations counted in INSPIRE as of 16 Nov 2021

%\cite{Kachru:2019dvo}
\bibitem{Kachru:2019dvo}
S.~Kachru, M.~Kim, L.~Mcallister and M.~Zimet,
%``de Sitter Vacua from Ten Dimensions,''
[arXiv:1908.04788 [hep-th]].
%39 citations counted in INSPIRE as of 16 Nov 2021

%\cite{AbdusSalam:2020ywo}
\bibitem{AbdusSalam:2020ywo}
S.~AbdusSalam, S.~Abel, M.~Cicoli, F.~Quevedo and P.~Shukla,
%``A systematic approach to K\"ahler moduli stabilisation,''
JHEP \textbf{08} (2020) no.08, 047
%doi:10.1007/JHEP08(2020)047
[arXiv:2005.11329 [hep-th]].
%15 citations counted in INSPIRE as of 11 Nov 2021

%\cite{Cicoli:2021rub}
\bibitem{Cicoli:2021rub}
M.~Cicoli, F.~Quevedo, R.~Savelli, A.~Schachner and R.~Valandro,
%``Systematics of the $\alpha'$ Expansion in F-Theory,''
JHEP \textbf{2021} (2021), 99
%doi:10.1007/JHEP08(2021)099
[arXiv:2106.04592 [hep-th]].
%3 citations counted in INSPIRE as of 16 Nov 2021

	%\cite{Cunillera:2021izz}
\bibitem{coin}
F.~Cunillera and A.~Padilla,
%``A stringy perspective on the coincidence problem,''
JHEP \textbf{10} (2021), 055
%doi:10.1007/JHEP10(2021)055
[arXiv:2105.03426 [hep-th]].
%1 citations counted in INSPIRE as of 26 Nov 2021
	%\cite{Garg:2018zdg}
\bibitem{Garg1}
S.~K.~Garg, C.~Krishnan and M.~Zaid Zaz,
%``Bounds on Slow Roll at the Boundary of the Landscape,''
JHEP \textbf{03} (2019), 029
%doi:10.1007/JHEP03(2019)029
[arXiv:1810.09406 [hep-th]].
%67 citations counted in INSPIRE as of 26 Nov 2021
	
	%\cite{ValeixoBento:2020ujr}
\bibitem{ivonne}
B.~Valeixo Bento, D.~Chakraborty, S.~L.~Parameswaran and I.~Zavala,
%``Dark Energy in String Theory,''
PoS \textbf{CORFU2019} (2020), 123
%doi:10.22323/1.376.0123
[arXiv:2005.10168 [hep-th]].
%3 citations counted in INSPIRE as of 26 Nov 2021


	
    \bibitem{no_runaway}
	M.~Cicoli, F.~Cunillera, A.~Padilla and F.~G.~Pedro,
	to appear.


	%\cite{Hebecker:2019csg}
	\bibitem{Hebecker}
	A.~Hebecker, T.~Skrzypek and M.~Wittner,
	%``The $F$-term Problem and other Challenges of Stringy Quintessence,''
	JHEP \textbf{11} (2019), 134
	%doi:10.1007/JHEP11(2019)134
	[arXiv:1909.08625 [hep-th]].
	%10 citations counted in INSPIRE as of 05 Nov 2020
	
		\bibitem{us}
	M.~Cicoli, F.~Cunillera, A.~Padilla and F.~G.~Pedro,
	to appear.

%\cite{col2}
\bibitem{col1}
E.~\'O.~Colg\'ain and H.~Yavartanoo,
%``Testing the Swampland: $H_0$ tension,''
Phys. Lett. B \textbf{797} (2019), 134907
%doi:10.1016/j.physletb.2019.134907
[arXiv:1905.02555 [astro-ph.CO]].
%44 citations counted in INSPIRE as of 15 Dec 2021

%\cite{Banerjee:2020xcn}
\bibitem{col2}
A.~Banerjee, H.~Cai, L.~Heisenberg, E.~\'O.~Colg\'ain, M.~M.~Sheikh-Jabbari and T.~Yang,
%``Hubble sinks in the low-redshift swampland,''
Phys. Rev. D \textbf{103} (2021) no.8, L081305
%doi:10.1103/PhysRevD.103.L081305
[arXiv:2006.00244 [astro-ph.CO]].
%55 citations counted in INSPIRE as of 15 Dec 2021

%\cite{Riess:2021jrx}
\bibitem{5sig}
A.~G.~Riess, W.~Yuan, L.~M.~Macri, D.~Scolnic, D.~Brout, S.~Casertano, D.~O.~Jones, Y.~Murakami, L.~Breuval and T.~G.~Brink, \textit{et al.}
%``A Comprehensive Measurement of the Local Value of the Hubble Constant with 1 km/s/Mpc Uncertainty from the Hubble Space Telescope and the SH0ES Team,''
[arXiv:2112.04510 [astro-ph.CO]].
%4 citations counted in INSPIRE as of 15 Dec 2021

%\cite{Palti:2019pca}
\bibitem{Palti:2019pca}
E.~Palti,
%``The Swampland: Introduction and Review,''
Fortsch. Phys. \textbf{67} (2019) no.6, 1900037
%doi:10.1002/prop.201900037
[arXiv:1903.06239 [hep-th]].
%443 citations counted in INSPIRE as of 16 Nov 2021


	%\cite{Vafa:2005ui}
	\bibitem{Vafa}
	C.~Vafa,
	%``The String landscape and the swampland,''
	[arXiv:hep-th/0509212 [hep-th]].
	%502 citations counted in INSPIRE as of 05 Nov 2020

	%\cite{Obied:2018sgi}
	\bibitem{Obied}
	G.~Obied, H.~Ooguri, L.~Spodyneiko and C.~Vafa,
	%``De Sitter Space and the Swampland,''
	[arXiv:1806.08362 [hep-th]].
	%475 citations counted in INSPIRE as of 05 Nov 2020
	
	\bibitem{Garg:2018reu}
    S.~K.~Garg and C.~Krishnan,
    %``Bounds on Slow Roll and the de Sitter Swampland,''
    JHEP \textbf{11} (2019), 075
    %doi:10.1007/JHEP11(2019)075
    [arXiv:1807.05193 [hep-th]].
    %391 citations counted in INSPIRE as of 13 Nov 2021
	
	%\cite{Danielsson:2018ztv}
	\bibitem{Danielsson}
	U.~H.~Danielsson and T.~Van Riet,
	%``What if string theory has no de Sitter vacua?,''
	Int. J. Mod. Phys. D \textbf{27} (2018) no.12, 1830007
%	doi:10.1142/S0218271818300070
	[arXiv:1804.01120 [hep-th]].
	%201 citations counted in INSPIRE as of 05 Nov 2020
	
	%\cite{Dudas:2015eha}
 \bibitem{Dudas:2015eha} E.~Dudas, S.~Ferrara, A.~Kehagias and A.~Sagnotti, %``Properties of Nilpotent Supergravity,'' 
 JHEP \textbf{09} (2015), 217
 %doi:10.1007/JHEP09(2015)217 
 [arXiv:1507.07842 [hep-th]]. %84 citations counted in INSPIRE as of 10 Dec 2021

%\cite{Bergshoeff:2015tra}
 \bibitem{Bergshoeff:2015tra} E.~A.~Bergshoeff, D.~Z.~Freedman, R.~Kallosh and A.~Van Proeyen, %``Pure de Sitter Supergravity,'' 
 Phys. Rev. D \textbf{92} (2015) no.8, 085040 [erratum: Phys. Rev. D \textbf{93} (2016) no.6, 069901] 
 %doi:10.1103/PhysRevD.93.069901
 [arXiv:1507.08264 [hep-th]]. %116 citations counted in INSPIRE as of 10 Dec 2021
 
 %\cite{Bandos:2015xnf}
 \bibitem{Bandos:2015xnf} I.~Bandos, L.~Martucci, D.~Sorokin and M.~Tonin, %``Brane induced supersymmetry breaking and de Sitter supergravity,'' 
 JHEP \textbf{02} (2016), 080 
 %doi:10.1007/JHEP02(2016)080
 [arXiv:1511.03024 [hep-th]]. %57 citations counted in INSPIRE
% as of 10 Dec 2021
	
	%\cite{Bergshoeff:2017vqp}
%\bibitem{Bergshoeff:2017vqp}
%E.~Bergshoeff, D.~Freedman, R.~Kallosh and A.~Van Proeyen,
%``Supergravity and the cosmological constant,''
%doi:10.1142/9789813226609\_0567
%0 citations counted in INSPIRE as of 10 Dec 2021

%\cite{Nagy:2019ywi}
 \bibitem{Nagy:2019ywi} S.~Nagy, A.~Padilla and I.~Zavala, %``The Super-St\"uckelberg procedure and dS in pure supergravity,'' 
 Proc. Roy. Soc. Lond. A \textbf{476} (2020) no.2237, 20200035 %doi:10.1098/rspa.2020.0035 
 [arXiv:1910.14349 [hep-th]]. %9 citations
 %counted in INSPIRE as of 10 Dec 2021


%\cite{Bansal:2020krz}
 \bibitem{Bansal:2020krz} S.~Bansal, S.~Nagy, A.~Padilla and I.~Zavala, %``Unimodular vs Nilpotent Superfield Approach to Pure dS Supergravity,'' 
 JHEP \textbf{01} (2021), 146 
% doi:10.1007/JHEP01(2021)146 
 [arXiv:2010.13758 [hep-th]]. %3 citations counted in INSPIRE
 %as of 10 Dec 2021

%	%\cite{Metsaev:1987zx}
%	\bibitem{Tseytlin}
%	R.~R.~Metsaev and A.~A.~Tseytlin,
%	%``Order alpha-prime (Two Loop) Equivalence of the String Equations of Motion and the Sigma Model Weyl Invariance Conditions: Dependence on the Dilaton and the Antisymmetric Tensor,''
%	Nucl. Phys. B \textbf{293} (1987), 385-419
%	doi:10.1016/0550-3213(87)90077-0
%	%500 citations counted in INSPIRE as of 02 Nov 2020

	%\cite{Montero:2020rpl}
	\bibitem{Montero}
	M.~Montero, T.~Van Riet and G.~Venken,
	%``A dS obstruction and its phenomenological consequences,''
	JHEP \textbf{05} (2020), 114
%	doi:10.1007/JHEP05(2020)114
	[arXiv:2001.11023 [hep-th]].
	%4 citations counted in INSPIRE as of 30 Oct 202
	
	%\cite{Green:2011cn}
\bibitem{add1}
S.~R.~Green, E.~J.~Martinec, C.~Quigley and S.~Sethi,
%``Constraints on String Cosmology,''
Class. Quant. Grav. \textbf{29} (2012), 075006
%doi:10.1088/0264-9381/29/7/075006
[arXiv:1110.0545 [hep-th]].
%69 citations counted in INSPIRE as of 15 Dec 2021

%\cite{Gautason:2012tb}
\bibitem{add2}
F.~F.~Gautason, D.~Junghans and M.~Zagermann,
%``On Cosmological Constants from alpha'-Corrections,''
JHEP \textbf{06} (2012), 029
%doi:10.1007/JHEP06(2012)029
[arXiv:1204.0807 [hep-th]].
%47 citations counted in INSPIRE as of 15 Dec 2021

%\cite{Kutasov:2015eba}
\bibitem{add3}
D.~Kutasov, T.~Maxfield, I.~Melnikov and S.~Sethi,
%``Constraining de Sitter Space in String Theory,''
Phys. Rev. Lett. \textbf{115} (2015) no.7, 071305
%doi:10.1103/PhysRevLett.115.071305
[arXiv:1504.00056 [hep-th]].
%74 citations counted in INSPIRE as of 15 Dec 2021

%\cite{Quigley:2015jia}
\bibitem{add4}
C.~Quigley,
%``Gaugino Condensation and the Cosmological Constant,''
JHEP \textbf{06} (2015), 104
%doi:10.1007/JHEP06(2015)104
[arXiv:1504.00652 [hep-th]].
%37 citations counted in INSPIRE as of 15 Dec 2021
	
	\bibitem{Campbell}
	B.~A.~Campbell, M.~J.~Duncan, N.~Kaloper and K.~A.~Olive,
	%``Gravitational dynamics with Lorentz Chern-Simons terms,''
	Nucl. Phys. B \textbf{351} (1991), 778-792
%	doi:10.1016/S0550-3213(05)80045-8
	%77 citations counted in INSPIRE as of 30 Oct 2020

	\bibitem{Zwiebach}
	B.~Zwiebach,
	%``Curvature Squared Terms and String Theories,''
	Phys. Lett. B \textbf{156} (1985), 315-317
%	doi:10.1016/0370-2693(85)91616-8
	%1070 citations counted in INSPIRE as of 30 Oct 2020
	
	\bibitem{Zumino}
	B.~Zumino,
	%``Gravity Theories in More Than Four-Dimensions,''
	Phys. Rept. \textbf{137} (1986), 109
%	doi:10.1016/0370-1573(86)90076-1
	%427 citations counted in INSPIRE as of 30 Oct 2020
	
	%\cite{Cecotti:1985nf}
	\bibitem{Cecotti}
	S.~Cecotti, S.~Ferrara, L.~Girardello and M.~Porrati,
	%``Lorentz Chern-simons Terms in $N=1$ Four-dimensional Supergravity Consistent With Supersymmetry and String Compactification,''
	Phys. Lett. B \textbf{164} (1985), 46-50
%	doi:10.1016/0370-2693(85)90028-0
	%66 citations counted in INSPIRE as of 30 Oct 2020
	
		%\cite{Gross:1986mw}
\bibitem{Gross}
D.~J.~Gross and J.~H.~Sloan,
%``The Quartic Effective Action for the Heterotic String,''
Nucl. Phys. B \textbf{291} (1987), 41-89
%doi:10.1016/0550-3213(87)90465-2
%878 citations counted in INSPIRE as of 29 Nov 2021
	
	\bibitem{Gaume}
	L.~Alvarez-Gaume, P.~H.~Ginsparg, G.~W.~Moore and C.~Vafa,
	%``An O(16) x O(16) Heterotic String,''
	Phys. Lett. B \textbf{171} (1986), 155-162
%	doi:10.1016/0370-2693(86)91524-8
	%297 citations counted in INSPIRE as of 02 Nov 2020
	
	%\cite{Becker:2005nb}
\bibitem{Becker:2005nb}
K.~Becker and L.~S.~Tseng,
%``Heterotic flux compactifications and their moduli,''
Nucl. Phys. B \textbf{741} (2006), 162-179
%doi:10.1016/j.nuclphysb.2006.02.013
[arXiv:hep-th/0509131 [hep-th]].
%38 citations counted in INSPIRE as of 29 Nov 2021

	%\cite{Maldacena:2000mw}
	\bibitem{Maldacena}
	J.~M.~Maldacena and C.~Nunez,
	%``Supergravity description of field theories on curved manifolds and a no go theorem,''
	Int. J. Mod. Phys. A \textbf{16} (2001), 822-855
%	doi:10.1142/S0217751X01003937
	[arXiv:hep-th/0007018 [hep-th]].
	%950 citations counted in INSPIRE as of 01 Nov 2020
	
	%\cite{Charmousis:2008ce}
\bibitem{GBpaper}
C.~Charmousis and A.~Padilla,
%``The Instability of Vacua in Gauss-Bonnet Gravity,''
JHEP \textbf{12} (2008), 038
%doi:10.1088/1126-6708/2008/12/038
[arXiv:0807.2864 [hep-th]].
%43 citations counted in INSPIRE as of 30 Nov 2021

%\cite{Gross:1986iv}
\bibitem{GW}
D.~J.~Gross and E.~Witten,
%``Superstring Modifications of Einstein's Equations,''
Nucl. Phys. B \textbf{277} (1986), 1
%doi:10.1016/0550-3213(86)90429-3
%877 citations counted in INSPIRE as of 08 Dec 2021

\bibitem{michelson}
A.~A.~Michelson,
``Light Waves and Their Uses'',
Univ of Chicago, reprint edition, 1903.

\bibitem{kelvin}
Right.~Hon.~Lord~Kelvin~G.C.V.O.~D.C.L.~LL.D.~F.R.S.~M.R.I., 
The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science, 2:7, 1-40, 
doi:10.1080/14786440109462664. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF CHAPTER 9 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% APPENDIX 1 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%NO REFERENCES!!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF APPENDIX 1 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% APPENDIX 2 %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\cite{Polchinski:1998rr}
\bibitem{Polchinski:1998rr}
J.~Polchinski,
%``String theory. Vol. 2: Superstring theory and beyond,''
doi:10.1017/CBO9780511618123
%438 citations counted in INSPIRE as of 05 Nov 2021

%\cite{hep-th/0202168}
\bibitem{hep-th/0202168}
J.~Louis and A.~Micu,
%``Type 2 theories compactified on Calabi-Yau threefolds in the presence of background fluxes,''
Nucl. Phys. B \textbf{635} (2002), 395-431
doi:10.1016/S0550-3213(02)00338-3
[arXiv:hep-th/0202168 [hep-th]].
%247 citations counted in INSPIRE as of 15 Oct 2021

%\cite{hep-th/9804208}
\bibitem{hep-th/9804208}
A.~Dabholkar,
%``Lectures on orientifolds and duality,''
[arXiv:hep-th/9804208 [hep-th]].
%110 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/9403096}
\bibitem{hep-th/9403096}
S.~Hosono, A.~Klemm and S.~Theisen,
%``Lectures on mirror symmetry,''
Lect. Notes Phys. \textbf{436} (1994), 235-280
doi:10.1007/3-540-58453-6\_13
[arXiv:hep-th/9403096 [hep-th]].
%127 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0804.1248}
\bibitem{0804.1248}
E.~Palti, G.~Tasinato and J.~Ward,
%``WEAKLY-coupled IIA Flux Compactifications,''
JHEP \textbf{06} (2008), 084
doi:10.1088/1126-6708/2008/06/084
[arXiv:0804.1248 [hep-th]].
%70 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0412277}
\bibitem{hep-th/0412277}
T.~W.~Grimm and J.~Louis,
%``The Effective action of type IIA Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{718} (2005), 153-202
doi:10.1016/j.nuclphysb.2005.04.007
[arXiv:hep-th/0412277 [hep-th]].
%265 citations counted in INSPIRE as of 09 Nov 2021

%\cite{Romans:1985tz}
\bibitem{Romans:1985tz}
L.~J.~Romans,
%``Massive N=2a Supergravity in Ten-Dimensions,''
Phys. Lett. B \textbf{169} (1986), 374
doi:10.1016/0370-2693(86)90375-8
%552 citations counted in INSPIRE as of 08 Nov 2021

%\cite{1507.06793}
\bibitem{1507.06793}
S.~Bielleman, L.~E.~Ibanez and I.~Valenzuela,
%``Minkowski 3-forms, Flux String Vacua, Axion Stability and Naturalness,''
JHEP \textbf{12} (2015), 119
doi:10.1007/JHEP12(2015)119
[arXiv:1507.06793 [hep-th]].
%69 citations counted in INSPIRE as of 02 Nov 2021

%\cite{1606.00508}
\bibitem{1606.00508}
F.~Carta, F.~Marchesano, W.~Staessens and G.~Zoccarato,
%``Open string multi-branched and K\"ahler potentials,''
JHEP \textbf{09} (2016), 062
doi:10.1007/JHEP09(2016)062
[arXiv:1606.00508 [hep-th]].
%56 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0505160}
\bibitem{hep-th/0505160}
O.~DeWolfe, A.~Giryavets, S.~Kachru and W.~Taylor,
%``Type IIA moduli stabilization,''
JHEP \textbf{07} (2005), 066
doi:10.1088/1126-6708/2005/07/066
[arXiv:hep-th/0505160 [hep-th]].
%375 citations counted in INSPIRE as of 02 Nov 2021

%\cite{hep-th/0607223}
\bibitem{hep-th/0607223}
B.~S.~Acharya, F.~Benini and R.~Valandro,
%``Fixing moduli in exact type IIA flux vacua,''
JHEP \textbf{02} (2007), 018
doi:10.1088/1126-6708/2007/02/018
[arXiv:hep-th/0607223 [hep-th]].
%96 citations counted in INSPIRE as of 25 Oct 2021

%\cite{Hosono:1994av}
\bibitem{hep-th/9403096}
S.~Hosono, A.~Klemm and S.~Theisen,
%``Lectures on mirror symmetry,''
Lect. Notes Phys. \textbf{436} (1994), 235-280
doi:10.1007/3-540-58453-6\_13
[arXiv:hep-th/9403096 [hep-th]].
%127 citations counted in INSPIRE as of 09 Nov 2021
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% END OF APPENDIX 2 %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{thebibliography}

==> Bibliography/bib_include.tex <==
\begin{thebibliography}{99}
\include{intro-references}
\include{pert-references}
\include{openqs-references}
\include{clockwork-references}
\include{coincidence-references}
\include{intermezzo-references}
\include{non_pert-references}
\include{model_building-references}
\include{gbds-references}
\include{outlook-references}
\include{iia_details-references}
\end{thebibliography}

==> Bibliography/clockwork-references.tex <==
%\cite{1912.04905}
\bibitem{1912.04905}
L.~Bordin, F.~Cunillera, A.~Leh\'ebel and A.~Padilla,
%``A natural theory of dark energy,''
Phys. Rev. D \textbf{101} (2020), 085012
doi:10.1103/PhysRevD.101.085012
[arXiv:1912.04905 [hep-th]].
%6 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1511.00132}
\bibitem{1511.00132}
K.~Choi and S.~H.~Im,
%``Realizing the relaxion from multiple axions and its UV completion with high scale supersymmetry,''
JHEP \textbf{01} (2016), 149
doi:10.1007/JHEP01(2016)149
[arXiv:1511.00132 [hep-ph]].
%211 citations counted in INSPIRE as of 15 Oct 2021

%\cite{1511.01827}
\bibitem{1511.01827}
D.~E.~Kaplan and R.~Rattazzi,
%``Large field excursions and approximate discrete symmetries from a clockwork axion,''
Phys. Rev. D \textbf{93} (2016) no.8, 085007
doi:10.1103/PhysRevD.93.085007
[arXiv:1511.01827 [hep-ph]].
%236 citations counted in INSPIRE as of 15 Oct 2021

%\cite{hep-th/0410286}
\bibitem{hep-th/0410286}
G.~Dvali,
%``Large hierarchies from attractor vacua,''
Phys. Rev. D \textbf{74} (2006), 025018
doi:10.1103/PhysRevD.74.025018
[arXiv:hep-th/0410286 [hep-th]].
%92 citations counted in INSPIRE as of 12 Oct 2021

%\cite{hep-th/0507215}
\bibitem{hep-th/0507215}
G.~Dvali,
%``Three-form gauging of axion symmetries and gravity,''
[arXiv:hep-th/0507215 [hep-th]].
%122 citations counted in INSPIRE as of 25 Oct 2021

%\cite{0811.1989}
\bibitem{0811.1989}
N.~Kaloper and L.~Sorbo,
%``A Natural Framework for Chaotic Inflation,''
Phys. Rev. Lett. \textbf{102} (2009), 121301
doi:10.1103/PhysRevLett.102.121301
[arXiv:0811.1989 [hep-th]].
%318 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1101.0026}
\bibitem{1101.0026}
N.~Kaloper, A.~Lawrence and L.~Sorbo,
%``An Ignoble Approach to Large Field Inflation,''
JCAP \textbf{03} (2011), 023
doi:10.1088/1475-7516/2011/03/023
[arXiv:1101.0026 [hep-th]].
%268 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0303252}
\bibitem{hep-th/0303252}
T.~Banks, M.~Dine, P.~J.~Fox and E.~Gorbatov,
%``On the possibility of large axion decay constants,''
JCAP \textbf{06} (2003), 001
doi:10.1088/1475-7516/2003/06/001
[arXiv:hep-th/0303252 [hep-th]].
%337 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0409138}
\bibitem{hep-th/0409138}
S.~Ghosh,
%``Extended space duality in the noncommutative plane,''
Phys. Lett. B \textbf{601} (2004), 93-98
doi:10.1016/j.physletb.2004.09.023
[arXiv:hep-th/0409138 [hep-th]].
%5 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/0601001}
\bibitem{hep-th/0601001}
N.~Arkani-Hamed, L.~Motl, A.~Nicolis and C.~Vafa,
%``The String landscape, black holes and gravity as the weakest force,''
JHEP \textbf{06} (2007), 060
doi:10.1088/1126-6708/2007/06/060
[arXiv:hep-th/0601001 [hep-th]].
%881 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1503.04783}
\bibitem{1503.04783}
J.~Brown, W.~Cottrell, G.~Shiu and P.~Soler,
%``Fencing in the Swampland: Quantum Gravity Constraints on Large Field Inflation,''
JHEP \textbf{10} (2015), 023
doi:10.1007/JHEP10(2015)023
[arXiv:1503.04783 [hep-th]].
%198 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1402.2287}
\bibitem{1402.2287}
C.~Cheung and G.~N.~Remmen,
%``Naturalness and the Weak Gravity Conjecture,''
Phys. Rev. Lett. \textbf{113} (2014), 051601
doi:10.1103/PhysRevLett.113.051601
[arXiv:1402.2287 [hep-ph]].
%165 citations counted in INSPIRE as of 22 Oct 2021

%\cite{1503.00795}
\bibitem{1503.00795}
T.~Rudelius,
%``Constraints on Axion Inflation from the Weak Gravity Conjecture,''
JCAP \textbf{09} (2015), 020
doi:10.1088/1475-7516/2015/9/020
[arXiv:1503.00795 [hep-th]].
%177 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1610.07962}
\bibitem{1610.07962}
G.~F.~Giudice and M.~McCullough,
%``A Clockwork Theory,''
JHEP \textbf{02} (2017), 036
doi:10.1007/JHEP02(2017)036
[arXiv:1610.07962 [hep-ph]].
%159 citations counted in INSPIRE as of 14 Oct 2021

%\cite{tHooft:1979rat}
\bibitem{tHooft:1979rat}
G.~'t Hooft,
%``Naturalness, chiral symmetry, and spontaneous chiral symmetry breaking,''
NATO Sci. Ser. B \textbf{59} (1980), 135-157
doi:10.1007/978-1-4684-7571-5\_9
%713 citations counted in INSPIRE as of 25 Oct 2021

%\cite{0803.3085}
\bibitem{0803.3085}
E.~Silverstein and A.~Westphal,
%``Monodromy in the CMB: Gravity Waves and String Inflation,''
Phys. Rev. D \textbf{78} (2008), 106003
doi:10.1103/PhysRevD.78.106003
[arXiv:0803.3085 [hep-th]].
%800 citations counted in INSPIRE as of 22 Oct 2021

%\cite{0808.0706}
\bibitem{0808.0706}
L.~McAllister, E.~Silverstein and A.~Westphal,
%``Gravity Waves and Linear Inflation from Axion Monodromy,''
Phys. Rev. D \textbf{82} (2010), 046003
doi:10.1103/PhysRevD.82.046003
[arXiv:0808.0706 [hep-th]].
%721 citations counted in INSPIRE as of 22 Oct 2021

%\cite{1611.00394}
\bibitem{1611.00394}
I.~Valenzuela,
%``Backreaction Issues in Axion Monodromy and Minkowski 4-forms,''
JHEP \textbf{06} (2017), 098
doi:10.1007/JHEP06(2017)098
[arXiv:1611.00394 [hep-th]].
%74 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1607.06105}
\bibitem{1607.06105}
N.~Kaloper and A.~Lawrence,
%``London equation for monodromy inflation,''
Phys. Rev. D \textbf{95} (2017) no.6, 063526
doi:10.1103/PhysRevD.95.063526
[arXiv:1607.06105 [hep-th]].
%32 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1806.04740}
\bibitem{1806.04740}
A.~Padilla,
%``Monodromy inflation and an emergent mechanism for stabilising the cosmological constant,''
JHEP \textbf{01} (2019), 175
doi:10.1007/JHEP01(2019)175
[arXiv:1806.04740 [hep-th]].
%7 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1903.07612}
\bibitem{1903.07612}
B.~K.~El-Menoufi, S.~Nagy, F.~Niedermann and A.~Padilla,
%``Quantum corrections to vacuum energy sequestering (with monodromy),''
Class. Quant. Grav. \textbf{36} (2019) no.21, 215014
doi:10.1088/1361-6382/ab46f6
[arXiv:1903.07612 [hep-th]].
%4 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1806.03308}
\bibitem{1806.03308}
N.~Kaloper,
%``Irrational Monodromies of Vacuum Energy,''
JHEP \textbf{11} (2019), 106
doi:10.1007/JHEP11(2019)106
[arXiv:1806.03308 [hep-th]].
%8 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2013zca}
\bibitem{Kaloper:2013zca}
N.~Kaloper and A.~Padilla,
%``Sequestering the Standard Model Vacuum Energy,''
Phys. Rev. Lett. \textbf{112} (2014) no.9, 091304
doi:10.1103/PhysRevLett.112.091304
[arXiv:1309.6562 [hep-th]].
%128 citations counted in INSPIRE as of 20 Oct 2021

%\cite{Kaloper:2014dqa}
\bibitem{Kaloper:2014dqa}
N.~Kaloper and A.~Padilla,
%``Vacuum Energy Sequestering: The Framework and Its Cosmological Consequences,''
Phys. Rev. D \textbf{90} (2014) no.8, 084023
doi:10.1103/PhysRevD.90.084023
[arXiv:1406.0711 [hep-th]].
%85 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2014fca}
\bibitem{Kaloper:2014fca}
N.~Kaloper and A.~Padilla,
%``Sequestration of Vacuum Energy and the End of the Universe,''
Phys. Rev. Lett. \textbf{114} (2015) no.10, 101302
doi:10.1103/PhysRevLett.114.101302
[arXiv:1409.7073 [hep-th]].
%40 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2015jra}
\bibitem{Kaloper:2015jra}
N.~Kaloper, A.~Padilla, D.~Stefanyszyn and G.~Zahariade,
%``Manifestly Local Theory of Vacuum Energy Sequestering,''
Phys. Rev. Lett. \textbf{116} (2016) no.5, 051302
doi:10.1103/PhysRevLett.116.051302
[arXiv:1505.01492 [hep-th]].
%66 citations counted in INSPIRE as of 13 Oct 2021

%\cite{Kaloper:2016yfa}
\bibitem{Kaloper:2016yfa}
N.~Kaloper, A.~Padilla and D.~Stefanyszyn,
%``Sequestering effects on and of vacuum decay,''
Phys. Rev. D \textbf{94} (2016) no.2, 025022
doi:10.1103/PhysRevD.94.025022
[arXiv:1604.04000 [hep-th]].
%17 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kaloper:2016jsd}
\bibitem{Kaloper:2016jsd}
N.~Kaloper and A.~Padilla,
%``Vacuum Energy Sequestering and Graviton Loops,''
Phys. Rev. Lett. \textbf{118} (2017) no.6, 061303
doi:10.1103/PhysRevLett.118.061303
[arXiv:1606.04958 [hep-th]].
%29 citations counted in INSPIRE as of 11 Oct 2021

%\cite{DAmico:2017ngr}
\bibitem{DAmico:2017ngr}
G.~D'Amico, N.~Kaloper, A.~Padilla, D.~Stefanyszyn, A.~Westphal and G.~Zahariade,
%``An \'etude on global vacuum energy sequester,''
JHEP \textbf{09} (2017), 074
doi:10.1007/JHEP09(2017)074
[arXiv:1705.08950 [hep-th]].
%18 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Niedermann:2017cel}
\bibitem{Niedermann:2017cel}
F.~Niedermann and A.~Padilla,
%``Gravitational Mechanisms to Self-Tune the Cosmological Constant: Obstructions and Ways Forward,''
Phys. Rev. Lett. \textbf{119} (2017) no.25, 251306
doi:10.1103/PhysRevLett.119.251306
[arXiv:1706.04778 [hep-th]].
%13 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Coltman:2019mql}
\bibitem{Coltman:2019mql}
B.~Coltman, Y.~Li and A.~Padilla,
%``Cosmological consequences of Omnia Sequestra,''
JCAP \textbf{06} (2019), 017
doi:10.1088/1475-7516/2019/06/017
[arXiv:1903.02829 [hep-th]].
%4 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9510227}
\bibitem{hep-th/9510227}
J.~Polchinski and A.~Strominger,
%``New vacua for type II string theory,''
Phys. Lett. B \textbf{388} (1996), 736-742
doi:10.1016/S0370-2693(96)01219-1
[arXiv:hep-th/9510227 [hep-th]].
%346 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0004134}
\bibitem{hep-th/0004134}
R.~Bousso and J.~Polchinski,
%``Quantization of four form fluxes and dynamical neutralization of the cosmological constant,''
JHEP \textbf{06} (2000), 006
doi:10.1088/1126-6708/2000/06/006
[arXiv:hep-th/0004134 [hep-th]].
%1208 citations counted in INSPIRE as of 22 Oct 2021

%\cite{Lee:1987qc}
\bibitem{Lee:1987qc}
K.~M.~Lee and E.~J.~Weinberg,
%``Decay of the True Vacuum in Curved Space-time,''
Phys. Rev. D \textbf{36} (1987), 1088
doi:10.1103/PhysRevD.36.1088
%148 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0607223}
\bibitem{hep-th/0607223}
B.~S.~Acharya, F.~Benini and R.~Valandro,
%``Fixing moduli in exact type IIA flux vacua,''
JHEP \textbf{02} (2007), 018
doi:10.1088/1126-6708/2007/02/018
[arXiv:hep-th/0607223 [hep-th]].
%96 citations counted in INSPIRE as of 25 Oct 2021

%\cite{0812.3551}
\bibitem{0812.3551}
C.~Caviezel, P.~Koerber, S.~Kors, D.~Lust, T.~Wrase and M.~Zagermann,
%``On the Cosmology of Type IIA Compactifications on SU(3)-structure Manifolds,''
JHEP \textbf{04} (2009), 010
doi:10.1088/1126-6708/2009/04/010
[arXiv:0812.3551 [hep-th]].
%133 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1807.09698}
\bibitem{1807.09698}
D.~Andriot,
%``New constraints on classical de Sitter: flirting with the swampland,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800103
doi:10.1002/prop.201800103
[arXiv:1807.09698 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Ibanez:2017vfl}
\bibitem{Ibanez:2017vfl}
L.~E.~Ibanez and M.~Montero,
%``A Note on the WGC, Effective Field Theory and Clockwork within String Theory,''
JHEP \textbf{02} (2018), 057
doi:10.1007/JHEP02(2018)057
[arXiv:1709.02392 [hep-th]].
%36 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1507.06793}
\bibitem{1507.06793}
S.~Bielleman, L.~E.~Ibanez and I.~Valenzuela,
%``Minkowski 3-forms, Flux String Vacua, Axion Stability and Naturalness,''
JHEP \textbf{12} (2015), 119
doi:10.1007/JHEP12(2015)119
[arXiv:1507.06793 [hep-th]].
%67 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1606.00508}
\bibitem{1606.00508}
F.~Carta, F.~Marchesano, W.~Staessens and G.~Zoccarato,
%``Open string multi-branched and K\"ahler potentials,''
JHEP \textbf{09} (2016), 062
doi:10.1007/JHEP09(2016)062
[arXiv:1606.00508 [hep-th]].
%56 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0103233}
\bibitem{hep-th/0103233}
E.~Bergshoeff, R.~Kallosh, T.~Ortin, D.~Roest and A.~Van Proeyen,
%``New formulations of D = 10 supersymmetry and D8 - O8 domain walls,''
Class. Quant. Grav. \textbf{18} (2001), 3359-3382
doi:10.1088/0264-9381/18/17/303
[arXiv:hep-th/0103233 [hep-th]].
%303 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0411271}
\bibitem{hep-th/0411271}
A.~Saltman and E.~Silverstein,
%``A New handle on de Sitter compactifications,''
JHEP \textbf{01} (2006), 139
doi:10.1088/1126-6708/2006/01/139
[arXiv:hep-th/0411271 [hep-th]].
%99 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0505160}
\bibitem{hep-th/0505160}
O.~DeWolfe, A.~Giryavets, S.~Kachru and W.~Taylor,
%``Type IIA moduli stabilization,''
JHEP \textbf{07} (2005), 066
doi:10.1088/1126-6708/2005/07/066
[arXiv:hep-th/0505160 [hep-th]].
%374 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1705.10162}
\bibitem{1705.10162}
G.~F.~Giudice and M.~McCullough,
%``Comment on ''Disassembling the Clockwork Mechanism'',''
[arXiv:1705.10162 [hep-ph]].
%43 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-ph/9905221}
\bibitem{hep-ph/9905221}
L.~Randall and R.~Sundrum,
%``A Large mass hierarchy from a small extra dimension,''
Phys. Rev. Lett. \textbf{83} (1999), 3370-3373
doi:10.1103/PhysRevLett.83.3370
[arXiv:hep-ph/9905221 [hep-ph]].
%9248 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1808.08967}
\bibitem{1808.08967}
M.~Cicoli, S.~De Alwis, A.~Maharana, F.~Muia and F.~Quevedo,
%``De Sitter vs Quintessence in String Theory,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800079
doi:10.1002/prop.201800079
[arXiv:1808.08967 [hep-th]].
%133 citations counted in INSPIRE as of 11 Oct 2021

==> Bibliography/coincidence-references.tex <==

%\cite{Ooguri:2006in}
\bibitem{distance1}
H.~Ooguri and C.~Vafa,
%``On the Geometry of the String Landscape and the Swampland,''
Nucl. Phys. B \textbf{766} (2007), 21-33
%doi:10.1016/j.nuclphysb.2006.10.033
[arXiv:hep-th/0605264 [hep-th]].
%483 citations counted in INSPIRE as of 17 Dec 2020


%\cite{Klaewer:2016kiy}
\bibitem{distance2}
D.~Klaewer and E.~Palti,
%``Super-Planckian Spatial Field Variations and Quantum Gravity,''
JHEP \textbf{01} (2017), 088
%doi:10.1007/JHEP01(2017)088
[arXiv:1610.00010 [hep-th]].
%154 citations counted in INSPIRE as of 17 Dec 2020


%\cite{Grimm:2018ohb}
\bibitem{distance3}
T.~W.~Grimm, E.~Palti and I.~Valenzuela,
%``Infinite Distances in Field Space and Massless Towers of States,''
JHEP \textbf{08} (2018), 143
%doi:10.1007/JHEP08(2018)143
[arXiv:1802.08264 [hep-th]].
%128 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Blumenhagen:2018nts}
\bibitem{distance4}
R.~Blumenhagen, D.~Kl\"awer, L.~Schlechter and F.~Wolf,
%``The Refined Swampland Distance Conjecture in Calabi-Yau Moduli Spaces,''
JHEP \textbf{06} (2018), 052
%doi:10.1007/JHEP06(2018)052
[arXiv:1803.04989 [hep-th]].
%68 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Agrawal:2018own}
\bibitem{swampcos}
P.~Agrawal, G.~Obied, P.~J.~Steinhardt and C.~Vafa,
%``On the Cosmological Implications of the String Swampland,''
Phys. Lett. B \textbf{784} (2018), 271-276
%doi:10.1016/j.physletb.2018.07.040
[arXiv:1806.09718 [hep-th]].
%287 citations counted in INSPIRE as of 18 Dec 2020


%\cite{Obied:2018sgi}
\bibitem{dscon1}
G.~Obied, H.~Ooguri, L.~Spodyneiko and C.~Vafa,
%``De Sitter Space and the Swampland,''
[arXiv:1806.08362 [hep-th]].
%475 citations counted in INSPIRE as of 17 Dec 2020


%\cite{Garg:2018reu}
\bibitem{chet}
S.~K.~Garg and C.~Krishnan,
%``Bounds on Slow Roll and the de Sitter Swampland,''
JHEP \textbf{11} (2019), 075
%doi:10.1007/JHEP11(2019)075
[arXiv:1807.05193 [hep-th]].
%369 citations counted in INSPIRE as of 06 Aug 2021


%\cite{Ooguri:2018wrx}
\bibitem{dscon2}
H.~Ooguri, E.~Palti, G.~Shiu and C.~Vafa,
%``Distance and de Sitter Conjectures on the Swampland,''
Phys. Lett. B \textbf{788} (2019), 180-184
%doi:10.1016/j.physletb.2018.11.018
[arXiv:1810.05506 [hep-th]].
%306 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Baume:2016psm}
\bibitem{moredist1}
F.~Baume and E.~Palti,
%``Backreacted Axion Field Ranges in String Theory,''
JHEP \textbf{08} (2016), 043
%doi:10.1007/JHEP08(2016)043
[arXiv:1602.06517 [hep-th]].
%99 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Hebecker:2017lxm}
\bibitem{moredist2}
A.~Hebecker, P.~Henkenjohann and L.~T.~Witkowski,
%``Flat Monodromies and a Moduli Space Size Conjecture,''
JHEP \textbf{12} (2017), 033
%doi:10.1007/JHEP12(2017)033
[arXiv:1708.06761 [hep-th]].
%49 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Cicoli:2018tcq}
\bibitem{moredist3}
M.~Cicoli, D.~Ciupke, C.~Mayrhofer and P.~Shukla,
%``A Geometrical Upper Bound on the Inflaton Range,''
JHEP \textbf{05} (2018), 001
%doi:10.1007/JHEP05(2018)001
[arXiv:1801.05434 [hep-th]].
%47 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Blumenhagen:2017cxt}
\bibitem{moredist4}
R.~Blumenhagen, I.~Valenzuela and F.~Wolf,
%``The Swampland Conjecture and F-term Axion Monodromy Inflation,''
JHEP \textbf{07} (2017), 145
%doi:10.1007/JHEP07(2017)145
[arXiv:1703.05776 [hep-th]].
%86 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Heidenreich:2018kpg}
\bibitem{moredist4}
B.~Heidenreich, M.~Reece and T.~Rudelius,
%``Emergence of Weak Coupling at Large Distance in Quantum Gravity,''
Phys. Rev. Lett. \textbf{121} (2018) no.5, 051601
%doi:10.1103/PhysRevLett.121.051601
[arXiv:1802.08698 [hep-th]].
%83 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Landete:2018kqf}
\bibitem{moredist5}
A.~Landete and G.~Shiu,
%``Mass Hierarchies and Dynamical Field Range,''
Phys. Rev. D \textbf{98} (2018) no.6, 066012
d%oi:10.1103/PhysRevD.98.066012
[arXiv:1806.01874 [hep-th]].
%33 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Lee:2018urn}
\bibitem{moredist6}
S.~J.~Lee, W.~Lerche and T.~Weigand,
%``Tensionless Strings and the Weak Gravity Conjecture,''
JHEP \textbf{10} (2018), 164
%doi:10.1007/JHEP10(2018)164
[arXiv:1808.05958 [hep-th]].
%87 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Blumenhagen:2018hsh}
\bibitem{moredist7}
R.~Blumenhagen,
%``Large Field Inflation/Quintessence and the Refined Swampland Distance Conjecture,''
PoS \textbf{CORFU2017} (2018), 175
%doi:10.22323/1.318.0175
[arXiv:1804.10504 [hep-th]].
%47 citations counted in INSPIRE as of 17 Dec 2020

  %\cite{Mukhanov:2007zz}
\bibitem{mukbook}
V.~Mukhanov and S.~Winitzki,
``Introduction to quantum effects in gravity.''
%122 citations counted in INSPIRE as of 26 Apr 2021

%\cite{Bordin:2019fek}
\bibitem{dsstuff}
F.~Cunillera and A.~Padilla,
In preparation.

\bibitem{AS}
M.~Abramowitz and I.~Stegun,
``Handbook of Mathematical Functions with Formulas, Graphs, and Mathematical Tables."
%122 citations counted in INSPIRE as of 26 Apr 2021

%\cite{Khoury:2003aq}
\bibitem{cham1}
J.~Khoury and A.~Weltman,
%``Chameleon fields: Awaiting surprises for tests of gravity in space,''
Phys. Rev. Lett. \textbf{93} (2004), 171104
%doi:10.1103/PhysRevLett.93.171104
[arXiv:astro-ph/0309300 [astro-ph]].
%1202 citations counted in INSPIRE as of 30 Apr 2021

%\cite{Khoury:2003rn}
\bibitem{cham2}
J.~Khoury and A.~Weltman,
%``Chameleon cosmology,''
Phys. Rev. D \textbf{69} (2004), 044026
%doi:10.1103/PhysRevD.69.044026
[arXiv:astro-ph/0309411 [astro-ph]].
%1279 citations counted in INSPIRE as of 30 Apr 2021

%\cite{Padilla:2015wlv}
\bibitem{cham3}
A.~Padilla, E.~Platts, D.~Stefanyszyn, A.~Walters, A.~Weltman and T.~Wilson,
%``How to Avoid a Swift Kick in the Chameleons,''
JCAP \textbf{03} (2016), 058
%doi:10.1088/1475-7516/2016/03/058
[arXiv:1511.05761 [hep-th]].
%11 citations counted in INSPIRE as of 30 Apr 2021

%\cite{Font:2019cxq}
\bibitem{Font:2019cxq}
A.~Font, A.~Herr\'aez and L.~E.~Ib\'a\~nez,
%``The Swampland Distance Conjecture and Towers of Tensionless Branes,''
JHEP \textbf{08} (2019), 044
%doi:10.1007/JHEP08(2019)044
[arXiv:1904.05379 [hep-th]].
%39 citations counted in INSPIRE as of 17 Dec 2020

%\cite{Hebecker:2019csg}
\bibitem{Heb}
A.~Hebecker, T.~Skrzypek and M.~Wittner,
%``The $F$-term Problem and other Challenges of Stringy Quintessence,''
JHEP \textbf{11} (2019), 134
%doi:10.1007/JHEP11(2019)134
[arXiv:1909.08625 [hep-th]].
%13 citations counted in INSPIRE as of 07 Jul 2021

%\cite{1808.09440}
\bibitem{1808.09440}
Y.~Akrami, R.~Kallosh, A.~Linde and V.~Vardanyan,
%``The Landscape, the Swampland and the Era of Precision Cosmology,''
Fortsch. Phys. \textbf{67} (2019) no.1-2, 1800075
doi:10.1002/prop.201800075
[arXiv:1808.09440 [hep-th]].
%191 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/0603057}
\bibitem{hep-th/0603057}
E.~J.~Copeland, M.~Sami and S.~Tsujikawa,
%``Dynamics of dark energy,''
Int. J. Mod. Phys. D \textbf{15} (2006), 1753-1936
doi:10.1142/S021827180600942X
[arXiv:hep-th/0603057 [hep-th]].
%4627 citations counted in INSPIRE as of 20 Oct 2021

%\cite{1909.11063}
\bibitem{1909.11063}
A.~Bedroya and C.~Vafa,
%``Trans-Planckian Censorship and the Swampland,''
JHEP \textbf{09} (2020), 123
doi:10.1007/JHEP09(2020)123
[arXiv:1909.11063 [hep-th]].
%188 citations counted in INSPIRE as of 15 Oct 2021

%\cite{2110.07300}
\bibitem{2110.07300}
M.~Dine and Y.~Yu,
%``Comments on the Transplanckian Censorship Conjecture,''
[arXiv:2110.07300 [hep-th]].
%0 citations counted in INSPIRE as of 20 Oct 2021


==> Bibliography/ii_a_details-references.tex <==
%\cite{Polchinski:1998rr}
\bibitem{Polchinski:1998rr}
J.~Polchinski,
%``String theory. Vol. 2: Superstring theory and beyond,''
doi:10.1017/CBO9780511618123
%435 citations counted in INSPIRE as of 13 Oct 2021

%\cite{hep-th/0202168}
\bibitem{hep-th/0202168}
J.~Louis and A.~Micu,
%``Type 2 theories compactified on Calabi-Yau threefolds in the presence of background fluxes,''
Nucl. Phys. B \textbf{635} (2002), 395-431
doi:10.1016/S0550-3213(02)00338-3
[arXiv:hep-th/0202168 [hep-th]].
%247 citations counted in INSPIRE as of 15 Oct 2021

%\cite{hep-th/0507153}
\bibitem{hep-th/0507153}
T.~W.~Grimm,
%``The Effective action of type II Calabi-Yau orientifolds,''
Fortsch. Phys. \textbf{53} (2005), 1179-1271
doi:10.1002/prop.200510253
[arXiv:hep-th/0507153 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9804208}
\bibitem{hep-th/9804208}
A.~Dabholkar,
%``Lectures on orientifolds and duality,''
[arXiv:hep-th/9804208 [hep-th]].
%110 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/9403096}
\bibitem{hep-th/9403096}
S.~Hosono, A.~Klemm and S.~Theisen,
%``Lectures on mirror symmetry,''
Lect. Notes Phys. \textbf{436} (1994), 235-280
doi:10.1007/3-540-58453-6\_13
[arXiv:hep-th/9403096 [hep-th]].
%127 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0804.1248}
\bibitem{0804.1248}
E.~Palti, G.~Tasinato and J.~Ward,
%``WEAKLY-coupled IIA Flux Compactifications,''
JHEP \textbf{06} (2008), 084
doi:10.1088/1126-6708/2008/06/084
[arXiv:0804.1248 [hep-th]].
%70 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0412277}
\bibitem{hep-th/0412277}
T.~W.~Grimm and J.~Louis,
%``The Effective action of type IIA Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{718} (2005), 153-202
doi:10.1016/j.nuclphysb.2005.04.007
[arXiv:hep-th/0412277 [hep-th]].
%263 citations counted in INSPIRE as of 25 Oct 2021

%\cite{Romans:1985tz}
\bibitem{Romans:1985tz}
L.~J.~Romans,
%``Massive N=2a Supergravity in Ten-Dimensions,''
Phys. Lett. B \textbf{169} (1986), 374
doi:10.1016/0370-2693(86)90375-8
%551 citations counted in INSPIRE as of 19 Oct 2021

%\cite{1606.00508}
\bibitem{1606.00508}
F.~Carta, F.~Marchesano, W.~Staessens and G.~Zoccarato,
%``Open string multi-branched and K\"ahler potentials,''
JHEP \textbf{09} (2016), 062
doi:10.1007/JHEP09(2016)062
[arXiv:1606.00508 [hep-th]].
%56 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0505160}
\bibitem{hep-th/0505160}
O.~DeWolfe, A.~Giryavets, S.~Kachru and W.~Taylor,
%``Type IIA moduli stabilization,''
JHEP \textbf{07} (2005), 066
doi:10.1088/1126-6708/2005/07/066
[arXiv:hep-th/0505160 [hep-th]].
%374 citations counted in INSPIRE as of 25 Oct 2021

==> Bibliography/pert-references.tex <==
%\cite{Grimm:2004uq}
\bibitem{Grimm:2004uq}
T.~W.~Grimm and J.~Louis,
%``The Effective action of N = 1 Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{699} (2004), 387-426
doi:10.1016/j.nuclphysb.2004.08.005
[arXiv:hep-th/0403067 [hep-th]].
%365 citations counted in INSPIRE as of 13 Oct 2021

%\cite{Grimm:2004ua}
\bibitem{Grimm:2004ua}
T.~W.~Grimm and J.~Louis,
%``The Effective action of type IIA Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{718} (2005), 153-202
doi:10.1016/j.nuclphysb.2005.04.007
[arXiv:hep-th/0412277 [hep-th]].
%263 citations counted in INSPIRE as of 25 Oct 2021

%\cite{Grimm:2005fa}
\bibitem{Grimm:2005fa}
T.~W.~Grimm,
%``The Effective action of type II Calabi-Yau orientifolds,''
Fortsch. Phys. \textbf{53} (2005), 1179-1271
doi:10.1002/prop.200510253
[arXiv:hep-th/0507153 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Polchinski:1998rr}
\bibitem{Polchinski:1998rr}
J.~Polchinski,
%``String theory. Vol. 2: Superstring theory and beyond,''
doi:10.1017/CBO9780511618123
%435 citations counted in INSPIRE as of 13 Oct 2021

%\cite{hep-th/9908007}
\bibitem{hep-th/9908007}
R.~Bohm, H.~Gunther, C.~Herrmann and J.~Louis,
%``Compactification of type IIB string theory on Calabi-Yau threefolds,''
Nucl. Phys. B \textbf{569} (2000), 229-246
doi:10.1016/S0550-3213(99)00796-8
[arXiv:hep-th/9908007 [hep-th]].
%78 citations counted in INSPIRE as of 15 Oct 2021

%\cite{hep-th/0507153}
\bibitem{hep-th/0507153}
T.~W.~Grimm,
%``The Effective action of type II Calabi-Yau orientifolds,''
Fortsch. Phys. \textbf{53} (2005), 1179-1271
doi:10.1002/prop.200510253
[arXiv:hep-th/0507153 [hep-th]].
%76 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Ferrara:1988ff}
\bibitem{Ferrara:1988ff}
S.~Ferrara and S.~Sabharwal,
%``Dimensional Reduction of Type {II} Superstrings,''
Class. Quant. Grav. \textbf{6} (1989), L77
doi:10.1088/0264-9381/6/4/002
%71 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Ferrara:1989ik}
\bibitem{Ferrara:1989ik}
S.~Ferrara and S.~Sabharwal,
%``Quaternionic Manifolds for Type II Superstring Vacua of Calabi-Yau Spaces,''
Nucl. Phys. B \textbf{332} (1990), 317-332
doi:10.1016/0550-3213(90)90097-W
%327 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9804208}
\bibitem{hep-th/9804208}
A.~Dabholkar,
%``Lectures on orientifolds and duality,''
[arXiv:hep-th/9804208 [hep-th]].
%110 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/0103068}
\bibitem{hep-th/0103068}
M.~Haack and J.~Louis,
%``M theory compactified on Calabi-Yau fourfolds with background flux,''
Phys. Lett. B \textbf{507} (2001), 296-304
doi:10.1016/S0370-2693(01)00464-6
[arXiv:hep-th/0103068 [hep-th]].
%145 citations counted in INSPIRE as of 13 Oct 2021

%\cite{hep-th/0107044}
\bibitem{hep-th/0107044}
K.~Becker and M.~Becker,
%``Supersymmetry breaking, M theory and fluxes,''
JHEP \textbf{07} (2001), 038
doi:10.1088/1126-6708/2001/07/038
[arXiv:hep-th/0107044 [hep-th]].
%131 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0907.0665}
\bibitem{0907.0665}
M.~Cicoli,
%``String Loop Moduli Stabilisation and Cosmology in IIB Flux Compactifications,''
Fortsch. Phys. \textbf{58} (2010), 115-338
doi:10.1002/prop.200900096
[arXiv:0907.0665 [hep-th]].
%18 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Wess:1992cp}
\bibitem{Wess:1992cp}
J.~Wess and J.~Bagger,
%``Supersymmetry and supergravity,''
%429 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Gates:1983nr}
\bibitem{Gates:1983nr}
S.~J.~Gates, M.~T.~Grisaru, M.~Rocek and W.~Siegel,
%``Superspace Or One Thousand and One Lessons in Supersymmetry,''
Front. Phys. \textbf{58} (1983), 1-548
[arXiv:hep-th/0108200 [hep-th]].
%811 citations counted in INSPIRE as of 20 Oct 2021

%\cite{hep-th/0105097}
\bibitem{hep-th/0105097}
S.~B.~Giddings, S.~Kachru and J.~Polchinski,
%``Hierarchies from fluxes in string compactifications,''
Phys. Rev. D \textbf{66} (2002), 106006
doi:10.1103/PhysRevD.66.106006
[arXiv:hep-th/0105097 [hep-th]].
%1940 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/9910053}
\bibitem{hep-th/9910053}
R.~C.~Myers,
%``Dielectric branes,''
JHEP \textbf{12} (1999), 022
doi:10.1088/1126-6708/1999/12/022
[arXiv:hep-th/9910053 [hep-th]].
%1364 citations counted in INSPIRE as of 14 Oct 2021

%\cite{hep-th/0007018}
\bibitem{hep-th/0007018}
J.~M.~Maldacena and C.~Nunez,
%``Supergravity description of field theories on curved manifolds and a no go theorem,''
Int. J. Mod. Phys. A \textbf{16} (2001), 822-855
doi:10.1142/S0217751X01003937
[arXiv:hep-th/0007018 [hep-th]].
%1016 citations counted in INSPIRE as of 12 Oct 2021

%\cite{hep-th/9602052}
\bibitem{hep-th/9602052}
J.~Polchinski, S.~Chaudhuri and C.~V.~Johnson,
%``Notes on D-branes,''
[arXiv:hep-th/9602052 [hep-th]].
%598 citations counted in INSPIRE as of 25 Oct 2021

%\cite{Johnson:2003glb}
\bibitem{Johnson:2003glb}
C.~V.~Johnson,
%``D-branes,''
doi:10.1017/CBO9780511606540
%50 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Becker:2006dvp}
\bibitem{Becker:2006dvp}
K.~Becker, M.~Becker and J.~H.~Schwarz,
%``String theory and M-theory: A modern introduction,''
%149 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Green:1987mn}
\bibitem{Green:1987mn}
M.~B.~Green, J.~H.~Schwarz and E.~Witten,
%``SUPERSTRING THEORY. VOL. 2: LOOP AMPLITUDES, ANOMALIES AND PHENOMENOLOGY,''
%249 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0007191}
\bibitem{hep-th/0007191}
I.~R.~Klebanov and M.~J.~Strassler,
%``Supergravity and a confining gauge theory: Duality cascades and chi SB resolution of naked singularities,''
JHEP \textbf{08} (2000), 052
doi:10.1088/1126-6708/2000/08/052
[arXiv:hep-th/0007191 [hep-th]].
%1780 citations counted in INSPIRE as of 22 Oct 2021

%\cite{0708.2865}
\bibitem{0708.2865}
C.~P.~Burgess,
%``Lectures on Cosmic Inflation and its Potential Stringy Realizations,''
PoS P \textbf{2GC} (2006), 008
doi:10.1088/0264-9381/24/21/S04
[arXiv:0708.2865 [hep-th]].
%151 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0710.2951}
\bibitem{0710.2951}
L.~McAllister and E.~Silverstein,
%``String Cosmology: A Review,''
Gen. Rel. Grav. \textbf{40} (2008), 565-605
doi:10.1007/s10714-007-0556-6
[arXiv:0710.2951 [hep-th]].
%326 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0808.2811}
\bibitem{0808.2811}
D.~Baumann, A.~Dymarsky, S.~Kachru, I.~R.~Klebanov and L.~McAllister,
%``Holographic Systematics of D-brane Inflation,''
JHEP \textbf{03} (2009), 093
doi:10.1088/1126-6708/2009/03/093
[arXiv:0808.2811 [hep-th]].
%94 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0802.2916}
\bibitem{0802.2916}
E.~Pajer,
%``Inflation at the Tip,''
JCAP \textbf{04} (2008), 031
doi:10.1088/1475-7516/2008/04/031
[arXiv:0802.2916 [hep-th]].
%47 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0810.5001}
\bibitem{0810.5001}
A.~Avgoustidis and I.~Zavala,
%``Warped Wilson Line DBI Inflation,''
JCAP \textbf{01} (2009), 045
doi:10.1088/1475-7516/2009/01/045
[arXiv:0810.5001 [hep-th]].
%27 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9912152}
\bibitem{hep-th/9912152}
T.~R.~Taylor and C.~Vafa,
%``R R flux on Calabi-Yau and partial supersymmetry breaking,''
Phys. Lett. B \textbf{474} (2000), 130-137
doi:10.1016/S0370-2693(00)00005-8
[arXiv:hep-th/9912152 [hep-th]].
%449 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0204254}
\bibitem{hep-th/0204254}
K.~Becker, M.~Becker, M.~Haack and J.~Louis,
%``Supersymmetry breaking and alpha-prime corrections to flux induced potentials,''
JHEP \textbf{06} (2002), 060
doi:10.1088/1126-6708/2002/06/060
[arXiv:hep-th/0204254 [hep-th]].
%409 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0208123}
\bibitem{hep-th/0208123}
O.~DeWolfe and S.~B.~Giddings,
%``Scales and hierarchies in warped compactifications and brane worlds,''
Phys. Rev. D \textbf{67} (2003), 066008
doi:10.1103/PhysRevD.67.066008
[arXiv:hep-th/0208123 [hep-th]].
%277 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/0403067}
\bibitem{hep-th/0403067}
T.~W.~Grimm and J.~Louis,
%``The Effective action of N = 1 Calabi-Yau orientifolds,''
Nucl. Phys. B \textbf{699} (2004), 387-426
doi:10.1016/j.nuclphysb.2004.08.005
[arXiv:hep-th/0403067 [hep-th]].
%365 citations counted in INSPIRE as of 13 Oct 2021

%\cite{deWit:1986mwo}
\bibitem{deWit:1986mwo}
B.~de Wit, D.~J.~Smit and N.~D.~Hari Dass,
%``Residual Supersymmetry of Compactified D=10 Supergravity,''
Nucl. Phys. B \textbf{283} (1987), 165
doi:10.1016/0550-3213(87)90267-7
%265 citations counted in INSPIRE as of 11 Oct 2021

%\cite{hep-th/9510017}
\bibitem{hep-th/9510017}
J.~Polchinski,
%``Dirichlet Branes and Ramond-Ramond charges,''
Phys. Rev. Lett. \textbf{75} (1995), 4724-4727
doi:10.1103/PhysRevLett.75.4724
[arXiv:hep-th/9510017 [hep-th]].
%2784 citations counted in INSPIRE as of 11 Oct 2021

%\cite{0803.1194}
\bibitem{0803.1194}
F.~Denef,
%``Les Houches Lectures on Constructing String Vacua,''
Les Houches \textbf{87} (2008), 483-610
[arXiv:0803.1194 [hep-th]].
%427 citations counted in INSPIRE as of 22 Oct 2021

%\cite{Cicoli:2007xp}
\bibitem{Cicoli:2007xp}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``Systematics of String Loop Corrections in Type IIB Calabi-Yau Flux Compactifications,''
JHEP \textbf{01} (2008), 052
doi:10.1088/1126-6708/2008/01/052
[arXiv:0708.1873 [hep-th]].
%174 citations counted in INSPIRE as of 14 Oct 2021

%\cite{Cicoli:2008va}
\bibitem{Cicoli:2008va}
M.~Cicoli, J.~P.~Conlon and F.~Quevedo,
%``General Analysis of LARGE Volume Scenarios with String Loop Moduli Stabilisation,''
JHEP \textbf{10} (2008), 105
doi:10.1088/1126-6708/2008/10/105
[arXiv:0805.1029 [hep-th]].
%162 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Kachru:2019dvo}
\bibitem{Kachru:2019dvo}
S.~Kachru, M.~Kim, L.~Mcallister and M.~Zimet,
%``de Sitter Vacua from Ten Dimensions,''
[arXiv:1908.04788 [hep-th]].
%38 citations counted in INSPIRE as of 11 Oct 2021

%\cite{AbdusSalam:2020ywo}
\bibitem{AbdusSalam:2020ywo}
S.~AbdusSalam, S.~Abel, M.~Cicoli, F.~Quevedo and P.~Shukla,
%``A systematic approach to K\"ahler moduli stabilisation,''
JHEP \textbf{08} (2020) no.08, 047
doi:10.1007/JHEP08(2020)047
[arXiv:2005.11329 [hep-th]].
%14 citations counted in INSPIRE as of 13 Oct 2021

%\cite{Cicoli:2021rub}
\bibitem{Cicoli:2021rub}
M.~Cicoli, F.~Quevedo, R.~Savelli, A.~Schachner and R.~Valandro,
%``Systematics of the $\alpha'$ Expansion in F-Theory,''
doi:10.1007/JHEP08(2021)099
[arXiv:2106.04592 [hep-th]].
%2 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Palti:2019pca}
\bibitem{Palti:2019pca}
E.~Palti,
%``The Swampland: Introduction and Review,''
Fortsch. Phys. \textbf{67} (2019) no.6, 1900037
doi:10.1002/prop.201900037
[arXiv:1903.06239 [hep-th]].
%431 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0509212}
\bibitem{hep-th/0509212}
C.~Vafa,
%``The String landscape and the swampland,''
[arXiv:hep-th/0509212 [hep-th]].
%618 citations counted in INSPIRE as of 25 Oct 2021

%\cite{hep-th/0605264}
\bibitem{hep-th/0605264}
H.~Ooguri and C.~Vafa,
%``On the Geometry of the String Landscape and the Swampland,''
Nucl. Phys. B \textbf{766} (2007), 21-33
doi:10.1016/j.nuclphysb.2006.10.033
[arXiv:hep-th/0605264 [hep-th]].
%590 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1610.00010}
\bibitem{1610.00010}
D.~Klaewer and E.~Palti,
%``Super-Planckian Spatial Field Variations and Quantum Gravity,''
JHEP \textbf{01} (2017), 088
doi:10.1007/JHEP01(2017)088
[arXiv:1610.00010 [hep-th]].
%176 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1602.06517}
\bibitem{1602.06517}
F.~Baume and E.~Palti,
%``Backreacted Axion Field Ranges in String Theory,''
JHEP \textbf{08} (2016), 043
doi:10.1007/JHEP08(2016)043
[arXiv:1602.06517 [hep-th]].
%105 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1903.06239}
\bibitem{1903.06239}
E.~Palti,
%``The Swampland: Introduction and Review,''
Fortsch. Phys. \textbf{67} (2019) no.6, 1900037
doi:10.1002/prop.201900037
[arXiv:1903.06239 [hep-th]].
%431 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1611.00394}
\bibitem{1611.00394}
I.~Valenzuela,
%``Backreaction Issues in Axion Monodromy and Minkowski 4-forms,''
JHEP \textbf{06} (2017), 098
doi:10.1007/JHEP06(2017)098
[arXiv:1611.00394 [hep-th]].
%74 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1611.07084}
\bibitem{1611.07084}
S.~Bielleman, L.~E.~Ibanez, F.~G.~Pedro, I.~Valenzuela and C.~Wieck,
%``Higgs-otic Inflation and Moduli Stabilization,''
JHEP \textbf{02} (2017), 073
doi:10.1007/JHEP02(2017)073
[arXiv:1611.07084 [hep-th]].
%28 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1703.05776}
\bibitem{1703.05776}
R.~Blumenhagen, I.~Valenzuela and F.~Wolf,
%``The Swampland Conjecture and F-term Axion Monodromy Inflation,''
JHEP \textbf{07} (2017), 145
doi:10.1007/JHEP07(2017)145
[arXiv:1703.05776 [hep-th]].
%95 citations counted in INSPIRE as of 13 Oct 2021

%\cite{1708.06761}
\bibitem{1708.06761}
A.~Hebecker, P.~Henkenjohann and L.~T.~Witkowski,
%``Flat Monodromies and a Moduli Space Size Conjecture,''
JHEP \textbf{12} (2017), 033
doi:10.1007/JHEP12(2017)033
[arXiv:1708.06761 [hep-th]].
%54 citations counted in INSPIRE as of 11 Oct 2021

%\cite{1801.05434}
\bibitem{1801.05434}
M.~Cicoli, D.~Ciupke, C.~Mayrhofer and P.~Shukla,
%``A Geometrical Upper Bound on the Inflaton Range,''
JHEP \textbf{05} (2018), 001
doi:10.1007/JHEP05(2018)001
[arXiv:1801.05434 [hep-th]].
%57 citations counted in INSPIRE as of 13 Oct 2021

%\cite{1904.05379}
\bibitem{1904.05379}
A.~Font, A.~Herr\'aez and L.~E.~Ib\'a\~nez,
%``The Swampland Distance Conjecture and Towers of Tensionless Branes,''
JHEP \textbf{08} (2019), 044
doi:10.1007/JHEP08(2019)044
[arXiv:1904.05379 [hep-th]].
%55 citations counted in INSPIRE as of 25 Oct 2021

%\cite{1806.09718}
\bibitem{1806.09718}
P.~Agrawal, G.~Obied, P.~J.~Steinhardt and C.~Vafa,
%``On the Cosmological Implications of the String Swampland,''
Phys. Lett. B \textbf{784} (2018), 271-276
doi:10.1016/j.physletb.2018.07.040
[arXiv:1806.09718 [hep-th]].
%354 citations counted in INSPIRE as of 22 Oct 2021

%\cite{1807.06581}
\bibitem{1807.06581}
F.~Denef, A.~Hebecker and T.~Wrase,
%``de Sitter swampland conjecture and the Higgs potential,''
Phys. Rev. D \textbf{98} (2018) no.8, 086004
doi:10.1103/PhysRevD.98.086004
[arXiv:1807.06581 [hep-th]].
%126 citations counted in INSPIRE as of 14 Oct 2021

%\cite{1807.05193}
\bibitem{1807.05193}
S.~K.~Garg and C.~Krishnan,
%``Bounds on Slow Roll and the de Sitter Swampland,''
JHEP \textbf{11} (2019), 075
doi:10.1007/JHEP11(2019)075
[arXiv:1807.05193 [hep-th]].
%387 citations counted in INSPIRE as of 22 Oct 2021

%\cite{1810.05506}
\bibitem{1810.05506}
H.~Ooguri, E.~Palti, G.~Shiu and C.~Vafa,
%``Distance and de Sitter Conjectures on the Swampland,''
Phys. Lett. B \textbf{788} (2019), 180-184
doi:10.1016/j.physletb.2018.11.018
[arXiv:1810.05506 [hep-th]].
%413 citations counted in INSPIRE as of 20 Oct 2021

%\cite{Dine:1985he}
\bibitem{Dine:1985he}
M.~Dine and N.~Seiberg,
%``Is the Superstring Weakly Coupled?,''
Phys. Lett. B \textbf{162} (1985), 299-302
doi:10.1016/0370-2693(85)90927-X
%357 citations counted in INSPIRE as of 15 Oct 2021

%\cite{2008.12399}
\bibitem{2008.12399}
M.~Dine, J.~A.~P.~Law-Smith, S.~Sun, D.~Wood and Y.~Yu,
%``Obstacles to Constructing de Sitter Space in String Theory,''
JHEP \textbf{02} (2021), 050
doi:10.1007/JHEP02(2021)050
[arXiv:2008.12399 [hep-th]].
%7 citations counted in INSPIRE as of 15 Oct 2021
